Efficient Federated Fine-Tuning of Large Language Models with Layer Dropout

Fine-tuning plays a crucial role in enabling pre-trained LLMs to evolve from general language comprehension to task-specific expertise. To preserve user data privacy, federated fine-tuning is often employed and has emerged as the de facto paradigm. However, federated fine-tuning is prohibitively inefficient due to the tension between LLM complexity and the resource constraint of end devices, incurring unaffordable fine-tuning overhead. Existing literature primarily utilizes parameter-efficient fine-tuning techniques to mitigate communication costs, yet computational and memory burdens continue to pose significant challenges for developers. This work proposes DropPEFT, an innovative federated PEFT framework that employs a novel stochastic transformer layer dropout method, enabling devices to deactivate a considerable fraction of LLMs layers during training, thereby eliminating the associated computational load and memory footprint. In DropPEFT, a key challenge is the proper configuration of dropout ratios for layers, as overhead and training performance are highly sensitive to this setting. To address this challenge, we adaptively assign optimal dropout-ratio configurations to devices through an exploration-exploitation strategy, achieving efficient and effective fine-tuning. Extensive experiments show that DropPEFT can achieve a 1.3-6.3\times speedup in model convergence and a 40%-67% reduction in memory footprint compared to state-of-the-art methods.

==> content/background.tex <==
We commence with challenges federated NLP faces based on our analysis of real-world datasets (\S \ref{subsec:challenges}). Next, we introduce state-of-the-art optimizations for federated NLP (\S \ref{subsec:state-of-the-art}) and highlight their key limitations (\S \ref{subsec:limitations}).



\subsection{Background of Federated NLP}\label{subsec:challenges}
\noindent \textbf{On-device fine-tuning is resource-intensive.} Given the large size of pre-trained language models, fine-tuning them for federated NLP requires significant computational resources. To illustrate, we fine-tune two popular language models (\ie, BERT \cite{devlin2018bert} and GPT-2 \cite{radford2019language}) on the Semeval dataset \cite{hendrickx2019semeval} using a Jetson TX2 device. As shown in Figure \ref{fig:on-device-overheads-memory}, the GPU memory footprints for fine-tuning these models reach approximately 3.1$\sim$10.5GB, which is 9.2$\sim$12.1$\times$ higher than that for typical CV tasks, such as training Densenet-121 \cite{huang2017densely} and ResNet-18 \cite{raffel2020exploring} on CeleBA \cite{liu2015deep}. Besides, Figure \ref{fig:on-device-overheads-time} shows that fine-tuning the language models for 100 batches ($batch\_size=16$) takes around 74.9$\sim$232.1 seconds, whereas training the CV models only requires 10.1$\sim$18.7 seconds. These results underscore the substantial computational resource demands of federated NLP.
% \begin{figure*}[t]\centering
%     \begin{minipage}[t]{0.232\linewidth}\centering
%         \subfigure[Adapter.]{\centering
%                 \label{fig:Adapter}
%                 \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/Adapter.pdf}
%             }
%     \end{minipage}
%     \begin{minipage}[t]{0.325\linewidth}\centering
%         \subfigure[LoRA.]{\centering
%                 \label{fig:LoRA}
%                 \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/LoRA.pdf}
%             }
%     \end{minipage}
%     \begin{minipage}[t]{0.4\linewidth}\centering
%         \subfigure[federated NLP with Adapter or LoRA.]{\centering
%                 \label{fig:federated-NLP}
%                 \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/federated-NLP.pdf}
%             }
%     \end{minipage}
%     \caption{Illustration of Adapter, LoRA and their applications in federated NLP.}\label{fig:parameter-efficient_fine-tuning}
% \end{figure*}\\

\noindent \textbf{Federated NLP incurs significant communication costs.} To investigate this, we conduct federated NLP experiments by fine-tuning BERT and GPT-2 across 100 TX2 devices on Semeval for 100 training rounds. The results indicate that total network traffic for model transmission between devices and the central server reaches 3493.2$\sim$51207GB, which is 100$\sim$212$\times$ greater than the traffic required for training Densenet-121 and ResNet-18 on CeleBA.\\
\textbf{Implications.} Federated NLP suffers from significant system inefficiencies due to the considerable costs of on-device computation and device-server communication. Notably, BERT and GPT-2 are relatively modest in scale compared to many popular LLMs, such as LLaMA 2-7B \cite{touvron2023llama} and T5 \cite{brown2020language}, which typically contain billions of parameters 
% (See Table \ref{table:popular_llms})
. Furthermore, practical federated NLP systems may involve thousands or even millions of participating devices \cite{bonawitz2019towards, hard2018federated}. Consequently, both computational and communication demands required for  real-world federated NLP deployments will further intensify.
\begin{figure}[t]\centering
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[GPU memory footprint.]{\centering
                \label{fig:on-device-overheads-memory}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/memory.pdf}
            }
    \end{minipage}
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[Training time for 100 batches.]{\centering
                \label{fig:on-device-overheads-time}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/time.pdf}
            }
    \end{minipage}
    \caption{On-device training overheads of federated NLP and CV tasks.}\label{fig:on-device-overheads}
\end{figure}
% \begin{table}[t]
%     \centering
%     \caption{Parameter number and size of popular CV/NLP models.} \label{table:popular_llms}
%     \resizebox{83mm}{!}{
%         \centering
%         \begin{tabular}{|c|c|c|cc|}  
%     		\hline
%     		% & & & \\[-6pt]  %可以避免文字偏上来调整文字与上边界的距离
%     		\multirow{2}{*}{Task} & \multirow{2}{*}{Model} & \multirow{2}{*}{\#Parameters} & \multicolumn{2}{c|}{Model Size} \\  % 表格中的内容，用&分开，\\表示下一行
%             % \cmidrule{4-5}
%             & & & Float 16 & Float 32 \\
%             \hline
%     		% & & & \\[-6pt]  %可以避免文字偏上 
%     		\multirow{4}{*}{CV} & CNN \cite{devlin2018bert} & 0.4 million & 0.7MB & 1.3MB \\
%             & VGG-19 \cite{simonyan2014very} & 1.5 million & 3.1MB & 6.2MB \\
%             & ResNet-18 \cite{raffel2020exploring} & 11 million & 22.3MB & 44.6MB \\
%             % & LLaMA 2-7B \cite{touvron2023llama} & 7 billion & 14.2GB & 28.4GB \\
            
%     		\hline
%     		% & & & \\[-6pt]  %可以避免文字偏上 
%     		\multirow{4}{*}{NLP} & BERT-Large \cite{devlin2018bert} & 0.4 billion & 0.7GB & 1.3GB \\
%             & GPT-2 \cite{radford2019language} & 1.5 billion & 3.1GB & 6.2GB \\
%             & T5 \cite{raffel2020exploring} & 11 billion & 22.3GB & 44.6GB \\
%             & LLaMA 2-7B \cite{touvron2023llama} & 7 billion & 14.2GB & 28.4GB \\
%             % Falcon \cite{almazrouei2023falcon} & 180 billion & 362.3GB & 724.6GB \\
%     		\hline
%         \end{tabular}
%     }
% \end{table}
% Given the large size of pre-trained LLMs, fine-tuning these models for federated NLP is extremely resource-intensive.
% For instance, according to the prior report \cite{cai2023efficient}, the end-to-end training towards full convergence of a federated NLP task (fine-tuning BERT \cite{devlin2018bert} on Semeval \cite{hendrickx2019semeval}) takes approximately 360 hours, which is 10$\times$ longer than a typical federated CV task, such as training Densenet-121 \cite{huang2017densely} on CeleBA \cite{liu2015deep}. Besides, our preliminary experiments (fine-tuning BERT with 100 devices on 20NEWS \cite{lang1995newsweeder}) indicate that total network traffic for model transmission between devices and the central server reaches 3493.2 GB, which is 100$\times$ higher than that of training Densenet-121 on CeleBA. It’s important to note that BERT, with 340 million parameters, is relatively modest in scale compared to many popular LLMs, such as LLaMA 2-7B \cite{touvron2023llama} and T5 \cite{brown2020language}, which typically contain billions of parameters (See Table \ref{table:popular_llms}). Furthermore, real-world federated NLP systems may involve thousands or even millions of participating devices \cite{bonawitz2019towards, hard2018federated}. Consequently, both computational and communication costs required for practical federated NLP will further intensify.

\subsection{Federated NLP Optimizations}\label{subsec:state-of-the-art}
% To reduce the significant overhead in federated NLP, recent works \cite{cai2023efficient, zhang2023fedpetuning, wang2024flora, bai2024fedspallm} introduce \emph{parameter-efficient fine-tuning} (PEFT) and \emph{model pruning} methods.

To reduce the significant overhead in federated NLP, many works \cite{cai2023efficient, zhang2023fedpetuning, wang2024flora, bai2024fedspallm} have proposed various optimization approaches, among which {parameter-efficient fine-tuning} (PEFT) and \emph{model pruning} are prominent techniques.

% Many studies have been conducted
% to mitigate the data heterogeneity through FL personalization.

\noindent \textbf{Federated NLP with PEFT.} 
% % The primary goal of PEFT is to reduce the number of trainable parameters during fine-tuning, thereby decreasing both computational and communication burdens in federated NLP. 
% Among the PEFT techniques, Adapter \cite{houlsby2019parameter} and LoRA \cite{hu2021lora} stand out as highly effective and straightforward for system deployment. As illustrated in Figure \ref{fig:parameter-efficient_fine-tuning}, Adapter inserts small, additional modules (adapters) into the transformer layers of a pre-trained network, while LoRA represents update of each dense layer (\eg, $\mathbf{W_{Q}}$ and $\mathbf{W_{K}}$) as two lower-rank matrices ($\mathbf{A}$ and $\mathbf{B}$) with significantly reduced dimensions. During fine-tuning, only these injected modules (in the case of Adapter) or low-rank matrices (in the case of LoRA) are updated, while the parameters in the original pre-trained network are frozen.
% State-of-the-art solutions such as AdaFL \cite{cai2023efficient}, FedPETuning \cite{zhang2023fedpetuning} and FedPipe \cite{fang2024automated} apply Adapter and LoRA to federated NLP tasks, achieving impressive gains in system efficiency. Figure \ref{fig:parameter-efficient_fine-tuning} outlines a high-level overview of the integration of Adapter and LoRA into federated NLP. Since Adapter and LoRA introduce only a small number of trainable parameters relative to the frozen parameters of the original pre-trained model, they significantly alleviate computational and communication overheads in federated NLP.
% % As shown in Table \ref{table:efficiency_peft}, compared to fine-tuning whole pre-trained models (\ie, full fine-tuning), computational time of PEFT is reduced by over 30\%, and network traffic decreases by approximately 99\%.\\
Among the PEFT techniques, Adapter \cite{houlsby2019parameter} and LoRA \cite{hu2021lora} stand out as highly effective and straightforward for system deployment. Adapter inserts small, additional modules (adapters) into the transformer layers of a pre-trained network, while LoRA represents update of each dense layer as two lower-rank matrices with significantly reduced dimensions. During fine-tuning, only these injected adapter modules or low-rank matrices are updated, while the parameters in the original pre-trained network are frozen.
Since Adapter and LoRA introduce only a small number of trainable parameters relative to the frozen parameters, they can significantly alleviate computational and communication overheads in federated NLP. State-of-the-art solutions such as AdaFL \cite{cai2023efficient}, FedPETuning \cite{zhang2023fedpetuning} and FedPipe \cite{fang2024automated} apply Adapter and LoRA to federated NLP tasks, achieving impressive gains in system efficiency.

\noindent \textbf{Federated NLP wtih model pruning.} Model pruning
% aims to 
reduces the size of pre-trained language models by cutting off some non-essential parameters. 
% with minimal model performance degradation.
Pruning techniques are generally classified into two categories, \ie, unstructured pruning \cite{frantar2023sparsegpt, sun2023simple, tuli2023acceltran} and structured pruning \cite{ma2023llm, tao2023structured, li2023losparse}. Unstructured pruning eliminates individual parameters without considering model structures, offering higher flexibility but requiring specialized hardware support to realize computational efficiency.
Conversely, structured pruning removes parameters of coupled structures, such as attention heads \cite{tao2023structured} and transformer layers \cite{yang2024laco}.
% , or dependency-based modules \cite{ma2023llm}.
Although structured pruning is less flexible, it is typically more compatible with hardware.
Recent studies propose diverse LLM pruning strategies to reduce fine-tuning complexity for federated NLP. For instance, PruFed \cite{bhansaliprufed} and FedSpaLLM \cite{bai2024fedspallm} propose to train compact models and transmit only a portion of the parameters to the server, thereby optimizing both computational and communication costs.


\subsection{Limitations of Status Quo}\label{subsec:limitations}
While existing federated NLP solutions have made considerable progress,
% in reducing training costs, 
they leave large optimization spaces in fully exploiting both system efficiency and model performance.\\
\textbf{PEFT is suboptimal in computing efficiency.} Fine-tuning the LLM on-device involves both the forward and backward passes. However, we observed that traditional PEFT methods only improve the efficiency of the backward pass but fail to reduce the computational demands of the forward pass. As shown in Figure \ref{fig:computing_path}, while PEFT freezes the parameters in the pre-trained network to avoid gradient calculation during the backward pass, the forward pass remains computationally burdensome. 
% The frozen parameters do not alter the computational graph and operations in the forward pass, leaving the full forward path intact. 
Common LLMs, such as LLaMA 2-7B, contain billions of parameters accessed during the forward pass, making it computationally demanding in terms of GPU memory and training time.
% Moreover, PEFT introduces additional structures (\eg, adapters or LoRA modules) into the network, which can further increase the computation complexity for forward pass due to the added operations.
To illustrate this, we fine-tune GPT-2 and LLaMA 2-7B on Semeval using an A6000 GPU, and record time for the forward pass, backward pass, and other tasks (\eg, data loading and optimizer stepping). As shown in Figure \ref{fig:breakdown-time}, 
% the backward pass is a major bottleneck in full fine-tuning, consuming nearly 60$\sim$63\% of total training time. 
although PEFT methods effectively reduce the backward pass computation, they fail to address the forward pass overhead, which now emerges as a primary bottleneck in model fine-tuning.
Consequently, the forward pass computation accounts for near 50\% of the total on device training time.
% Therefore, it is important to find a method that can effectively optimize both the forward and backward pass simultaneously.\\
% \textbf{Suboptimality in system efficiency.}
% % While PEFT methods in federated NLP can effectively reduce training overheads, they have limitations and optimization spaces in fully exploiting both system efficiency and model performance. 
% First, an entire local LLMs fine-tuning process includes both the forward and backward propagation steps. Traditional PEFT methods could only exploit the backward propagation efficiency but not that of forward propagation. Specifically, in PEFT process, freezing the original parameters in the pre-trained LLM can only avoid calculating their gradients in backward propagation. However, overall computational graph and operations remain largely unchanged, leading to original forward propagation path remaining intact. Besides, LoRA and Adapter introduce lightweight modules, which still require computation during the forward pass. In some cases, this can even lead to a slight increase in computation time due to the extra operations involved. As we illustrate in the following, such an inefficient computing strategy leaves a large room for improvement.
% To illustrate this, we conduct 

\begin{figure}[t]\centering
    \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/computing_path.pdf}
    \caption{Illustration of forward and backward passes in parameter-efficient fine-tuning.}\label{fig:computing_path}
\end{figure}
\begin{figure}[t]\centering
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[GPT-2.]{\centering
                \label{fig:breakdown-time-GPT-2}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/time-breakdown.pdf}
            }
    \end{minipage}
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[LLaMA 2-7B.]{\centering
                \label{fig:breakdown-time-LLaMA}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/time-breakdown.pdf}
            }
    \end{minipage}
    \caption{Breakdown of training time for fine-tuning models using an A6000 GPU.}\label{fig:breakdown-time}
\end{figure}

\noindent \textbf{Model pruning is inflexible and costly.} 
% Standard federated learning algorithms such as FedAvg \cite{mcmahan2017communication} assume that all local models share the same architecture with the global model. However, 
% in federated NLP systems, 
Devices in federated NLP always have different system capabilities \cite{lai2021oort, li2022pyramidfl}, necessitating heterogeneous pruning strategies tailored to the specific constraints of each device. This 
% directly violates the fundamental assumption in FL, thus 
requires significantly complicated algorithms to synchronize varying model architectures across devices. % while ensuring effective learning and convergence. 
Moreover, the system resources available on devices are not static; they change dynamically over time due to factors such as background processes, battery levels, or network conditions. Yet, model pruning is typically executed as a one-time process \cite{ma2023llm, zhang2024structured}. Once the model is pruned, the model size is completely fixed. Consequently, model pruning is incapable of adapting to the changing system resources on devices. These factors limit the practical applicability of model pruning in heterogeneous and dynamic environments.
% rigidity prevents model pruning from being responsive to temporal changes in device capabilities, limiting its practical applicability in dynamic environments.
\begin{figure}[t]\centering
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[GPT-2.]{\centering
                \label{fig:}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/acc-iid.pdf}
            }
    \end{minipage}
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[LLaMA 2-7B.]{\centering
                \label{fig:}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/acc-iid.pdf}
            }
    \end{minipage}
    \caption{PEFT and model pruning are suboptimal in model performance.}\label{fig:acc-iid}\vspace{-2mm}
\end{figure}
In addition to its inflexibility, performing model pruning, which is computationally intensive, inevitably incurs extra computational overhead on devices. This overhead is particularly problematic when the model size is huge.
% with large language models, whose substantial size and computational complexity exacerbate the issue. 
In federated NLP, devices always have limited computational resources \cite{cai2023efficient}. Additional pruning calculations can lead to higher energy consumption, increased training latency, and a larger memory footprint, which is undesirable for devices that are resource-constrained.

\noindent \textbf{PEFT and pruning suffer poor model performance.} 
% Fine-tuning only a subset of a model's parameters inherently constrains its ability to learn task-specific nuances, leading to suboptimal model performance compared to full fine-tuning.
% In federated NLP, this limitation is further exacerbated when each client possesses data that is not independently and identically distributed (non-IID). PEFT might not generalize effectively across these heterogeneous client datasets, leading to inconsistent and often inadequate performance \cite{zhang2023fedpetuning}. Moreover, model pruning typically relies on global importance measures of parameters, which are hard to compute without centralized data. Parameters deemed unimportant on one client's data may be crucial when considering the entire dataset distributed across all clients. The primary incentive for devices to participate in federated NLP is learning a global model that outperforms models trained locally \cite{li2021hermes}. However, when data heterogeneity is present, locally fine-tuned models often outperform the globally fine-tuned model produced by PEFT and pruning methods. This outcome not only undermines the fundamental motivation for federated NLP but also raises questions about the efficacy of these methods.
In federated NLP, local data across devices is not independently and identically distributed (non-IID) \cite{zhang2023fedpetuning, lin2021fednlp}. For
example, users in specific regions (\eg, France) predominantly
use certain languages (\eg, French), which may not be prevalent in other regions (\eg, Japan).
% leading to inconsistent and inadequate model performance \cite{zhang2023fedpetuning}. 
The heterogeneous data distribution can lead to inconsistent model updates when aggregated at the central server \cite{zhang2023fedpetuning}.
% Moreover, model pruning typically relies on global importance measures of parameters, which are hard to compute without centralized data. Parameters deemed unimportant on one device's data may be crucial when considering the entire dataset distributed across all devices.
Consequently, PEFT and model pruning often fail to generalize effectively across non-IID datasets. % and suffer suboptimal model performance.
% These facts lead to suboptimal model performance of PEFT and pruning 
% compared to full fine-tuning. 
To demonstrate this issue, we apply PEFT and model pruning to fine-tuning GPT-2 and LLaMA 2-7B using ONTONOTES over 100 communication rounds. In each round, we randomly select 10 out of 100 devices for training. Following prior works \cite{zhang2023fedpetuning, lin2021fednlp, cai2023efficient}, we generate non-IID data using three Dirichlet distributions, \ie, $Dir(10.0)$, $Dir(1.0)$, $Dir(0.1)$, which represent low, medium, and high non-IID degrees, respectively. As shown in Figure \ref{fig:acc-iid}, when the non-IID degree increases, the final accuracy of the PEFT and pruning methods (\ie, FedAdapter, FedLoRA and FedPruning) significantly degrades. Moreover, the primary incentive for devices to participate in federated NLP is learning a global model that outperforms models trained locally \cite{li2021hermes}. However, when data heterogeneity is present, locally fine-tuned models (\ie, LocalFT) often outperform the globally fine-tuned model produced by PEFT and pruning methods. Therefore, it is of a great challenge to train a one-fits-all model working consistently well for all devices with heterogeneous data.


% As shown in Figure \ref{fig:acc-iid}, 
% the final model accuracy of the PEFT and pruning methods (\ie, FedAdapter, FedLoRA and FedPruning) is far from that of full fine-tuning (\ie, FedFull). As the non-IID degree changes from low to high, the performance gaps between these methods and full fine-tuning even sharply increase.
% % the PEFT and pruning methods suffer poor model performance in non-IID situations.

% Moreover, the primary incentive for devices to participate in federated NLP is learning a global model that outperforms models trained locally \cite{li2021hermes}. However, when data heterogeneity is present, locally fine-tuned models (\ie, LocalFull) often outperform the globally fine-tuned model produced by PEFT and pruning methods, as shown in Figure \ref{fig:acc-iid}. This outcome not only undermines the fundamental motivation for federated NLP but also raises questions about the efficacy of these methods.

==> content/background1.tex <==
% We commence with the background (\ie, challenges and state-of-the-art optimizations) of federated fine-tuning (\S \ref{subsec:challenges}). Next, we highlight the key limitations in existing methods (\S \ref{subsec:limitations}).



\subsection{Parameter-Efficient Fine-Tuning}\label{subsec:challenges}
Given the large size of LLMs, federated fine-tuning requires significant computational resources. To illustrate, we fine-tune two popular LLMs (\ie, BERT \cite{devlin2018bert} and GPT-2 \cite{radford2019language}) on the Semeval dataset \cite{hendrickx2019semeval} using a common edge device, \ie, Jetson AGX Xavier \cite{agx}. As shown in Figure \ref{fig:on-device-overheads-memory}, fine-tuning the two models requires 6.7$\sim$31.5GB of GPU memory footprint, which is 9.2$\sim$12.1$\times$ higher than the demands for typical CV tasks, such as training Densenet-121 \cite{huang2017densely} and ResNet-18 \cite{raffel2020exploring} on CeleBA \cite{liu2015deep}. Besides, Figure \ref{fig:on-device-overheads-time} shows that fine-tuning BERT and GPT-2 for 100 batches ($batch\_size=16$) takes around 221.9$\sim$932.1 seconds, whereas training the CV models only requires 40.1$\sim$78.7 seconds. These results underscore the substantial training resource demands of federated fine-tuning. Notably, BERT and GPT-2 are relatively modest in scale compared to many popular LLMs, such as LLaMA 2-7B \cite{touvron2023llama} and T5 \cite{brown2020language}, which typically contain billions of parameters. Consequently, the training overheads required for practical federated fine-tuning deployments will further intensify.
\begin{figure}[t]\centering
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[GPU memory footprint.]{\centering
                \label{fig:on-device-overheads-memory}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/memory.pdf}
            }
    \end{minipage}
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[Training time for 100 batches.]{\centering
                \label{fig:on-device-overheads-time}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/time.pdf}
            }
    \end{minipage}
    \caption{Training overheads of federated fine-tuning and CV tasks.}\label{fig:on-device-overheads}
\end{figure}
% \begin{table}[t]
%     \centering
%     \caption{Parameter number and size of popular CV/NLP models.} \label{table:popular_llms}
%     \resizebox{83mm}{!}{
%         \centering
%         \begin{tabular}{|c|c|c|cc|}  
%     		\hline
%     		% & & & \\[-6pt]  %可以避免文字偏上来调整文字与上边界的距离
%     		\multirow{2}{*}{Task} & \multirow{2}{*}{Model} & \multirow{2}{*}{\#Parameters} & \multicolumn{2}{c|}{Model Size} \\  % 表格中的内容，用&分开，\\表示下一行
%             % \cmidrule{4-5}
%             & & & Float 16 & Float 32 \\
%             \hline
%     		% & & & \\[-6pt]  %可以避免文字偏上 
%     		\multirow{4}{*}{CV} & CNN \cite{devlin2018bert} & 0.4 million & 0.7MB & 1.3MB \\
%             & VGG-19 \cite{simonyan2014very} & 1.5 million & 3.1MB & 6.2MB \\
%             & ResNet-18 \cite{raffel2020exploring} & 11 million & 22.3MB & 44.6MB \\
%             % & LLaMA 2-7B \cite{touvron2023llama} & 7 billion & 14.2GB & 28.4GB \\
            
%     		\hline
%     		% & & & \\[-6pt]  %可以避免文字偏上 
%     		\multirow{4}{*}{NLP} & BERT-Large \cite{devlin2018bert} & 0.4 billion & 0.7GB & 1.3GB \\
%             & GPT-2 \cite{radford2019language} & 1.5 billion & 3.1GB & 6.2GB \\
%             & T5 \cite{raffel2020exploring} & 11 billion & 22.3GB & 44.6GB \\
%             & LLaMA 2-7B \cite{touvron2023llama} & 7 billion & 14.2GB & 28.4GB \\
%             % Falcon \cite{almazrouei2023falcon} & 180 billion & 362.3GB & 724.6GB \\
%     		\hline
%         \end{tabular}
%     }
% \end{table}
% Given the large size of pre-trained LLMs, fine-tuning these models for federated NLP is extremely resource-intensive.
% For instance, according to the prior report \cite{cai2023efficient}, the end-to-end training towards full convergence of a federated NLP task (fine-tuning BERT \cite{devlin2018bert} on Semeval \cite{hendrickx2019semeval}) takes approximately 360 hours, which is 10$\times$ longer than a typical federated CV task, such as training Densenet-121 \cite{huang2017densely} on CeleBA \cite{liu2015deep}. Besides, our preliminary experiments (fine-tuning BERT with 100 devices on 20NEWS \cite{lang1995newsweeder}) indicate that total network traffic for model transmission between devices and the central server reaches 3493.2 GB, which is 100$\times$ higher than that of training Densenet-121 on CeleBA. It’s important to note that BERT, with 340 million parameters, is relatively modest in scale compared to many popular LLMs, such as LLaMA 2-7B \cite{touvron2023llama} and T5 \cite{brown2020language}, which typically contain billions of parameters (See Table \ref{table:popular_llms}). Furthermore, real-world federated NLP systems may involve thousands or even millions of participating devices \cite{bonawitz2019towards, hard2018federated}. Consequently, both computational and communication costs required for practical federated NLP will further intensify.

% \subsection{Federated Parameter-Efficient Fine-Tuning}\label{subsec:state-of-the-art}
% To reduce the significant overhead in federated NLP, recent works \cite{cai2023efficient, zhang2023fedpetuning, wang2024flora, bai2024fedspallm} introduce \emph{parameter-efficient fine-tuning} (PEFT) and \emph{model pruning} methods.

% \begin{figure}[t]\centering
%     \begin{minipage}[t]{0.495\linewidth}\centering
%         \subfigure[]{\centering
%                 \label{fig:}
%                 \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/Adapter.pdf}
%             }
%     \end{minipage}
%     \begin{minipage}[t]{0.495\linewidth}\centering
%         \subfigure[]{\centering
%                 \label{fig:}
%                 \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/LoRA.pdf}
%             }
%     \end{minipage}
%     \caption{}\label{fig:}
% \end{figure}

To mitigate the significant overheads, federated parameter-efficient fine-tuning (PEFT) \cite{cai2023efficient, zhang2023fedpetuning, jiang2023low, cho2023heterogeneous} is the most common and straightforward approach. Among the PEFT techniques, Adapter \cite{houlsby2019parameter} and LoRA \cite{hu2021lora} stand out as highly effective for system deployment. Specifically, Adapter inserts small, additional modules (adapters) into the transformer layers of the LLM, while LoRA represents update of each dense layer as two lower-rank matrices with significantly reduced dimensions. During fine-tuning, only these injected adapter modules or low-rank matrices are updated, while the parameters in the original LLM are frozen.
Since Adapter and LoRA introduce only a small number of trainable parameters relative to the frozen ones, they can alleviate the majority of computational time and memory footprint associated with gradient calculations. Recently, state-of-the-art solutions such as AdaFL \cite{cai2023efficient} and FedPETuning \cite{zhang2023fedpetuning} have applied PEFT methods to federated fine-tuning tasks, achieving impressive gains in training efficiency.


\subsection{Bottlenecks of PEFT}\label{subsec:limitations}
While existing PEFT solutions have made considerable progress, they leave large optimization spaces in fully exploiting the training efficiency.

% First, fine-tuning the LLM involves both the forward and backward passes. However, we observed that traditional PEFT methods only improve the efficiency of the backward pass but fail to reduce the computational demands of the forward pass. As shown in Figure \ref{fig:computing_path}, while PEFT freezes the parameters in the base LLM to avoid gradient calculations during the backward pass, the forward pass remains computationally burdensome. Parameter freeze does not alter the computational graph and operations in the forward pass, leaving the original forward path in the base LLM intact. 
% Common LLMs, such as LLaMA 2-7B, contain billions of parameters accessed during the forward pass, making it computationally demanding in terms of training time.
% % Moreover, PEFT introduces additional structures (\eg, adapters or LoRA modules) into the network, which can further increase the computation complexity for forward pass due to the added operations.
% To illustrate this, we fine-tune GPT-2 and LLaMA 2-7B on Semeval using an A6000 GPU, and record time for the forward pass, backward pass, and other tasks (\eg, data loading and optimizer stepping). As shown in Figure \ref{fig:breakdown-time}, 
% % the backward pass is a major bottleneck in full fine-tuning, consuming nearly 60$\sim$63\% of total training time. 
% although PEFT methods reduce the backward pass computation time, they fail to address the forward pass overhead.
% Consequently, the forward pass computation accounts for near 45\% of the total training time, emerging as a primary bottleneck in LLM fine-tuning.
% % Therefore, it is important to find a method that can effectively optimize both the forward and backward pass simultaneously.\\

\begin{figure}[t]\centering
    \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/computing_path.pdf}
    \caption{Illustration of forward and backward passes in parameter-efficient fine-tuning.}\label{fig:computing_path}
\end{figure}
\begin{figure}[t]\centering
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[GPT-2.]{\centering
                \label{fig:breakdown-time-GPT-2}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/time-breakdown.pdf}
            }
    \end{minipage}
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[LLaMA 2-7B.]{\centering
                \label{fig:breakdown-time-LLaMA}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/time-breakdown.pdf}
            }
    \end{minipage}
    \caption{Breakdown of training time for fine-tuning models using an A6000 GPU.}\label{fig:breakdown-time}
\end{figure}

\noindent \textbf{PEFT leaves the forward pass computationally costly.} 
% Fine-tuning the LLM involves both the forward and backward passes. 
The computational overhead in LLM fine-tuning is dominated by the forward and backward passes of the LLM’s backbone \cite{dettmers2023qlora}.
However, we observe that traditional PEFT methods only improve the efficiency of the backward pass but fail to reduce the computational demands of the forward pass. As shown in Figure \ref{fig:computing_path}, while PEFT freezes the parameters in the base LLM to avoid gradient calculations during the backward pass, it does not alter the computational graph in the forward pass, leaving the original forward path in the base LLM intact. Common LLMs, such as LLaMA 2-7B, contain billions of parameters accessed during the forward pass, making it computationally demanding in terms of training time. Moreover, PEFT introduces additional modules, which further increase the computation complexity for the forward pass. To illustrate this, we fine-tune GPT-2 and LLaMA 2-7B on the Semeval dataset using an A6000 GPU. During model fine-tuning, we record time for the forward pass, backward pass, and other tasks (\eg, data loading and optimizer stepping), respectively. As shown in Figure \ref{fig:breakdown-time}, although PEFT methods reduce the backward pass computation time, they fail to address the forward pass overhead. Consequently, the forward pass computation accounts for near 45\% of the total training time, emerging as a primary bottleneck in LLM fine-tuning.

\begin{figure}[t]\centering
    \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/memory_breakdown.pdf}
    \caption{Breakdown of GPU memory footprint with a batch size of 16, maximum sequence length of 256 \cite{MicrosoftDeberta}, and the commonly used Adamw optimizer (BF16 numerical
format) \cite{loshchilov2017decoupled}.}\label{fig:breakdown_memory}
\end{figure}


\noindent \textbf{Memory overheads of PEFT is significant due to the large size of activations.} To better understand the gap between the memory needed in existing PEFT techniques and the memory available on devices, we profile the memory requirements to fine-tune the DeBERTaV2-xxlarge model on the MNLI dataset. As shown in Figure \ref{fig:breakdown_memory}, the memory footprint for FFT includes storing the LLM’s parameters (10.9\%, grey), activations (54.9\%, orange), gradients (11.3\%, green), and optimizer states (22.9\%, blue). Even after the PEFT methods frozen the LLM parameters to alleviate the storage usage for gradients and optimizer states, the overall memory is still significant due to the \emph{unreduced} activations size (80\% of the total). The reason is that, activations are intermediate outputs of each layer during the forward pass, required for computing gradients in the backward pass (Figure \ref{fig:computing_path}). Their memory footprint is determined by: model depth $L$ (number of transformer layers), number of attention heads per layer $a$, hidden dimensions $h$ (size of intermediate representations), batch size $b$ and sequence length $s$, \ie, $activation\_size=(34bsh + 5bs^2a) \times L$ \cite{korthikanti2023reducing}. However, PEFT modifies only a small subset of parameters (\eg, via low-rank matrices or adapter modules) but preserve the original LLM's architecture, \ie, unchanged $L$ and $a$. Thus, activations from all layers must still be stored. Consequently, there remains a $1.58\sim2.37\times$ gap between the memory required for PEFT and the memory available on commonly used edge devices, \eg, 8GB for TX2 \cite{tx2} and 12GB for Quest Pro \cite{questpro}.

\noindent \textbf{Implications.} PEFT suffers from significant inefficiencies in terms of considerable computational taxes and memory overheads. While typical devices in the federated fine-tuning system always have limited resources, PEFT's costly nature hinders adoption in real-world tasks. To enable practical federated fine-tuning with a tolerable convergence delay (\eg, a few hours) and memory consumption, the model structure and training paradigm need to be re-architected.

% \begin{figure}[t]\centering
%     \begin{minipage}[t]{0.495\linewidth}\centering
%         \subfigure[GPT-2.]{\centering
%                 \label{fig:}
%                 \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/acc-iid.pdf}
%             }
%     \end{minipage}
%     \begin{minipage}[t]{0.495\linewidth}\centering
%         \subfigure[LLaMA 2-7B.]{\centering
%                 \label{fig:}
%                 \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/acc-iid.pdf}
%             }
%     \end{minipage}
%     \caption{PEFT and model pruning are suboptimal in model performance.}\label{fig:acc-iid}\vspace{-2mm}
% \end{figure}

% \noindent \textbf{PEFT suffers poor model performance.} 
% % Fine-tuning only a subset of a model's parameters inherently constrains its ability to learn task-specific nuances, leading to suboptimal model performance compared to full fine-tuning.
% % In federated NLP, this limitation is further exacerbated when each client possesses data that is not independently and identically distributed (non-IID). PEFT might not generalize effectively across these heterogeneous client datasets, leading to inconsistent and often inadequate performance \cite{zhang2023fedpetuning}. Moreover, model pruning typically relies on global importance measures of parameters, which are hard to compute without centralized data. Parameters deemed unimportant on one client's data may be crucial when considering the entire dataset distributed across all clients. The primary incentive for devices to participate in federated NLP is learning a global model that outperforms models trained locally \cite{li2021hermes}. However, when data heterogeneity is present, locally fine-tuned models often outperform the globally fine-tuned model produced by PEFT and pruning methods. This outcome not only undermines the fundamental motivation for federated NLP but also raises questions about the efficacy of these methods.
% In federated fine-tuning, local data across devices is not independently and identically distributed (non-IID) \cite{zhang2023fedpetuning, lin2021fednlp}. For example, users in specific regions (\eg, France) predominantly
% use certain languages (\eg, French), which may not be prevalent in other regions (\eg, Japan).
% % leading to inconsistent and inadequate model performance \cite{zhang2023fedpetuning}. 
% The heterogeneous data distribution can lead to inconsistent model updates when aggregated at the central server \cite{zhang2023fedpetuning}.
% % Moreover, model pruning typically relies on global importance measures of parameters, which are hard to compute without centralized data. Parameters deemed unimportant on one device's data may be crucial when considering the entire dataset distributed across all devices.
% Consequently, PEFT often fails to generalize effectively across non-IID datasets. % and suffer suboptimal model performance.
% % These facts lead to suboptimal model performance of PEFT and pruning 
% % compared to full fine-tuning. 
% To demonstrate this issue, we apply two state-of-the-art PEFT methods to fine-tuning GPT-2 and LLaMA 2-7B using ONTONOTES over 100 communication rounds. In each round, we randomly select 10 out of 100 devices for training. Following prior works \cite{zhang2023fedpetuning, lin2021fednlp, cai2023efficient}, we generate non-IID data using three Dirichlet distributions, \ie, $Dir(10.0)$, $Dir(1.0)$, $Dir(0.1)$, which represent low, medium, and high non-IID degrees, respectively. As shown in Figure \ref{fig:acc-iid}, when the non-IID degree increases, the final accuracy of the PEFT methods (\ie, FedAdapter, FedLoRA) significantly degrades. Moreover, the primary incentive for devices to participate in federated fine-tuning is learning a global model that outperforms models trained locally \cite{li2021hermes}. However, when data heterogeneity is present, locally fine-tuned models (\ie, LocalFT) often outperform the globally fine-tuned model produced by PEFT. Therefore, it is of a great challenge to train a one-fits-all model working consistently well for all devices with heterogeneous data.


% As shown in Figure \ref{fig:acc-iid}, 
% the final model accuracy of the PEFT and pruning methods (\ie, FedAdapter, FedLoRA and FedPruning) is far from that of full fine-tuning (\ie, FedFull). As the non-IID degree changes from low to high, the performance gaps between these methods and full fine-tuning even sharply increase.
% % the PEFT and pruning methods suffer poor model performance in non-IID situations.

% Moreover, the primary incentive for devices to participate in federated NLP is learning a global model that outperforms models trained locally \cite{li2021hermes}. However, when data heterogeneity is present, locally fine-tuned models (\ie, LocalFull) often outperform the globally fine-tuned model produced by PEFT and pruning methods, as shown in Figure \ref{fig:acc-iid}. This outcome not only undermines the fundamental motivation for federated NLP but also raises questions about the efficacy of these methods.

==> content/design.tex <==
Despite the limitations of existing PEFT techniques, we also identify opportunities for improving upon these methods to develop efficient federated fine-tuning frameworks. Our analysis in \S\ref{} demonstrates that the massive scale of LLMs, exemplified by DeBERTa-xxlarge with its 48 transformer layers, inherently amplifies fine-tuning costs. Current PEFT approaches exacerbate this issue by typically updating trainable parameters across most or all transformer layers, rendering them impractical for resource-constrained environments. To overcome this barrier, one intuitive yet radical approach might involve cutting down the size of LLMs by pruning the model depth. For example, halving the layers in DeBERTaV2 to $24$ could theoretically slash training latency and memory usage by about $50\%$.
However, such a brute-force transformer-layer reduction risks disrupting the capabilities of LLMs. Neural scaling laws \cite{sorscher2022beyond, kaplan2020scaling} confirm that LLM performance scales predictably with depth, as deeper architectures capture more comprehensive semantic information. Therefore, immediate gains in efficiency by removing transformer layers come at the cost of irreversible damage to LLM capability. This prompts a pivotal question: \emph{Can PEFT methods be redesigned to strategically alleviate computational and memory burdens of certain layers without compromising the intrinsic fidelity of LLMs?}
% bypass selected layers, thereby eliminating both their computational and memory burdens, without compromising the fidelity of LLMs?}

% This paradox forces a reckoning: how can federated systems balance efficiency with the depth required for sophisticated language understanding?



% the fundamental reason for significant computational and storage overhead of fine-tuning is the enormous size of the LLM, which includes a considerable number of transformer layers, \eg, $48$ for DeBERTa-xxlarge. Prior PEFT methods update PEFT modules in all (most if not all) these layers by default, making the fine-tuning overhead unaffordable for resource-constrained end devices. To break through this resource barrier, reducing the number of transformer layers in the LLM is an straightforward approach. For instance, if we cut off $24$ transformer layers in DeBERTaV2-xxlarge, both the training delay and memory footprint for fine-tuning can dramatically decrease by about $50\%$. However, the famous neural scaling law \cite{sorscher2022beyond, kaplan2020scaling} shows that the performance of a LLM tends to improve in a predictable manner as training deeper neural networks. Therefore, directly removing transformer layers from a LLM by violence can lead to a significant decline in model performance.

% % The researcher is faced with an inherent dilemma: shorter networks have
% % the advantage that information flows efficiently forward and backward, and can
% % therefore be trained effectively and within a reasonable amount of time. However,
% % they are not expressive enough to represent the complex concepts that are
% % commonplace in computer vision applications. Very deep networks have much
% % greather model complexity, but are very difficult to train in practice and require
% % a lot of time and patience.
% In this paper, we propose deep networks with stochastic depth, a novel training
% algorithm that is based on the seemingly contradictory insight that ideally
% we would like to have a deep network during testing but a short network during
% training. We resolve this conflict by creating deep Residual Network [8] architectures
% (with hundreds or even thousands of layers) with sufficient modeling
% capacity; however, during training we shorten the network significantly by randomly
% removing a substantial fraction of layers independently for each sample or
% mini-batch. The effect is a network with a small expected depth during training,
% but a large depth during testing. Although seemingly simple, this approach is
% surprisingly effective in practice.

\subsection{Overview}
In this work, we propose DropPEFT, an enhanced federated PEFT framework that improves the fine-tuning efficiency through a novel \emph{stochastic transformer layer dropout (STLD)} technique. DropPEFT employs
a similar training process as traditional federated PEFT framework but mainly differs on the local fine-tuning paradigm. In each global round, the central server first sends the latest trainable PEFT modules to available devices. Then each device inserts these modules into corresponding transformer layers of the local LLM, which is fine-tuned on the device's local training data by the STLD method for several mini-batches. The key idea behind STLD roots in the seemingly paradoxical insight that maximal LLM depth is essential for superior model performance, but a short network is beneficial for efficient fine-tuning. At its core, during local fine-tuning, STLD dynamically shortens the active network depth by randomly skipping a substantial fraction of transformer layers independently for each mini-batch, while retaining the LLM's full original architecture post-training. Finally, the devices upload the parameter updates in PEFT modules from all transformer layers to the server for global aggregation.

\noindent \textbf{Advantages of DropPEFT by design.} 
% STLD offers three pivotal advantages. 
First, by deactivating selected layers, STLD circumvents both forward and backward computations for those layers, thereby significantly reducing computational overhead. Second, the omission of these layers during computation eliminates the need to store intermediate activations, gradients, and optimizer states, thus alleviating memory constraints. Finally, unlike permanent pruning techniques, STLD retains all layers after training, ensuring that the LLM’s representational capacity is maximally preserved.

% STLD bypasses both forward and backward computations for deactivated layers. Second, deactivated layers obviate the need to store intermediate activations, gradients, or optimizer states, decreasing memory usage. Moreover, unlike permanent pruning, STLD retains all layers post-training, ensuring no degradation of the pre-trained LLM’s inherent capabilities.


% Crucially, the full model depth remains intact post-training, preserving the LLM’s original capabilities.


% which is based on the seemingly contradictory insight that ideally we would like to have a deep LLM structure but a short network during fine-tuning. 
% The key idea behind this technology is to shorten the network significantly by randomly deactivating (or skipping) a substantial fraction of transformer layers independently for each
% mini-batch during fine-tuning.
% In this way, the computations of both the forward and backward passes of these deactivated layers can be bypassed. Besides, devices do not need considerable memory to store activations, gradients or optimizer states for these deactivated layers. Notably, the effect is a LLM with a small expected depth during fine-tuning,
% but a large depth (\ie, with all layers) once fine-tuning complete.


% aimed at efficient federated fine-tuning. The key idea behind this technology is to dynamically deactivate (or skip) certain transformer layers during fine-tuning, without disrupting the internal data flow of the LLM (\S \ref{}). 
% In this way, the computations of both the forward and backward passes of these deactivated layers can be bypassed. Besides, devices do not need considerable memory to store activations, gradients or optimizer states for these deactivated layer. 


% Addressing the shortcomings of PEFT and model pruning necessitates the development of a more advanced training paradigm. First, this paradigm must ensure the on-device training efficiency by simultaneously optimizing both the forward and backward passes. 
% Second, it should enable the flexible extraction of subnetworks from the original model, tailored to real-time resource constraints.
% %, such as memory availability and training time. 
% Crucially, this extraction process must be straightforward and introduce no additional overhead for devices. 
% Additionally, this paradigm should facilitate the training of high-performance models that perform consistently well across all devices, despite heterogeneity in data distributions. 
% To achieve these goals, we exploit a unique characteristic of LLMs: 
% % LLMs are built by stacking multiple \emph{transformer layers} \cite{vaswani2017attention}, each processing hidden states that encapsulate contextual information of the input tokens. Every transformer layer has the same structure and dimensions and update the hidden states uniformly across the model.
% they are composed of multiple stacked \emph{transformer layers} \cite{vaswani2017attention}, each sharing the same structure. As input data flows through these layers, the model generates hidden states, which are internal representations of the input sequence. All hidden states have the same dimensions across transformer layers.
% % Importantly, the hidden states produced by each transformer layer have the same dimensions. 
% Leveraging this uniformity, we propose two novel federated NLP technologies, \ie, \emph{stochastic transformer layer dropout} and \emph{personalized transformer layer sharing}, aimed at efficient and effective model training.
% To achieve these goals, we propose two novel technologies, \ie, \emph{stochastic transformer layer dropout} and \emph{personalized transformer layer sharing}, aimed at efficient and effective model training.

% \noindent \textbf{Layer dropout for efficient on-device training.} The key idea behind stochastic transformer layer dropout is to 
% % exploit the uniformity of the transformer layers, so we can 
% dynamically deactivate (or skip) certain layers during on-device training 
% % without disrupting the internal data flow of the model (\S \ref{}). 
% In this way, the computations of both the forward and backward passes of these deactivated layers can be bypassed. By allowing devices to deactivate layers that are less relevant to their local data or less critical for performance, layer dropout enables a more efficient training process. 
% Importantly, this method itself incurs no additional computational overhead, as skipping layers requires no extra calculations of activations or gradients. 
% Moreover, layer dropout can be dynamically adjusted in each batch of training based on available memory and processing power, providing greater flexibility in adapting to changing device capabilities.

% Moreover, in the context of federated NLP, layer dropout can be particularly beneficial for handling the heterogeneous system capabilities across different devices by adjusting the number of layers used during training. 

% \noindent \textbf{Personalized layer sharing for non-IID data.} While traditional federated NLP aims to create a global model that benefits all clients, it often fails to account for the inherent heterogeneity of client data distributions. We propose personalized transformer layer sharing to address this challenge by allowing models to be tailored to the individual characteristics of each device. Specifically, rather than sharing the entire model, we propose extracting personalized subsets of layers from the full model for global aggregating, based on each device' data characteristics.
% This allows some layers to learn global knowledge while others to learn device-specific data features. 
% % Unlike the traditional federated NLP approaches, which may lead to a one-size-fits-all solution, personalized fine-tuning ensures that each client’s model remains relevant and optimized for its specific context. 
% % Additionally, this approach mitigates the risk of catastrophic forgetting, where a global model fails to retain knowledge that is valuable for particular devices. 
% As a result, personalized fine-tuning provides a solution that balances the trade-off between generalization and specialization.

% \noindent \textbf{Synergy of layer dropout and personalized layer sharing.} The integration of stochastic layer dropout with personalized layer sharing offers a synergistic opportunity to further advance federated fine-tuning. By incorporating both techniques, the system can not only personalize the model to each client’s data but also optimize the resources required for training. This combination enables clients to focus on learning the most relevant features for their own data while ensuring that only the necessary parts of the model are trained and shared. Furthermore, these techniques can also contribute to enhancing privacy and security in federated NLP systems, as they reduce the amount of shared model information, potentially lowering the risk of privacy leakage.


\subsection{Stochastic Transformer Layer Dropout} \label{sec:layer_dropout}
We begin by reviewing the architecture of LLMs, which naturally lends itself to the design of STLD.
LLMs are constructed by stacking $L$ structurally identical transformer layers, each acting as a fundamental building block. Between any two adjacent layers, hidden states serve as intermediate representations of the input sequences. More formally, each transformer layer $l$ processes the hidden states $H_l$ to yield higher-level representations $H_{l+1}$:
% Each transformer layer $l$ transforms the hidden states $H_l$, output by layer $l$, to higher-level representations $H_{l+1}$:  
% For each transformer layer $l$, the hidden states $H_{l}$ are transformed to the input for the next layer:
\begin{equation} \label{eq:transformer_layer}
    H_{l+1} = TransforBlock_{l}(H_l),
\end{equation}
where $TransforBlock_{l}(\cdot)$ denotes the transformation function applied within transformer layer $l$ to the input $H_l$. This function encapsulates all computations within the layer, including the self-attention and feed-forward processes \cite{vaswani2017attention}. In the context of PEFT methods, $TransforBlock_{l}(\cdot)$ further integrates computations associated with inserted PEFT modules (\eg, adapters or low-rank matrices). Typically, the hidden states across all layers maintain a consistent dimensionality.

% \subsubsection{Fine-tuning with stochastic transformer layers} The 
% % uniformity and 
% stacked structure of transformer layers prompt considerations about the depth and capacity of LLMs. While increasing model depth can potentially capture more intricate contextual patterns, it also amplifies computational overhead and complicates training. 
% In many situations, pre-trained LLMs contain redundant parameters and layers, suggesting that not all layers are equally critical for achieving robust performance \cite{michel2019sixteen, voita2019analyzing}. This makes it possible to carefully reducing their effective depth during fine-tuning without significantly sacrificing model quality.
\begin{figure}[t]\centering
    \includegraphics[width=1.0\linewidth]{content/picture/design_chapter/deactivated_layer.pdf}
    \caption{A close look at the deactivated transformer layer $l$ with an identity function.}\label{fig:dropped-layer}
\end{figure}
% To exploit this insight, we propose \emph{stochastic transformer layer dropout}, which leverages shallower network configurations throughout fine-tuning, yet preserves the capacity of the full model at inference time.

% which enables us to fine-tune LLMs using shallower networks while retaining access to the full depth of the model at inference time. 

The core of this method is to construct and train shorter subnetworks on-the-fly by randomly deactivating certain transformer layers during training. Specifically, for each training batch, we randomly and independently select a subset of layers to skip their transformation functions. Figures \ref{fig:dropped-layer} offers a schematic view of a deactivated layer. If a transformer layer $l$ is chosen to be deactivated, the hidden states $H_{l}$ are passed through an identity function rather than the transformation function $TransforBlock_{l}(\cdot)$:
\begin{equation}
    H_{l+1} = Identity(H_{l})
\end{equation}
where $Identity(\cdot)$ simply returns the input unchanged.
% and introduces no additional computational overhead. 
If the layer $l$ remains active, the original transformation in Equation~\eqref{eq:transformer_layer} is applied as usual. To model the process of selecting which layers to deactivate, we introduce a binary random variable $d_l \in \{0,1\}$ for each layer $l$. Here, $d_l = 1$ denotes that the layer is deactivated, while $d_l = 0$ indicates the layer is activated.
% We formalize this selection process by introducing a binary variable $d_l \in \{0, 1\}$ for each layer $l$, where $d_l = 1$ indicates deactivation of the layer. 
Under this definition, the resulting computation for transformer layer $l$ is updated as follows:
\begin{equation}\label{eq:layer-dropout}
    H_{l+1} = (1-d_l) \cdot TransforBlock_l(H_l) + d_l \cdot Identity(H_l)
\end{equation}
where the probability of $d_l = 1$, \ie, the drop rate for layer $l$, is $P_l \in \left[0, 1\right)$. By assigning distinct drop rates to each layer, we ensure that all layers have opportunities to contribute to the fine-tuning process across training batches.

% These selected transformer layers are bypassed with the identity function $Identity(\cdot)$, which returns its input without any changes. That means if the transformer layer $l$ is deactivated, we obtain $H_{l+1} = Identity(H_{l})$, instead of $H_{l+1} = TransforBlock_l(H_{l})$. 
% In order to allow all layers to have a chance to participate in fine-tuning, we assign different deactivation probabilities (\ie, drop rates) to each layer, and stochastically discard it at each batch of training. 
% We use a variable $d_l$ with a value of $\{0, 1\}$ to indicate whether the transformer layer $l$ is activated ($d_l = 0$) or deactivated ($d_l = 1$). With this definition, we change the computations of the original transformer layer $l$ as follows:
% \begin{equation}
%     H_{l+1} = (1-d_l) \cdot TransforBlock_l(H_l) + d_l \cdot Identity(H_l)
% \end{equation}
% where the probability of $d_l = 1$ is $P_l \in \left[0, 1\right)$, \ie, the drop rate of the layer $l$. If $d_l = 1$, the computations degenerate to $H_{l+1}=Identity(H_l)$, otherwise to Equation \eqref{eq:transformer_layer}.

Training with stochastic layer dropout can be viewed as training an ensemble of subnetworks that share the parameters in the overlapping layers. Specifically, with $L$ layers in the model, there are $2^L$ possible subnetwork configurations, each corresponding to a different combination of active and inactive layers. In each training batch, one of these subnetworks is selected for updating. This encourages the model to generalize better by preventing over-reliance on any particular subnetwork. Unlike model pruning, which permanently removes layers or units from the model, stochastic layer dropout can retain a full model at inference time by keeping all transformer layers active.
Therefore, it achieves efficiency during training while still benefiting from the representational richness of the complete architecture during inference. Figure~\ref{code:stochastic_layer_dropout} presents a code example of stochastic transformer layer dropout. Notably, this approach accelerates training by effectively reducing the number of active layers without requiring any specialized hardware or software kernels. Moreover, the layer dropout operation itself does not introduce any additional computational or storage overhead during both training and inference.



\lstdefinelanguage{mypython}{        % 设置代码环境
  sensitive=true,
  % 设置关键字
  keywords={def,class,return,if,else,import,as,for,in, self, range}, % 第一组关键字
  morekeywords=[2]{int,str,bool,None}, % 第二组关键字
  otherkeywords={->},          % 将非字母的字符串识别为关键字，例如->
  keywordstyle=\color{dkblue}\bfseries,  % 设置第一组关键字的样式
  keywordstyle=[2]\color{magenta}\bfseries,  % 设置第二组关键字的样式
  % 设置注释
  comment=[l]{\#},        % 以 '#' 开始的行
  morecomment=[s]{/*}{*/}, % 以'/*'开始，以'*/'结束的代码块
  commentstyle=\color{dkgreen}\scriptsize, % 设置注释颜色和斜体
  % 其他
  stringstyle=\color{mauve},           % 设置字符串样式
}
\lstset{
    language=mypython,
    frame=b,                        % 设置边框
    % 设置代码块和边框大小，以及与正文的间距
    % framexleftmargin=-5pt,           % 边框大小（左）
    % framexrightmargin=-1pt,          % 边框大小（右）
    % framextopmargin=-1pt,            % 边框大小（上）
    % framexbottommargin=-1pt,         % 边框大小（下）
    xleftmargin=6pt, xrightmargin=3pt, % 设置代码块的大小（左，右）
    aboveskip=2mm,                     % 与正文的间距（上）
    belowskip=2mm,                     % 与正文的间距（下）
    basicstyle=\fontsize{7pt}{9pt}\ttfamily,  % 设置字体大小、行间距和字体格式
    % 设置行号
    numbers=left,   % 设置行号位置none不显示行号
    numbersep=5pt,  % 设置行号和代码之间的距离
    numberstyle=\scriptsize\color{gray}, % 设置行号样式
    % 其他
    showstringspaces=false,
    columns=flexible,
    breaklines=true,              % 自动换行
    breakatwhitespace=true,
    tabsize=4,                    % 缩进
    extendedchars=false,          % 解决代码跨页时，章节标题，页眉等汉字不显示的问题
    escapeinside={(*@}{@*)}    
}

% % 设置标题格式
% \captionsetup[lstlisting]{
%   labelsep=colon,
%   singlelinecheck=false
% }


\begin{figure}
\centering
\begin{lstlisting}
import random
import torch.nn as nn

class LLM(PreTrainedModel):              # e,g, LlamaModel
    def __init__(self, config):
        ...                    # omit codes in Transformers
        self.layers = nn.ModuleList(  # transformer layers
            [LLMLayer(config, layer_idx) for layer_idx in range(config.num_hidden_layers)]
        )
    
    def forward(self, (*@\footnotesize\textcolor{magenta}{drop\_rates}@*), hidden_states, ...):
        ...
        # for each transformer layer
        for i, layer in enumerate(self.layers):
            # stochastic transformer layer dropout
            (*@\footnotesize\textbf{\textcolor{magenta}{if self}}\textcolor{magenta}{.training:}@*)
                (*@\footnotesize\textcolor{magenta}{drop = random.random()}@*)
                (*@\footnotesize\textbf{\textcolor{magenta}{if}} \textcolor{magenta}{drop < drop\_rates[i]:}@*)
                    (*@\footnotesize\textbf{\textcolor{magenta}{continue}}@*)
                    
            # transformation function of transformer layer
            hidden_states = layer(hidden_states, ...)
            ...
        ...
\end{lstlisting}
\captionof{figure}{Code snippet of stochastic transformer layer dropout built atop Transformers \cite{Transformers}, a famous LLMs library developed by Hugging Face. The codes we inserted into Transformers are marked in \textcolor{magenta}{red}.} \label{code:stochastic_layer_dropout}
\end{figure}


\noindent \textbf{Training efficiency analysis.} In a given batch, the number of layers \emph{activated}, denoted as $\widetilde{L}$, is a random variable. Under the assumption of independent deactivations across layers, the expected number of active layers is:
\begin{equation}
    \mathbb{E}(\widetilde{L}) = \sum_{l=1}^{L}(1-P_{l})
\end{equation}
where $P_l$ is the drop rate for layer $l$.
Thus, rather than consistently training all \(L\) layers, we train a subnetwork with an average number of $\mathbb{E}(\widetilde{L})$ layers for each batch. This reduced model depth directly cuts down not only the chain of the forward pass but also gradient computations of the backward pass. 
% computation chains of both the forward and backward passes.
% chain and the backward pass computations required for gradient updates. 
% with stochastic depth, we train a language model with an average number of $\mathbb{E}(\widetilde{L})$ layers for each batch. 
% Shortening the depth during training reduces not only the chain of the forward pass but also gradient computations of the backward pass. 
Consequently, training with stochastic layer dropout can reduce the training overhead by $[L - \mathbb{E}(\widetilde{L})] / L$, compared to standard fine-tuning with all layers active (\ie, full fine-tuning). The practical experimental results are consistent with this analysis (see \S\ref{}).


% \noindent \textbf{Trade-off between training efficiency and model performance.} In a given batch, the number of layers \emph{activated}, denoted as $\widetilde{L}$, is a random variable. Under the assumption of independent deactivations across layers, the expected number of active layers is:
% \begin{equation}
%     \mathbb{E}(\widetilde{L}) = \sum_{l=1}^{L}(1-P_{l})
% \end{equation}
% where $P_l$ is the drop rate for layer $l$.
% Thus, rather than consistently training all \(L\) layers, we train a subnetwork with an average number of $\mathbb{E}(\widetilde{L})$ layers for each batch. This reduced model depth directly cuts down not only the chain of the forward pass but also gradient computations of the backward pass. 
% % computation chains of both the forward and backward passes.
% % chain and the backward pass computations required for gradient updates. 
% % with stochastic depth, we train a language model with an average number of $\mathbb{E}(\widetilde{L})$ layers for each batch. 
% % Shortening the depth during training reduces not only the chain of the forward pass but also gradient computations of the backward pass. 
% Consequently, training with stochastic layer dropout can reduce the training overhead by $[L - \mathbb{E}(\widetilde{L})] / L$, compared to standard fine-tuning with all layers active (\ie, full fine-tuning).
% % the training overhead (\eg, training time and memory) can be reduced proportionally by $[L - \mathbb{E}(\widetilde{L})] / L$ compared to that of standard fine-tuning with all layers active.
% While higher drop rates further diminish training costs, they also introduce a risk of degrading the model performance.
% % Therefore, the drop rate configuration is critical for the training performance. $P=\{P_1, P_2, \dots, P_L\}$ for all $L$ layers are critical configurations for the training procedure.
% % However, deactivating too many layers will result in inferior model accuracy. 
% To explore this trade-off, 
% % between the training efficiency
% % and model performance, 
% we fine-tune GPT-2 and LlaMA 2-7B with the ONTONOTES dataset under various drop rate configurations. As shown in Figure~\ref{fig:trade-off-acc-time}, when the drop rates increase, the training overhead decreases nearly linearly. Notably, the accuracy remains relatively stable for moderately increased drop rates (\eg, from 0.1 to 0.4). However, when the drop rate exceeds a certain threshold (\eg, from 0.6 to 0.7), a more substantial decline in accuracy is observed.
% % but it exhibits a larger decline once the drop rates become sufficiently large (\eg, from 0.6 to 0.7).
% % significantly reduces the cost of model training, it also introduces the model accuracy loss. More specifically, the savings in training overhead vary linearly with the increase in drop rates, while the accuracy loss shows a trend of being flat-to-steep.

% \begin{figure}[t]\centering
%     \begin{minipage}[t]{0.495\linewidth}\centering
%         \subfigure[GPT-2.]{\centering
%                 \label{fig:}
%                 \includegraphics[width=1.0\linewidth]{content/picture/design_chapter/tradeoff-time-acc.pdf}
%             }
%     \end{minipage}
%     \begin{minipage}[t]{0.495\linewidth}\centering
%         \subfigure[LLaMA 2-7B.]{\centering
%                 \label{fig:}
%                 \includegraphics[width=1.0\linewidth]{content/picture/design_chapter/tradeoff-time-acc.pdf}
%             }
%     \end{minipage}
%     \caption{Trade-off between efficiency and accuracy under various layer dropout configurations. Communication rounds: 100; number of devices: 10 out of 100 for each round; non-IID setting: $Dir(1.0)$.}\label{fig:trade-off-acc-time}
% \end{figure}


% To achieve the optimal trade-off between model performance and training efficiency, it is crucial to determine the appropriate drop rate configurations for devices. In this work, 
% % to speed up federated NLP training while achieving a higher final model performance, 
% we adopt a widely-used metric, \ie, time-to-accuracy \cite{lai2021oort, li2022pyramidfl, cai2023efficient}, which indicates the wall clock time for training a model to reach a target accuracy, as our key performance objective. 
% % This metric provides a more practical perspective than evaluating either model performance or training time alone. Unlike single-dimensional metrics, time-to-accuracy inherently captures both factors by revealing how quickly the model accuracy improves over elapsed time.
% This metric provides a more comprehensive view of the trade-offs than evaluating model performance or training time independently, as such single-dimensional metrics overemphasize one dimension at the expense of the other. 
% In contrast, time-to-accuracy inherently captures the interplay between both factors by revealing how quickly the model accuracy improves over time.
% To enhance time-to-accuracy performance, we propose an \emph{online configurator} that dynamically adjusts the drop rates throughout the federated training process by employing an exploration-exploitation strategy.
% % targeting the highest gain in accuracy per unit time. 
% Specifically, in each communication round, the configurator samples different drop-rate assignments for devices and monitors the resulting improvements in model accuracy versus elapsed time. Based on these observations, it steers future assignments that yield favorable accuracy improvements more quickly. We elaborate on the detailed decision-making mechanism of the configurator in \S \ref{}, explaining how it adjusts per-device drop rates in an online manner and how these adjustments accumulate to yield optimal time-to-accuracy results.

\begin{figure}[t]\centering
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[GPU memory footprint.]{\centering
                \label{fig:}
                \includegraphics[width=1.0\linewidth]{content/picture/design_chapter/PEFT-STLD.pdf}
            }
    \end{minipage}
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[Training time for 100 batches.]{\centering
                \label{fig:}
                \includegraphics[width=1.0\linewidth]{content/picture/design_chapter/PEFT-STLD.pdf}
            }
    \end{minipage}
    \caption{On-device training overheads for fine-tuning GPT-2 on ONTONOTES. Full FT denotes full fine-tuning. PEFT + STLD denotes integration of stochastic transformer layer dropout (drop rate is 0.5) with PEFT (\eg, LoRA and Adapter).}\label{fig:}
\end{figure}

\subsubsection{Configurator for Drop Rates}\label{sec:configurator}
A unique concern raised by stochastic transformer layer dropout is its sensitivity to the configurations regarding the layer drop rates. To illustrate this, we fine-tune GPT-2 with the ONTONOTES dataset under various drop rate configurations. As shown in Figure~\ref{fig:impact-average-drop-rate}, while the higher drop rate (\ie, lower $\mathbb{E}(\widetilde{L})$) diminishes training costs, it also introduces a risk of degrading the model performance. Besides, for the specific drop rate degree, different distributions of drop rates cross layers (\ie, $\{P_1, P_2, \dots, P_L\}$) also result in various model accuracies (Figure \ref{fig:impact-drop-rate-distribution}). Therefore, choosing an optimal drop rate configuration for each device towards high training efficiency and good model performance is critical. Next, % we build an online configurator that automatically adjusts the drop rate configurations throughout the life cycle of federated NLP. 
we build a configurator for the drop rate configurations.
To better guide the configurator to determine proper drop rates, 
% to speed up federated NLP training while achieving a higher final model performance, 
we adopt a widely-used metric, \ie, time-to-accuracy \cite{lai2021oort, li2022pyramidfl, cai2023efficient}, which indicates the wall clock time for training a model to reach a target accuracy, as the key performance objective. 
% This metric provides a more comprehensive view of the trade-offs than evaluating model performance or training time independently, as such single-dimensional metrics overemphasize one dimension at the expense of the other. 
This metric captures the interplay between training efficiency and model performance by revealing how quickly the model accuracy improves over time. 


\begin{figure}[t]\centering
    \begin{minipage}[t]{0.5\linewidth}\centering
        \subfigure[Impact of the drop rate degree (each layer has the same drop rate).]{\centering
                \label{fig:impact-average-drop-rate}
                \includegraphics[width=0.99\linewidth]{content/picture/design_chapter/tradeoff-time-acc.pdf}
            }
    \end{minipage}
    \begin{minipage}[t]{0.49\linewidth}\centering
        \subfigure[Impact of the drop rate distribution across layers (the average drop rate is 0.5).]{\centering
                \label{fig:impact-drop-rate-distribution}
                \includegraphics[width=0.835\linewidth]{content/picture/design_chapter/drop_rate_distribution.pdf}
            }
    \end{minipage}
    \caption{Training performance under various layer dropout configurations. Communication rounds: 100; number of devices: 10 out of 100 for each round; non-IID setting: $Dir(1.0)$. In Figure \ref{fig:impact-drop-rate-distribution}, the \emph{uniform} distribution sets $P_l=0.5$ uniformly for each layer $l$; the \emph{decay} distribution sets $P_l=1-\frac{l}{L+1}$; the \emph{incremental} distribution sets $P_l=\frac{l}{L+1}$; the normal distribution sets $P_l\sim N(0.5, 0.1)$.}\label{fig:}
\end{figure}

\noindent \textbf{Challenges for the configuration.} Choosing
an optimal configuration towards fast convergence is fundamentally challenging due to the large configuration space. First, the drop rate is a continuous variable ranging from 0 to 1. Consequently, the number of candidate drop rates is infinite. Besides, various configurations are required to adapt to the heterogeneous computing resources of different devices. Another dimension of design space is
that the optimal configuration can be switched across FL
rounds during a training session. Figure \ref{fig:accuracy_speed} elaborates how
such switching is important for achieving the highest gain in
model accuracy during training. Therefore, making a decision offline is inadequate for good time-to-accuracy performance.
\begin{figure}[t]\centering
    \includegraphics[width=0.7\linewidth]{content/picture/design_chapter/acc_speed.pdf}
    \caption{Speeds of the accuracy gains across multiple training rounds under different drop rate configurations. Model and dataset: GPT-2 with ONTONOTES; number of devices: 10 out of 100 for each round; non-IID setting: $Dir(1.0)$.}\label{fig:accuracy_speed}
\end{figure}


\noindent \textbf{Online exploration-exploitation of configurations.} To tackle these challenges, we develop an online exploration-exploitation strategy for effectively configurating the drop rate (Algorithm \ref{alg:configurator}). This strategy balances exploration (trying new drop rate configurations) (Line \ref{line:explor_start}-\ref{line:explor_end}) with exploitation (leveraging historically successful drop rates) (Line \ref{line:exploi_start}-\ref{line:exploi_end}) to converge on near-optimal time-to-accuracy outcomes. 
% Specifically, in each communication round, the configurator samples different drop-rate assignments for devices and monitors the resulting improvements in model accuracy versus elapsed time. Based on these observations, it steers future assignments that yield favorable accuracy improvements more quickly. 
This process can be modeled as a multi-armed bandit problem, where each configuration is an “arm”
of the bandit, and the accuracy gains per unit time is the “reward”. Next, we adaptively balance the exploration and exploitation of different arms to maximize the long-term rewards, which accumulate to yield high time-to-accuracy performance.




% We elaborate on the detailed decision-making mechanism of the configurator in \S \ref{}, explaining how it adjusts per-device drop rates in an online manner and how these adjustments accumulate to yield optimal time-to-accuracy results.

Consider a federated setting with $N$ participating devices in each round indexed by $i \in \{1, \dots, N\}$. At the beginning of each round, the server selects a drop-rate vector $\mathbf{P}_i = \{P_{i,1}, \dots, P_{i,L}\}$ for each participating device $i$, where $L$ is the number of transformer layers in the model. Then, each device trains locally with its assigned drop rates for a local epoch (with multiple batch steps) and returns model updates to the server (Line \ref{line:training1}, \ref{line:training2} and \ref{line:training_start}-\ref{line:training_end}). The trained model's accuracy $A_i$ is evaluated locally on the local validation set and the wall-clock time $T_i$ for the round is measured by combining device training and communication time.
We define the reward $R(\mathbf{P}_i)$ for device $i$ based on the accuracy gain $\Delta A_i$ per unit time:
\begin{equation}
    R(\mathbf{P}_i) = \frac{\Delta A_i}{ T_i}
\end{equation}
The algorithm's goal is to find drop-rate configurations that maximize this accuracy-improvement-per-time slice for each device, thereby minimizing the time-to-accuracy. For unseen drop rates, the configurator randomly explore potential configurations that had not been selected before (Line \ref{line:random_start}-\ref{line:random_end}). Meanwhile, the configurator narrows down the decision space by exploiting the high-reward explored drop rates (Line \ref{line:narrow_start}-\ref{line:narrow_end}, \ref{line:narrow}).
% For the explored configurations, the configurator narrows down the decision space by exploiting the high-reward drop rates (Line xx-xx). Meanwhile, the configurator explores potential participants that had not been selected before (Line xx-xx). 
To avoid catastrophic accuracy collapse, drop rates may be capped below a maximum threshold (e.g., $P_l \leq 0.6$ in our system). The exploration-exploitation strategy adapts as the global model evolves, letting the algorithm quickly discard underperforming (Line \ref{line:narrow_end}) and overly staled (Line \ref{line:stale}) drop-rate configurations.
% In each round, the probability of exploiting the configuration is $\epsilon\in[0, 1]$, while the probability of drop rate exploration is $1-\epsilon$.

% fraction of participants to explore potential participants that
% had not been selected before (Line 16), which turns to full
% exploration as e!1.

\begin{algorithm}[t]
\footnotesize
\caption{Online Configurator for Drop Rates}\label{alg:configurator}
\SetAlgoNoEnd
\KwIn{Target accuracy $Acc_t$; Exploration interval $explor\_r$ (\eg, 5); Exploration rate $\epsilon\in [0, 1]$;
Start-up configuration list $list$; Number of candidate configurations $n$; Configuration window size $size_w$.}

\SetKwFunction{fclient}{ClientTraining}
\SetKwFunction{fserver}{ServerController}
\SetKwProg{Fn}{Function}{:}{}


{\color[RGB]{148,0,211}\scriptsize{\tcc{Initialize configurations.}}}
Candidate configurations $list_{c} \leftarrow list$\; 
Historical configurations $list_h \leftarrow \emptyset$\;

$is\_explore \leftarrow True$\;

\While{$\frac{1}{N} \sum_i^N A_i < Acc_t$}{

    {\color[RGB]{148,0,211}\scriptsize{\tcc{Explorations of configurations.}}}
    \eIf{$is\_explore$ is $True$}{ \label{line:explor_start}
    
        Randomly generate $(n\cdot \epsilon)$ configurations $list_{e}$\;\label{line:random_start}
        
        $list_{c} \leftarrow list_{c} \cup list_{e}$\; \label{line:random_end}
        
        \For{each configuration $\{\mathbf{P}_i\}_{i=i}^{N}$ in $list_{c}$}{
             \fclient{$\{\mathbf{P}_i\}_{i=i}^{N}$}\; \label{line:training1}
             Aggregate received local model updates\;
        }
        $list_{h} \leftarrow list_{h} \cup list_{c}$\;
        $list_{h} \leftarrow$ Latest $size_w$ configurations in $list_{h}$\; \label{line:stale}
        % Compute rewards for configurations in $list_{c}$\;
        Update rewards for configurations in $list_{h}$\; \label{line:narrow_start}
        
        
        $list_{c} \leftarrow$ Configurations in $list_{h}$ with top-$(n\cdot(1-\epsilon))$ rewards\; \label{line:narrow_end}
        
        $is\_explore \leftarrow False$\; \label{line:explor_end}
    }
    {{\color[RGB]{148,0,211}\scriptsize{\tcc{Exploitations of configurations.}}}
        Exploitation round $r \leftarrow 0$\;\label{line:exploi_start}
        $\mathbf{P}_{win} \leftarrow$ Configuration in $list_{h}$ with highest reward\; \label{line:narrow}
        \While{$r < explor\_r$}{
            \fclient{$\mathbf{P}_{win}$}; $r++$\; \label{line:training2}
            Aggregate received local model updates\;
        }
        
        $is\_explore \leftarrow True$\;\label{line:exploi_end}
    }
}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\fclient{$\mathbf{P}$}}{ \label{line:training_start}
    \For{each device $i = 1$ to $N$ \textbf{in parallel}}{
        Send $\mathbf{P}_i \in \mathbf{P}$ to participating device $i$\;
        Train locally by stochastic layer dropout using $\mathbf{P}_i$\;
        Upload local model updates to server\; \label{line:training_end}
    }
}

\end{algorithm}

% \vspace{-6pt}



\noindent \textbf{Further narrowing the decision space.} For practical implementation, one can discretize the per-layer drop rates into a finite set (e.g., $\{0.0, 0.1, 0.2, \dots, 0.9\}$). This yields a finite action space for each layer on each device. Though the approach can be extended to continuous drop rates, discrete sets are common in online optimization to simplify exploration. Besides, a good drop rate distribution across layers can be preset through experience or pre-experiment. We consider several different drop rate distributions, \ie, the uniform, decay, incremental and normal distributions. In practice, we observe that the decay distribution works surprisingly well across many models and datasets. To explore the reason, we perform an in-depth analysis on the hidden values $H_l$ of each layer $l$ in the model. As shown in Figure \ref{}, xxx. This analysis reveals that early layers in LLMs play a dominant role in converting inputs into outputs, \ie, larger $\Delta H_{(l-1, l)}$. Notably, skipping one of these early layers can cause significantly distorted outputs, reducing the model performance to near random guessing \cite{chen2024llama, yu2024edge}. In contrast, skipping other layers typically results in only marginal performance degradation \cite{zhang2024investigating}.

% (from round $r-1$ to round $r$) per unit time $T_i^{(r)}$. The algorithm's goal is to find drop-rate configurations that maximize this accuracy-improvement-per-time slice, thereby minimizing the time-to-accuracy. For practical implementation, one can discretize the per-layer drop rates into a finite set (e.g., $\{0.0, 0.1, 0.2, \dots\}, 0.9$). This yields a finite action space for each layer on each device. Though the approach can be extended to continuous drop rates, discrete sets are common in online optimization to simplify exploration. Besides, a good drop rate distribution across layers can be preset through experience or pre experiment to further reduce the decision space of configuration

% \paragraph{Algorithmic Core: Multi-Armed Bandit for Each Device.}
% We treat each device's \emph{drop-rate configuration} (i.e., the collection of layer-wise drop rates) as an \emph{arm} in a multi-armed bandit (MAB) framework. If every device has $K_i$ possible configurations (e.g., combinations or single-layer drop choices), the server faces an MAB with $K_i$ arms per device. At each round, the server chooses one drop-rate configuration $\mathbf{P}_i^{(r)}$ for each device $i$. 
% The \emph{reward} observed is:
% \[
%     R^{(r)}(\mathbf{P}_1^{(r)}, \dots, \mathbf{P}_N^{(r)}) \;\;=\;\; \frac{\Delta A^{(r)}}{T^{(r)}}.
% \]
% Below is a step-by-step pseudocode for an \textbf{online drop-rate configurator} that blends MAB exploration-exploitation with federated training.


% \begin{algorithm}
% \footnotesize
% \caption{Online Configurator for Layer Drop Rates}
% \begin{algorithmic}[1]
% % \Require Number of devices $N$; discrete set of configurations $\{\mathbf{p}_{i,1}, \dots, \mathbf{p}_{i,K_i}\}$ for each device $i$; MAB hyperparameters (exploration rate, etc.); maximum rounds $R$.
% \Require Target accuracy $t\_acc$; Exploration interval $explor\_r$; 
% % Exploitation round $exploit\_r$;
% Start-up configuration list $list$; Number of candidate configurations $n$.
% % Bandit policy $\pi_i$ for each device $i$, e.g., using 
% % Upper Confidence Bound (UCB) or 
% % Thompson Sampling; An empty log $Z$ to record each history reward $R(\mathbf{P}_i^{(k)})$.
% % \State \textbf{Initialize:} model $M^{(0)}$ randomly or from a pre-trained checkpoint.
% % \State \textbf{Initialize} an empty log $Z$ to record $\Delta A^{(r)}/T^{(r)}$ each round.

% \State $explor\_list \leftarrow list$; $is\_explore \leftarrow True$.
% \While{$\frac{1}{N} \sum_i^N A_i < t\_acc$}
%     \If{$is\_explore$ is $True$}
%         \For{each configuration $\{\mathbf{P}_i\}_{i=i}^{N}$ in $explor\_list$}
%              \State \Call{ClientTraining}{$\{\mathbf{P}_i\}_{i=i}^{N}$}.
%         \EndFor
%         \State Compute rewards for configurations in $explor\_list$.
%         \State Update reward for historical configurations.
%         \State $\mathbf{P}_{win}, list_{candi.} \leftarrow$ Configurations with highest and top-$n$ rewards.
%         \State $is\_explore \leftarrow False$.
%     \Else
%         \State Exploitation round $k \leftarrow 0$
%         \While{$k < explor\_r$}
%             \State \Call{ClientTraining}{$\{\mathbf{P}_{win}$}; $k++$.
%         \EndWhile
%         \State $is\_explore \leftarrow True$.
%     \EndIf
%     \State Aggregate received local model updates from devices.
% \EndWhile
%     % \State $\mathbf{P}_i^{(r)} \gets \pi_i(Z, \epsilon)$ \Comment{Select drop-rate configuration via MAB policy.}
% \Function{ClientTraining}{$\mathbf{P}$}:
%     \For{each device $i = 1$ to $N$ \textbf{in parallel}}
%         \State Broadcast $\mathbf{P}_i \in \mathbf{P}$ and to participating device $i$.
%         \State Train locally by stochastic layer dropout using $\mathbf{P}_i$.
%         \State Upload local model updates to server.
%     \EndFor
% \EndFunction
%     % \EndFor
%     % \State \textbf{Broadcast} $M^{(r-1)}$ and $\{\mathbf{P}_i^{(r)}\}_{i=1}^N$ to all devices.
%     % \For{each device $i = 1$ to $N$ \textbf{in parallel}}
%     %     \State \textbf{Train locally} using the assigned drop-rate $\mathbf{P}_i^{(r)}$ for local epochs or steps.
%     %     \State \textbf{Upload local model updates} to server.
%     % \EndFor
% %     \State \textbf{Aggregate} updates to form new global model $M^{(r)}$.
% %     \State Evaluate $M^{(r)}$ to get validation accuracy $A^{(r)}$.
% %     \State Calculate $\Delta A^{(r)} = A^{(r)} - A^{(r-1)}$ and measure total time $T^{(r)}$.
% %     \State \textbf{Compute reward} $R^{(r)} = \Delta A^{(r)}/T^{(r)}$.
% %     \For{each device $i = 1$ to $N$}
% %         \State \textbf{Update bandit feedback} for $\pi_i$ based on $R^{(r)}$.
% %     \EndFor
% %     \State \textbf{Log} $R^{(r)}$ into $Z$.
% % \EndFor
% % \State \textbf{Return} the best global model $M^{(R)}$ and the final drop-rate configurations.
% \end{algorithmic}
% \end{algorithm}

% \paragraph{Computational Complexity.}
% Each device only trains one drop-rate configuration per round, so the overhead for exploration remains manageable. The aggregator updates the MAB policy using the \emph{global} reward $R^{(r)}$, which captures the global time-to-accuracy improvement. A more advanced approach could incorporate device-specific rewards (e.g., local $\Delta A_i^{(r)}/T_i^{(r)}$), enabling fine-grained scheduling in heterogeneous environments.

% \paragraph{Practical Considerations.}
% \begin{itemize}
%     % \item \textbf{Heterogeneity:} Different devices vary in computational speed, network bandwidth, and data distribution. The algorithm can incorporate device-specific time measurements $T_i^{(r)}$ to refine local rewards. 
%     % \item \textbf{Drop-Rate Bounds:} To avoid catastrophic accuracy collapse, drop rates may be capped below a maximum threshold (e.g., $P_l \leq 0.5$).
%     % \item \textbf{Scheduling Frequency:} The configurator can update drop rates every round or every few rounds. In practice, adjusting too frequently may cause instability, while updating too infrequently may limit adaptability.
%     % \item \textbf{Adaptive Discretization:} One could dynamically refine the drop-rate search space based on performance feedback (e.g., splitting intervals around promising configurations).
% \end{itemize}

% \paragraph{Algorithm Advantages.}
% \begin{enumerate}
%     \item \textbf{Minimal Overhead:} Exploration occurs by simply assigning different drop rates; no specialized computation or kernels are required.
%     \item \textbf{Robustness to Dynamics:} The MAB policy adapts as the global model evolves, letting the algorithm quickly discard underperforming drop-rate configurations.
%     \item \textbf{Scalability:} The same policy structure can scale to large federated networks, where each device may have different hardware capabilities and network constraints.
% \end{enumerate}

% \paragraph{Optimality and Convergence.}
% Under mild assumptions (e.g., bounded rewards and sub-Gaussian reward distributions), MAB algorithms with exploration-exploitation strategies enjoy theoretical regret bounds. Though the global time-to-accuracy objective here is more complex than a conventional single-agent bandit, the general principle still applies: repeated exploration of viable configurations gradually identifies (near-)optimal drop rates for each device’s local environment, improving the collective time-to-accuracy.


% \subsection{Selection and Analysis of Multi-Armed Bandit (MAB) Policies}
% \label{sec:mab_selection}

% In designing an online algorithm for optimal drop-rate assignment, the choice of Multi-Armed Bandit (MAB) policy is pivotal. Different MAB policies offer varying balances between exploration and exploitation, adaptability to non-stationary environments, and computational efficiency. This section analyzes several prominent MAB policies, evaluates their suitability for our federated NLP setting, and delineates the process of selecting drop-rate configurations using the chosen policy.

% \subsubsection{Overview of MAB Policies}

% \paragraph{1. $\epsilon$-Greedy}
% The $\epsilon$-Greedy algorithm selects the best-known action (exploitation) with probability $1-\epsilon$ and explores a random action with probability $\epsilon$. While simple and easy to implement, it treats all exploratory actions uniformly, which can lead to inefficient exploration, especially in large action spaces.

% \paragraph{2. Upper Confidence Bound (UCB)}
% UCB algorithms select actions based on both their estimated rewards and the uncertainty or variance in those estimates. Specifically, they choose the action with the highest upper confidence bound, balancing exploration and exploitation by favoring actions with higher uncertainty.

% \paragraph{3. Thompson Sampling (TS)}
% Thompson Sampling maintains a probability distribution over each action's potential rewards and samples from these distributions to select actions. This probabilistic approach naturally balances exploration and exploitation and has been empirically shown to perform well in various settings.

% \paragraph{4. EXP3 (Exponential-weight algorithm for Exploration and Exploitation)}
% EXP3 is designed for adversarial settings where rewards are not stochastic but can be chosen by an adversary. It assigns weights to actions based on their past performance and uses these weights to probabilistically select actions, ensuring no single action is overly favored without sufficient evidence.

% \paragraph{5. Sliding-Window UCB and Discounted UCB}
% These variants of UCB are tailored for non-stationary environments by giving more weight to recent observations. They maintain a sliding window of recent rewards or apply a discount factor to older rewards, allowing the algorithm to adapt to changes over time.

% \subsubsection{Policy Evaluation and Selection}

% Given the federated NLP context, several factors influence the suitability of an MAB policy:

% \begin{itemize}
%     \item \textbf{Non-Stationarity:} The global model evolves over time, potentially altering the effectiveness of specific drop-rate configurations.
%     \item \textbf{Scalability:** Each device may have a different set of possible drop-rate configurations, necessitating efficient handling of large action spaces.
%     \item \textbf{Communication Overhead:** Minimizing additional communication for policy updates is crucial in federated settings.
%     \item \textbf{Computational Efficiency:** The policy should incur minimal computational overhead on the server and devices.
% \end{itemize}

% \paragraph{Recommendation: Thompson Sampling with Contextual Adaptation}

% After evaluating the aforementioned policies, \textbf{Thompson Sampling (TS)} emerges as the most suitable choice for our scenario due to the following reasons:

% \begin{enumerate}
%     \item \textbf{Effective Exploration-Exploitation Balance:} TS naturally balances exploration and exploitation by sampling from the posterior distributions of action rewards.
%     \item \textbf{Adaptability to Non-Stationarity:} By periodically updating the posterior distributions, TS can adapt to changes in the environment, such as evolving model dynamics during training.
%     \item \textbf{Scalability:** TS can efficiently handle large and possibly heterogeneous action spaces, especially when combined with contextual information.
%     \item \textbf{Empirical Performance:** TS has been empirically validated to perform well in various federated and distributed settings.
% \end{enumerate}

% \subsubsection{Detailed Drop-Rate Configuration Process}

% Leveraging Thompson Sampling, the online configurator operates as follows to determine optimal drop-rate configurations for each device in every training round.

% \paragraph{1. Initialization}
% For each device \( i \in \{1, \dots, N\} \) and each possible drop-rate configuration \( \mathbf{p}_{i,k} \) where \( k \in \{1, \dots, K_i\} \), initialize prior distributions for the expected reward \( R_{i,k} \). Typically, a Beta distribution \( \text{Beta}(\alpha_{i,k}, \beta_{i,k}) \) is used for binary rewards or Gaussian distributions \( \mathcal{N}(\mu_{i,k}, \sigma_{i,k}^2) \) for continuous rewards.

% \paragraph{2. Action Selection via Thompson Sampling}
% For each device \( i \) in round \( r \):

% \begin{enumerate}
%     \item **Sample Reward Estimates:** Draw a sample \( \theta_{i,k} \) from the posterior distribution of each drop-rate configuration \( \mathbf{p}_{i,k} \).
%     \[
%         \theta_{i,k} \sim \text{Posterior}(R_{i,k})
%     \]
%     \item **Select Configuration:** Choose the drop-rate configuration \( \mathbf{p}_{i,k^*} \) with the highest sampled reward.
%     \[
%         k^* = \arg\max_{k} \theta_{i,k}
%     \]
%     \item **Assign Drop Rates:** Set \( \mathbf{P}_i^{(r)} = \mathbf{p}_{i,k^*} \) as the drop-rate vector for device \( i \) in round \( r \).
% \end{enumerate}

% \paragraph{3. Local Training and Reward Observation}
% Each device \( i \) performs local training using the assigned drop-rate configuration \( \mathbf{P}_i^{(r)} \) and uploads the model updates to the server. Upon aggregation, the server evaluates the global model's performance, obtaining the reward \( R^{(r)} \) defined as:
% \[
%     R^{(r)} = \frac{\Delta A^{(r)}}{T^{(r)}}
% \]
% where \( \Delta A^{(r)} \) is the improvement in validation accuracy and \( T^{(r)} \) is the wall-clock time for round \( r \).

% \paragraph{4. Posterior Update}
% For each device \( i \), update the posterior distribution of the selected drop-rate configuration \( \mathbf{p}_{i,k^*} \) based on the observed reward \( R^{(r)} \):

% \begin{itemize}
%     \item **Beta-Bernoulli Model:** If using a Beta distribution for binary rewards:
%     \[
%         \alpha_{i,k^*} \leftarrow \alpha_{i,k^*} + R^{(r)}
%     \]
%     \[
%         \beta_{i,k^*} \leftarrow \beta_{i,k^*} + (1 - R^{(r)})
%     \]
    
%     \item **Gaussian Model:** If using a Gaussian distribution for continuous rewards:
%     \[
%         \mu_{i,k^*} \leftarrow \text{Update}(\mu_{i,k^*}, R^{(r)})
%     \]
%     \[
%         \sigma_{i,k^*}^2 \leftarrow \text{Update}(\sigma_{i,k^*}^2, R^{(r)})
%     \]
% \end{itemize}

% \paragraph{5. Iterative Refinement}
% Repeat steps 2-4 for each round \( r \in \{1, \dots, R\} \), allowing the algorithm to continuously refine the drop-rate configurations based on observed rewards.

% \subsubsection{Handling Heterogeneous Devices}

% In federated settings, devices may vary in computational capabilities, network bandwidth, and local data distributions. To accommodate this heterogeneity, the algorithm incorporates the following strategies:

% \paragraph{Per-Device Reward Normalization}
% Normalize rewards \( R^{(r)} \) on a per-device basis to account for varying device speeds and data qualities. This ensures that the reward signal accurately reflects each device's contribution to the global time-to-accuracy objective.

% \paragraph{Adaptive Configuration Sets}
% Allow each device \( i \) to have a customized set of drop-rate configurations \( \{\mathbf{p}_{i,1}, \dots, \mathbf{p}_{i,K_i}\} \) tailored to its specific constraints and capabilities. This flexibility enables the algorithm to assign more aggressive drop rates to devices with higher computational resources, while assigning conservative drop rates to resource-constrained devices.

% \paragraph{Asynchronous Updates}
% Implement asynchronous communication protocols where devices can operate and update their configurations independently, mitigating the impact of stragglers and ensuring efficient utilization of all participating devices.

% \subsubsection{Algorithmic Pseudocode}

% The following pseudocode outlines the Thompson Sampling-based drop-rate configurator integrated into the federated training process.

% \begin{figure}[t]
% \begin{center}
% \begin{minipage}{0.98\linewidth}
% \begin{algorithmic}[1]
% \Require Number of devices $N$; discrete drop-rate configurations $\{\mathbf{p}_{i,1}, \dots, \mathbf{p}_{i,K_i}\}$ for each device $i$; MAB hyperparameters; maximum rounds $R$.
% \State \textbf{Initialize} posterior parameters for each device and configuration:
% \For{each device $i = 1$ to $N$}
%     \For{each configuration $k = 1$ to $K_i$}
%         \State Initialize $\alpha_{i,k} = 1$, $\beta_{i,k} = 1$ \Comment{For Beta prior}
%         % \State Initialize $\mu_{i,k} = 0$, $\sigma_{i,k}^2 = 1$ \Comment{For Gaussian prior, if applicable}
%     \EndFor
% \EndFor
% \State \textbf{Initialize} global model $M^{(0)}$.
% \For{round $r = 1$ to $R$}
%     \State \textbf{For each device $i = 1$ to $N$ \textbf{in parallel}:}
%         \For{each device $i = 1$ to $N$}
%             \For{each configuration $k = 1$ to $K_i$}
%                 \State Sample $\theta_{i,k} \sim \text{Beta}(\alpha_{i,k}, \beta_{i,k})$
%                 % \State Sample $\theta_{i,k} \sim \mathcal{N}(\mu_{i,k}, \sigma_{i,k}^2)$
%             \EndFor
%             \State Select configuration $k^* = \arg\max_{k} \theta_{i,k}$
%             \State Assign $\mathbf{P}_i^{(r)} = \mathbf{p}_{i,k^*}$
%         \EndFor
%     \EndFor
%     \State \textbf{Broadcast} $M^{(r-1)}$ and $\{\mathbf{P}_i^{(r)}\}_{i=1}^N$ to all devices.
%     \For{each device $i = 1$ to $N$ \textbf{in parallel}}
%         \State \textbf{Train locally} using $\mathbf{P}_i^{(r)}$.
%         \State \textbf{Upload} local model updates to server.
%     \EndFor
%     \State \textbf{Aggregate} updates to form new global model $M^{(r)}$.
%     \State Evaluate $M^{(r)}$ on validation set to obtain $A^{(r)}$.
%     \State Calculate $\Delta A^{(r)} = A^{(r)} - A^{(r-1)}$ and measure total time $T^{(r)}$.
%     \State Compute global reward $R^{(r)} = \Delta A^{(r)} / T^{(r)}$.
%     \For{each device $i = 1$ to $N$}
%         \State \textbf{Update} posterior for selected configuration $k^*$ based on $R^{(r)}$:
%         \State $\alpha_{i,k^*} \leftarrow \alpha_{i,k^*} + R^{(r)}$
%         \State $\beta_{i,k^*} \leftarrow \beta_{i,k^*} + (1 - R^{(r)})$
%         % \State Update Gaussian parameters if applicable
%     \EndFor
% \EndFor
% \State \textbf{Return} the optimized drop-rate configurations and the final global model $M^{(R)}$.
% \end{algorithmic}
% \end{minipage}
% \caption{Thompson Sampling-Based Online Drop-Rate Configurator for Federated Training.}
% \label{alg:thompson_sampling_configurator}
% \end{center}
% \end{figure}

% \paragraph{Algorithm Explanation}

% \begin{enumerate}
%     \item \textbf{Initialization:} For each device and its possible drop-rate configurations, initialize the parameters of the prior distributions. In this case, a Beta prior with parameters \( \alpha = 1 \) and \( \beta = 1 \) represents a uniform distribution over the interval \([0,1]\).
    
%     \item \textbf{Sampling and Selection:} In each round, for every device, sample a reward estimate \( \theta_{i,k} \) from the posterior distribution of each drop-rate configuration \( \mathbf{p}_{i,k} \). Select the configuration with the highest sampled reward \( k^* \).
    
%     \item \textbf{Local Training:** Assign the selected drop-rate configurations to the respective devices, which then perform local training and upload their updates to the server.
    
%     \item \textbf{Aggregation and Evaluation:** The server aggregates the updates to form the new global model and evaluates its performance to obtain the reward \( R^{(r)} \).
    
%     \item \textbf{Posterior Update:** Update the posterior distributions for the selected configurations based on the observed reward. For the Beta distribution, this involves incrementing \( \alpha \) and \( \beta \) parameters accordingly.
    
%     \item \textbf{Iteration:** Repeat the process for a predefined number of rounds \( R \), continually refining the drop-rate configurations based on cumulative rewards.
% \end{enumerate}

% \paragraph{Advantages of Thompson Sampling in This Context}

% \begin{itemize}
%     \item \textbf{Probabilistic Framework:** TS's probabilistic nature allows for a nuanced exploration of drop-rate configurations, efficiently navigating the trade-off between trying new configurations and exploiting known good ones.
    
%     \item \textbf{Adaptability:** As training progresses and the global model evolves, TS can adapt to changing optimal drop-rate configurations, ensuring sustained performance improvements.
    
%     \item \textbf{Scalability:** TS scales well with the number of devices and configurations, making it suitable for large-scale federated environments.
    
%     \item \textbf{Minimal Overhead:** The computational and communication overhead introduced by TS is negligible compared to the overall federated training process.
% \end{itemize}

% \paragraph{Potential Extensions}

% While Thompson Sampling provides a robust foundation for drop-rate configuration, several extensions can enhance its effectiveness:

% \begin{itemize}
%     \item \textbf{Contextual Thompson Sampling:** Incorporate contextual information, such as device-specific features or current training dynamics, to inform the sampling process.
    
%     \item \textbf{Hierarchical Bandits:** Use a hierarchical approach where configurations are first selected at a higher level (e.g., per device group) before being fine-tuned at the individual device level.
    
%     \item \textbf{Hybrid Policies:** Combine TS with other policies, such as UCB, to leverage their respective strengths in specific scenarios.
% \end{itemize}

% \paragraph{Conclusion}

% The adoption of Thompson Sampling as the MAB policy for online drop-rate configuration offers a principled and effective mechanism to optimize the time-to-accuracy metric in federated NLP. By judiciously balancing exploration and exploitation, and adapting to the non-stationary nature of federated training, TS facilitates the identification of optimal drop-rate settings that enhance training efficiency without compromising model performance.




\subsection{Personalized Transformer Layer Sharing}\label{sec:layer_sharing}
% Through stochastic transformer layer dropout, we can extract shallow sub-networks of any desired depth on demand from one single local model on the client for global sharing among clients.

Traditional federated NLP approaches aggregate model updates from devices to form a single global model. While effective in homogeneous settings, this strategy often fails to generalize well across devices in non-IID scenarios. To address this issue, we propose a personalized layer sharing method based on stochastic layer dropout. This approach enables each device to learn personalized representations for local data while benefiting from shared global knowledge, thereby mitigating the adverse effects of non-IID data.


% capture the unique characteristics of local data distributions in non-IID scenarios. In federated NLP, data distribution across devices is often non-IID, posing a significant challenge for training generalizable and high-performance models. To address this challenge, we propose a personalized layer sharing method based on stochastic layer dropout. This approach enables each device to learn personalized representations for local data while benefiting from shared global knowledge.
% , thereby mitigating the adverse effects of non-IID data distributions.

% \noindent \textbf{Motivation.}
% Traditional federated NLP approaches aggregate model updates from all devices to form a single global model. While effective in homogeneous settings, this strategy often fails to capture the unique characteristics of local data distributions in non-IID scenarios. Personalized federated learning aims to tailor models to individual devices, balancing personalization with the benefits of shared learning. Our proposed method extends stochastic layer dropout to facilitate personalized layer sharing, allowing devices to adaptively share and customize transformer layers based on their local data.

\begin{figure*}
    \centering
    \includegraphics[width=0.95\linewidth]{content/picture/design_chapter/hetero_agg.pdf}
    \caption{An example of heterogeneous layer aggregation on the central server.}
    \label{fig:hete_agg}
\end{figure*}

\noindent \textbf{Method overview.}
Personalized transformer layer sharing allows certain transformer layers to be shared globally across all devices, while other layers are personalized and maintained separately for each device. In this way, all layers in the model are categorized into two types: \emph{Shared layers}, which are common across all devices, capture global language patterns and prevent the model from overfitting to local data; \emph{Personalized layers} are unique to each device, allowing the model to adapt to specific local data distributions. After local training in each communication round, each participating device sends its shared layers to the central server for global aggregation. Then, the server returns the aggregated layers to each device. Finally, the devices assemble the received layers and their personalized layers to produce the entire local models. These steps are repeated for multiple rounds until the average model accuracy across devices reaches a predefined target. By selectively personalizing and sharing layers, devices can capture both global patterns and local nuances inherent in their data. 

% . The server then aggregates these layers from all devices to form updated global layers. Finally, the server returns the global layers to each participating device, and these devices assemble the received layers and their personalized layers to produce full models. These steps are repeated for multiple rounds until the average model accuracy across devices reaches the predefined target. By selectively personalizing layers, devices can capture both global patterns and local nuances inherent in their data. 
% In this method, all layers in the model are categorized into two types:
% \begin{itemize}
%     \item \textbf{Shared Layers:} These layers are common across all devices and capture global language patterns. They also prevent the model from overfitting to local data.
%     \item \textbf{Personalized Layers:} These layers are unique to each device, allowing the model to adapt to specific local data distributions. 
%     % Personalized layers are not dropped during training, ensuring that device-specific knowledge is preserved.
% \end{itemize}
% Let $L$ denote the total number of transformer layers. We define a subset of layers $\mathcal{S}_i \subseteq \{1, 2, \dots, L\}$ as shared layers in device $i$, and the remaining layers $\mathcal{P}_i = \{1, 2, \dots, L\} \setminus \mathcal{S}_i$ as personalized layers.
% During federated training, each device $i$ maintains its model parameters in personalized layers $\{TransforBlock_l\}_{l \in \mathcal{P}_i}$ locally, while uploading parameters in layers $\{TransforBlock_{l}\}_{l \in \mathcal{S}}$ to the central server for global aggregation.

% \noindent \textbf{Training procedure.}
% The training procedure alternates between updating shared and personalized layers. 
% In each communication round, each participating device first applies stochastic transformer layer dropout to train the local model using its own data. After local training, devices send parameters in the shared layers to the central server. The server then aggregates these parameters from all devices to form updated global layers. Finally, the central server returns the global parameters to each participating device, and these devices assemble the received parameters into their local models. These steps are repeated for multiple rounds until the average model accuracy across devices reaches the predefined target.

\noindent \textbf{Layer selection for personalizing and sharing.} Determining which layers to share versus personalize can significantly influence the model performance. Static assignment of shared and personalized layers may not capture the nuanced requirements of diverse local data distributions. Different devices may benefit from personalizing different layers based on their specific data characteristics. Therefore, an adaptive mechanism is crucial to enable the model to tailor its architecture dynamically without manual intervention. To facilitate adaptive layer personalization, it is essential to quantify the importance of each layer with respect to the local datasets. We leverage the "gradient criterion", which says layers with larger gradients during training are more sensitive and thus more critical for capturing unique data patterns. Inspired by this criterion, we utilize gradient magnitudes to assess the importance of each transformer layer for model personalization. Specifically, during local training, we compute the gradient norm $g_l^{(t)}$ of the parameters within each layer $l$ for each training batch $t$.
% To this end, we leverage "gradient criterion", which says data samples inducing larger gradients are often more informative and crucial for the model's learning process. Inspired by this criterion, we utilize gradient magnitudes to assess the sensitivity and importance of each transformer layer during training. Specifically, layers that consistently produce larger gradients when learning local data are deemed more critical for capturing unique and significant patterns inherent to that device's dataset.
% Formally, let \( \theta_l \) denote the parameters of layer \( l \). During local training, we compute the gradient of the loss function \( \mathcal{L}_i \) with respect to each layer's parameters\footnote{This process does not introduce additional overhead, as the gradients need to be calculated during training.}:
% \begin{equation}
%     g_{i,l} = \left\| \nabla_{\theta_l} \mathcal{L}_i \right\|_2,
% \end{equation}
% where \( \left\| \cdot \right\|_2 \) denotes the Euclidean norm, providing a scalar measure of gradient magnitude for layer \( l \) on device \( i \). 
By aggregating these gradient magnitudes over multiple training batches, we derive an importance score $I_l$ for each layer:
\begin{equation}
    % I_l = \frac{1}{T} \sum_{t=1}^{T} g_l^{(t)},
    I_l = \frac{1}{\sum_{t=1}^{T}(1-d_{l}^{(t)})} \sum_{t=1}^{T} g_l^{(t)}(1-d_{l}^{(t)})
\end{equation}
where $T$ is the number of training batches and $d_{l}^{(t)}$ indicates whether layer $l$ is deactivated ($d_{l}^{(t)} = 1$) or activated ($d_{l}^{(t)} = 0$) by stochastic layer dropout in batch $t$.
% indicates whether layer $l$ is activated ($d_{l}^{(t)}=0$) by stochastic layer dropout in batch $t$. 
Higher values of $I_l$ indicate that layer $l$ is more sensitive and thus more critical for learning from the local data. This metric effectively captures the cumulative gradient influence of each layer when it is active, providing a robust measure of its importance. Based on the computed importance scores, each device selects the top-$k$ layers with the highest importance scores to be included in the set of personalized layers. The choice of $k$ (\eg, $k = L/2$) can be based on empirical validation or computational constraints. The remaining $L - k$ layers are assigned to the shared set, which are uploaded to the central server for global aggregation.

\noindent \textbf{Heterogeneous layer aggregation.} Considering the non-IID data distribution across devices, the shared layers may be heterogeneous across devices, \ie, only parts of these layers are overlapped across devices. However, in the conventional federated NLP frameworks, devices share all layers in the model, thus the server can directly perform model aggregation on each layer.
% the local model of each device shares the same architecture, thus the server can directly performs the aggregation on all layers in all local models. 
To handle the heterogeneous shared transformer layers across devices, we design a specific aggregation strategy that performs averaging on only intersections of shared layers, while keeping the remaining non-intersected layers unchanged. % Then, the central server sends the updated global layers back to devices accordingly. 
As Figure \ref{fig:hete_agg} illustrates, the second layers of device $1$, $2$ and $3$ are intersected, and hence the parameter of these layers are averaged respectively. Likewise, the first layer of device $1$ and $2$ are aggregated. Because the third layer of device $1$ is personalized, there is no intersection of the third layer between device $1$ and $2$ (or $3$). Therefore, the third layer of device $1$ will be excluded from global aggregation. Notably, the devices holding similar local data will share similar layer architectures with more overlapped parameters. Therefore, this aggregation method can promote mutual benefits of devices with similar data distributions and reduce the interference between devices with different data distributions. After layer aggregation, the central server sends the updated global layers back to the participating devices accordingly.

% \begin{enumerate}
%     \item \textbf{Initialization:} Initialize shared layers $\{TransforBlock_l\}_{l \in \mathcal{S}}$ globally and personalized layers $\{TransforBlock_{i,l}\}_{l \in \mathcal{P}}$ locally for each device $i$. 
    
%     \item \textbf{Local Training:} For each training round $r$, each device $i$ performs the following steps:
%     \begin{enumerate}
%         \item Apply stochastic layer dropout to shared layers during the forward pass as per Equation~\eqref{eq:personalized_layer_forward}.
%         \item Train the model locally using its own data, updating both shared and personalized layers (only the shared layers are synchronized globally).
%     \end{enumerate}
    
%     \item \textbf{Aggregation:} After local training, devices send updates of the shared layers to the central server. The server aggregates these updates (e.g., via Federated Averaging) to form updated shared layers.
    
%     \item \textbf{Personalized Layer Maintenance:} Personalized layers remain local to each device and are not shared or aggregated.
    
%     \item \textbf{Iteration:} Repeat the local training and aggregation steps for $R$ rounds until convergence.
% \end{enumerate}

% \paragraph{Algorithm Pseudocode.}
% \begin{figure}[t]
% \begin{center}
% \begin{minipage}{0.98\linewidth}
% \begin{algorithmic}[1]
% \Require Number of devices $N$; shared layer indices $\mathcal{S}$; personalized layer indices $\mathcal{P}$; drop rates $P_l$ for $l \in \mathcal{S}$; maximum rounds $R$.
% \State \textbf{Initialize} shared layers $\{TransforBlock_l^{(0)}\}_{l \in \mathcal{S}}$ on the server.
% \For{each device $i = 1$ to $N$}
%     \State \textbf{Initialize} personalized layers $\{TransforBlock_{i,l}^{(0)}\}_{l \in \mathcal{P}}$ locally.
% \EndFor

% \For{$r = 1$ to $R$}
%     \For{each device $i = 1$ to $N$ \textbf{in parallel}}
%         \State \textbf{Download} shared layers $\{TransforBlock_l^{(r-1)}\}_{l \in \mathcal{S}}$ from the server.
%         \State \textbf{Initialize} local model with shared and personalized layers.
%         \For{each local epoch or mini-batch}
%             \For{each shared layer $l \in \mathcal{S}$}
%                 \State Sample $d_l \sim \text{Bernoulli}(P_l)$.
%             \EndFor
%             \State \textbf{Forward pass} using Equation~\eqref{eq:personalized_layer_forward}.
%             \State \textbf{Backward pass} and update parameters.
%         \EndFor
%         \State \textbf{Upload} updated shared layers $\{TransforBlock_l^{(r,i)}\}_{l \in \mathcal{S}}$ to the server.
%     \EndFor
%     \State \textbf{Aggregate} shared layers on the server:
%     \[
%         \TransforBlock_l^{(r)} = \frac{1}{N} \sum_{i=1}^N TransforBlock_l^{(r,i)}, \quad \forall l \in \mathcal{S}.
%     \]
%     \State \textbf{Evaluate} the global model's performance.
% \EndFor
% \State \textbf{Return} the aggregated shared layers and personalized layers for each device.
% \end{algorithmic}
% \end{minipage}
% \caption{Pseudocode for Personalized Transformer Layer Sharing using Stochastic Layer Dropout.}
% \label{alg:personalized_layer_sharing}
% \end{center}
% \end{figure}

\noindent \textbf{Other advantages of personalized layer sharing.} (1) \emph{Communication efficiency:} Since only shared layers are communicated between devices and the server, the method reduces communication overhead compared to approaches that require full model synchronization. (2) \emph{Security and privacy:} Personalized layers remain on-device, enhancing data privacy by ensuring that device-specific information is not transmitted.

\subsection{Integration with PEFT}
Stochastic layer dropout is naturally compatible with PEFT. 
% The integration of these two technologies is straightforward and does not introduce conflicts. 
This is because layer dropout operates at the granularity of transformer layers, whereas PEFT modifies the parameters within each layer without altering the overall model architecture.
% the LoRA method modifies computations of transformer layer $l$ in Equation~\eqref{eq:transformer_layer} as $H_{l+1} = TransforBlock(H_l) + LoRA_l(H_l)$, where $LoRA_l(H_l)$ denotes the function of inserted lower-rank matrices by LoRA within layer $l$. Then, 
In this work, we propose to seamlessly combine stochastic layer dropout with PEFT for better training efficiency by simply updating Equation~\eqref{eq:layer-dropout} as follows:
% . Specifically, the computation for layer $l$ in Equation~\eqref{eq:layer-dropout} is simply updated as follows:
\begin{equation}
\begin{split}
H_{l+1} &= (1-d_l) \cdot [TransforBlock_l(H_l) + \Delta \Theta_l]\\
&+ d_l \cdot Identity(H_l)
\end{split}
\end{equation}
where $\Delta \Theta_l$ denotes the PEFT adjustment (\eg, low-rank adaptation in LoRA) applied to the transformation function of layer $l$. During the backward pass, the parameters in $TransforBlock(\cdot)$ are frozen, and only the added parameters in $\Delta \Theta_l$ are updated. As shown in Figure~\ref{}, the combination of stochastic transformer layer dropout and PEFT create a powerful synergy for optimizing training efficiency. Together, they enable more scalable and efficient model deployments in federated NLP. % where resource constraints are key considerations.


% The integration of these techniques offers significant benefits for model deployment. 


% % and PEFT techniques are compatible and complementary. 
% Although Koto focuses on optimizing stochastic transformer layer dropout for federated NLP, it can be naturally and simply combined with the PEFT techniques to obtain an more efficient deployment. Therefore, they should benefit from each other. 

% \paragraph{Handling Layer Selection and Personalization.}
% Determining which layers to share versus personalize can significantly influence the model's effectiveness. Strategies for layer classification include:
% \begin{itemize}
%     \item \textbf{Fixed Assignment:} Predefine certain layers (e.g., lower or higher layers) as shared or personalized based on empirical studies.
%     \item \textbf{Dynamic Assignment:} Allow the model to learn which layers to personalize based on performance metrics or layer importance scores.
%     \item \textbf{Hybrid Approaches:} Combine fixed and dynamic strategies, where a core set of layers is always shared, and additional layers can be personalized as needed.
% \end{itemize}

% \paragraph{Experimental Validation.}
% To validate the effectiveness of the Personalized Transformer Layer Sharing method, we conduct experiments on federated versions of benchmark NLP datasets with varying degrees of non-IIDness. We compare our method against standard federated learning and other personalized federated learning approaches. Metrics include time-to-accuracy, model accuracy, and computational overhead. Preliminary results demonstrate that our approach achieves superior performance in non-IID settings by effectively balancing shared and personalized knowledge.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{personalized_layer_sharing.pdf}
%     \caption{Illustration of Personalized Transformer Layer Sharing. Shared layers are subject to stochastic dropout, promoting generalization, while personalized layers adapt to local data distributions.}
%     \label{fig:personalized_layer_sharing}
% \end{figure}

% \paragraph{Summary.}
% The Personalized Transformer Layer Sharing method leverages stochastic layer dropout to facilitate a balance between global knowledge sharing and local personalization. By categorizing transformer layers into shared and personalized subsets, devices can effectively learn from both aggregated and local data, addressing the challenges posed by non-IID data distributions in federated NLP. This approach enhances model performance, accelerates training, and maintains scalability, making it a robust solution for real-world federated learning applications.

% \paragraph{Future Work.}
% Future research can explore adaptive strategies for layer classification, investigate the impact of different layer sharing schemes, and extend the method to more complex model architectures. Additionally, integrating advanced personalization techniques, such as meta-learning or federated multi-task learning, could further enhance the adaptability and performance of personalized models in heterogeneous federated environments.
% The Personalized Transformer Layer Sharing method can be extended to multi-task federated learning scenarios, where devices may perform different tasks (e.g., sentiment analysis, translation). In such cases, personalized layers can be further specialized for specific tasks, while shared layers capture task-agnostic representations. This extension enhances the versatility and applicability of the federated model across diverse applications.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{personalized_layer_sharing_flow.pdf}
%     \caption{Flowchart of the Personalized Transformer Layer Sharing method. Shared layers undergo stochastic dropout, while personalized layers remain active to capture local data characteristics.}
%     \label{fig:personalized_layer_sharing_flow}
% \end{figure}

% \paragraph{Implementation Considerations.}
% \begin{itemize}
%     \item \textbf{Communication Efficiency:} Since only shared layers are communicated between devices and the server, the method reduces communication overhead compared to approaches that require full model synchronization.
%     \item \textbf{Security and Privacy:} Personalized layers remain on-device, enhancing data privacy by ensuring that device-specific information is not transmitted.
% \end{itemize}

% \paragraph{Conclusion.}
% Personalized Transformer Layer Sharing based on Stochastic Transformer Layer Dropout offers a novel solution to the non-IID data challenge in federated NLP. By enabling a dynamic balance between shared and personalized model components, it enhances both model performance and training efficiency, paving the way for more effective and scalable federated learning systems.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{personalized_vs_shared_layers.pdf}
%     \caption{Comparison between shared and personalized layers in the proposed method. Shared layers are trained collectively with stochastic dropout, while personalized layers are optimized locally to capture device-specific data distributions.}
%     \label{fig:shared_vs_personalized}
% \end{figure}

% \paragraph{Mathematical Formulation of Personalized Layer Updates.}
% To formalize the update rules for shared and personalized layers, consider the following optimization objectives:

% \begin{align}
%     \text{For shared layers:} \quad & \min_{\{TransforBlock_l\}_{l \in \mathcal{S}}} \sum_{i=1}^N \mathcal{L}_i(M_{\mathcal{S}, \mathcal{P}_i}^{(r)}, D_i), \\
%     \text{For personalized layers:} \quad & \min_{\{TransforBlock_{i,l}\}_{l \in \mathcal{P}}} \mathcal{L}_i(M_{\mathcal{S}, \mathcal{P}_i}^{(r)}, D_i),
% \end{align}
% where:
% \begin{itemize}
%     \item $\mathcal{L}_i$ denotes the loss function for device $i$.
%     \item $M_{\mathcal{S}, \mathcal{P}_i}^{(r)}$ represents the model at round $r$ with shared layers $\mathcal{S}$ and personalized layers $\mathcal{P}_i$ for device $i$.
%     \item $D_i$ denotes the local dataset for device $i$.
% \end{itemize}

% The optimization ensures that shared layers learn generalized representations across all devices, while personalized layers fine-tune the model to local data specifics.

% \paragraph{Integration with Federated Optimization Algorithms.}
% Our method is compatible with various federated optimization algorithms, such as Federated Averaging (FedAvg) or more advanced variants like FedProx and Scaffold. The choice of optimization algorithm can influence convergence rates and robustness to client heterogeneity. For instance, FedProx introduces a proximal term to handle data heterogeneity, which can complement our personalized layer sharing by further stabilizing the training process in non-IID settings.

% \paragraph{Empirical Results.}
% In our experiments, the Personalized Transformer Layer Sharing method demonstrated significant improvements in both model accuracy and training efficiency compared to baseline federated learning methods. Specifically, on the ONTONOTES dataset with highly non-IID partitions, our approach achieved a $5\%$ increase in accuracy while reducing training time by $20\%$. These results underscore the efficacy of combining stochastic dropout with personalized layer sharing to address the complexities of federated NLP.

% \paragraph{Conclusion.}
% Addressing non-IID data distributions is pivotal for the success of federated NLP. The Personalized Transformer Layer Sharing method, leveraging stochastic transformer layer dropout, offers a robust framework for balancing global knowledge sharing with local model personalization. By facilitating adaptive layer sharing, it enhances model performance, accelerates training, and maintains scalability, making it a valuable addition to the federated learning toolkit.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{performance_comparison.pdf}
%     \caption{Performance comparison between standard federated learning, personalized federated learning, and our Personalized Transformer Layer Sharing method on the ONTONOTES dataset.}
%     \label{fig:performance_comparison}
% \end{figure}

% \paragraph{Future Extensions.}
% Future work can explore adaptive mechanisms for dynamically selecting shared and personalized layers based on real-time performance metrics. Additionally, integrating our method with other personalization techniques, such as meta-learning or local fine-tuning, could further enhance adaptability and performance. Extending the approach to other model architectures beyond transformers and applying it to diverse NLP tasks will also broaden its applicability and impact.

% \paragraph{Summary.}
% The Personalized Transformer Layer Sharing method effectively addresses the non-IID data challenge in federated NLP by combining stochastic transformer layer dropout with personalized layer strategies. This approach enables devices to maintain local adaptability while benefiting from shared global knowledge, leading to improved model performance and training efficiency in heterogeneous federated environments.




% The challenge is a large configuration space of adapters: to which layer the adapters are injected (depth) and the capacities of individual adapters (width). The adapter configuration has a strong impact on training overhead as well as the model convergence delay.




% However, during training, function of the $l$-th layer is only active for a fraction $(1-p_{l})$ of all updates, and the corresponding weights of the next layer are calibrated for this probability. We therefore need to re-calibrate the outputs of any given function by the expected number of times it participates in training, \ie, $1-p_{l}$. The forward propagation update rule becomes $H_{l}=(1-p_{l})\cdot trans_{l}(H_{l-1}) + p_{l} \cdot Identify(H_{l-1})$. From the model ensemble perspective, the update rule can be interpreted
% as combining all possible networks into a single inference architecture, in which each layer is weighted by its dropping probability.

==> content/introduction.tex <==
Modern NLP has undergone significant advancements across various scenarios in recent years \cite{vaswani2017attention, devlin2018bert, liu2019roberta, radford2019language, brown2020language, zhao2023survey, kasneci2023chatgpt}. Notable examples include healthcare diagnostics \cite{harrer2023attention, thirunavukarasu2023large}, sentiment analysis \cite{araci2019finbert, zhang2023enhancing} and machine translation \cite{moslem2023adaptive, zhang2023prompting}.
% and content recommendation \cite{liu2024once, ren2024representation}. 
To fully realize the potential of NLP, it is required to pretrain modern NLP models (\ie, LLMs) 
% with a substantial number of parameters (ranging from hundreds of millions to thousands of billions) 
using large text corpora that typically include billions to trillions of tokens \cite{devlin2018bert, liu2019roberta, brown2020language, chowdhery2023palm, le2023bloom}. 
% Pretraining helps the models learn general linguistic patterns and knowledge of languages. 
Following this, these pretrained models are \emph{fine-tuned} on smaller, more specialized datasets labeled for specific NLP tasks and domains \cite{devlin2018bert, liu2019roberta, huang2022large}, such as question answering for mathematical problems. Fine-tuning is a pivotal step in modern NLP, as it allows models to translate their generalized language comprehension into specific expertise for downstream tasks.

\noindent \textbf{Federated NLP.} Traditionally, fine-tuning large language models (LLMs) has involved transferring text data from numerous mobile devices to central servers for training \cite{devlin2018bert, liu2019roberta, huang2022large, chen2023longlora, tinn2023fine}. However, this approach raises significant privacy concerns, due to the potential of untrusted servers and insecure communications. Fortunately, federated learning (FL) \cite{mcmahan2017communication, lai2021oort, niu2020billion, li2022pyramidfl, zheng2023autofed} offers a promising paradigm for addressing these privacy issues in NLP model fine-tuning, a practice known as federated NLP. Federated NLP \cite{cai2023efficient, zhang2023fedpetuning, lin2021fednlp} empowers mobile devices distributed across various geographical locations to collaboratively fine-tune a shared LLM while keeping their data localized. By preserving data privacy, federated NLP greatly enhances the applicability and adoption of modern NLP in privacy-sensitive mobile applications, such as healthcare diagnostics, mobile assistants, and intelligent keyboards.
% \textbf{Challenges of Federated NLP.} While federated NLP presents promising opportunities, deploying efficient and effective federated NLP systems poses significant challenges in system efficiency and model performance. First, federated NLP involves \emph{substantial training overhead}, 
% % which is significantly more demanding than traditional FL tasks, such as image classification. Specifically, the training overhead of federated NLP typically 
% which has two main components: (1) Communication.
% % Communication. In each training round, mobile devices upload their local parameters to the server and then download the updated global model. However, 
% % Modern NLP models are generally much larger than classic vision models. 
% Given that modern NLP models typically consist of a vast number of parameters, model transmissions between devices and the central server incur considerable communication costs.
% For instance, the widely-used NLP model LLaMA-7B \cite{touvron2023llama} has 7 billion trainable parameters, 
% % which is 36$\times$ more than the classic vision model DenseNet \cite{huang2017densely}. 
% % In each training round, mobile devices upload local parameters to the server and then download the updated global model. 
% leading to each model transfer round on a single device generating several gigabytes of network traffic and tens of minutes of communication delays.
% (2) Computation. The computational complexity of modern NLP models is extraordinarily high. For instance, fine-tuning LLaMA-7B with 1 million tokens requires over 40 peta floating point operations (FLOPs). % which is 500$\times$ higher than DenseNet \cite{cai2023efficient}. 
% As a result, one round of local training on each mobile device takes decades of minutes, and the end-to-end time for convergence in federated NLP can stretch to thousands of hours \cite{cai2023efficient}. 
% %In essence, while FL is generally known for its high overhead, federated NLP is particularly expensive due to the large sizes of modern NLP models and the intricate nature of NLP tasks.
% % While FL has been known for high overhead in general, federated NLP is particularly expensive, primarily because of the large sizes of modern NLP models.
% Second, the inherently \emph{non-independent and identically distributed (non-IID)} data across mobile devices represent a critical bottleneck in achieving satisfactory model performance. Local text data on mobile devices is typically collected based on the users' personal usage and geographic locations, resulting in heterogeneous data distributions across devices. For example, mobile users in specific regions may predominantly use certain languages, such as English or French, which are prevalent among certain demographics but not others. Prior works \cite{lin2021fednlp, zhang2023fedpetuning} have demonstrated that the global NLP model fine-tuned via FL often fails to generalize effectively across all devices. Consequently,  federated NLP typically experiences a model accuracy degradation of 5\%\textemdash30\% compared to centralized fine-tuning within a data center.\\

\noindent \textbf{Challenges of Federated NLP.} While federated NLP shows opportunities, deploying efficient federated NLP systems poses significant challenges due to substantial training overheads, 
% which is significantly more demanding than traditional FL tasks, such as image classification. Specifically, the training overhead of federated NLP typically 
which have two main components: (1) Communication.
% Communication. In each training round, mobile devices upload their local parameters to the server and then download the updated global model. However, 
% Modern NLP models are generally much larger than classic vision models. 
Given that modern NLP models typically consist of a vast number of parameters, model transmissions between devices and the central server incur considerable communication costs.
For instance, the widely-used NLP model LLaMA-7B \cite{touvron2023llama} has 7 billion trainable parameters, 
% which is 36$\times$ more than the classic vision model DenseNet \cite{huang2017densely}. 
% In each training round, mobile devices upload local parameters to the server and then download the updated global model. 
leading to each model transfer round on a single device generating several gigabytes of network traffic.
% and tens of minutes of communication delays.
(2) Computation. The computational complexity of modern NLP models is extraordinarily high. For instance, fine-tuning LLaMA-7B with 1 million tokens requires over 40 peta floating point operations (FLOPs). % which is 500$\times$ higher than DenseNet \cite{cai2023efficient}. 
As a result, one round of local training on each mobile device takes decades of minutes, and the end-to-end time for convergence in federated NLP can stretch to thousands of hours \cite{cai2023efficient}.

\noindent \textbf{Status Quo and Limitations.} Existing works \cite{cai2023efficient, zhang2023fedpetuning, jiang2023low, cho2023heterogeneous, qin2023federated} in federated NLP optimize the resource efficiency by leveraging solutions such as PEFT \cite{houlsby2019parameter, hu2021lora} and LLM pruning \cite{}. While PEFT is straightforward to deploy, it has significant limitations in achieving optimal efficiency. Specifically, PEFT only reduces computational overheads during the backward pass but fails to optimize the forward pass, which consumes nearly 50\% of the total on-device training costs. Besides, model pruning, a one-time and computationally intensive process, is inflexible and costly. Once model pruning is completed, it fixes the model size of all clients throughout the life cycle of federated NLP, rendering it incapable of adapting to the changing system resources. Moreover, performing pruning for LLMs inevitably incurs considerable computational overheads on devices.
% in fact, forward pass overhead may even slightly increase due to the introduction of these methods.

Even more concerning is their poor model performance in practical federated NLP scenarios. Fine-tuning only a subset of a model's parameters inherently constrains its ability to learn task-specific nuances, leading to suboptimal performance compared to full fine-tuning. In federated NLP, this limitation is further exacerbated when each device possesses data that is non-IID. The global model might not generalize well across the heterogeneous data, leading to inconsistent and inadequate performance \cite{zhang2023fedpetuning}. 

% Moreover, model pruning typically relies on global importance measures of parameters, which are hard to compute without centralized data. Parameters deemed unimportant on one client's data may be crucial when considering the entire dataset distributed across all clients. These facts lead to suboptimal model performance of PEFT and pruning compared to full fine-tuning.

% In federated NLP, the primary incentive for devices to participate in training is to collaboratively fine-tune a global model that outperforms what can be achieved locally. However, when data heterogeneity arises, performance of locally trained models often surpass that of the globally learned model through these methods (\S 2.3). This undermines the fundamental motivation for federated NLP.
% significant heterogeneity in text data distributions. Worse, these PET methods always lead to more severe model performance degradation compared to traditional fine-tuning approaches (\ie, full-parameter tuning) in practical few-shot learning scenarios (Section \ref{}). 
% Consequently, the practical implementation of existing PET methods in federated NLP is hindered by their sub-optimal system efficiency and poor model performance.
% these PET methods for federated NLP are not effectively implementable in practice due to their poor model performance.
% Alleviating the impact of few-shot or non-IID data on federated NLP has also been explored \cite{cai2023federated, jiang2023low, lit2022federated}. For instance, FeS \cite{cai2023federated} identifies pseudo labeling and prompt learning as key components for federated NLP. By carefully planning pseudo labeling and training, NLP models can be fine-tuned with only tens of labels, while achieving 85.8\%–97.0\% of the relative accuracy of fully supervised training. FedSplitBERT \cite{lit2022federated} handles heterogeneous data by splitting the BERT encoder layers into local part and global part. The local part parameters are trained by the local device only while the global part parameters are trained by aggregating gradients of multiple devices. However, no literature can fully address both data heterogeneity and few-shot learning simultaneously. We argue that data heterogeneity and few-shot learning are two prevalent challenges that often occur together in the real world. Therefore, addressing only one of the challenges while neglecting the other cannot yield optimal model performance (Section \ref{}).\\

% \noindent \textbf{Our Solutions.} To tackle the aforementioned limitations of existing methods, we identify 
% two promising opportunities for developing efficient and effective federated NLP solutions. On one hand, we highlight that the key bottleneck in enhancing on-device training efficiency stems from the necessity to update all transformer layers in the LLM. Leveraging the unique characteristic of LLMs, \ie, the uniform architecture comprising multiple identically stacked transformer layers, we introduce a comprehensive solution, \ie, stochastic transformer layer dropout, to fundamentally address computation challenges in federated NLP (\S \ref{}). The motivation behind stochastic transformer layer dropout is two folds. First, each layer in the LLM maintains consistent hidden state dimensions, ensuring that the input and output dimensions remain unchanged across layers. Second, the LLM possess a significant number of redundant layers, suggesting that not all layers are equally critical for model performance \cite{michel2019sixteen, voita2019analyzing}. Therefore, during training, we can dynamically deactivate certain layers, thereby eliminating both the forward and backward overheads associated with updating these layers without disrupting the data flow. Unlike conventional federated NLP frameworks that fine-tune all layer in the LLM, stochastic transformer layer dropout enables each device to identify an optimal subnetwork that adapts well to its changing computational resources. In contrast to model pruning, which permanently removes specific model parameters, stochastic layer dropout temporarily deactivates selected layers with certain probabilities during each training batch. A layer deactivated in the current batch retains the possibility of being activated in subsequent batches. Furthermore, upon completion of training, the LLM retains all transformer layers for inference. This approach not only ensures that every layer in the model has the opportunity to be updated, but also greatly reduces training costs by decreasing the effective model depth during training. 
% % By adopting stochastic transformer layer dropout, we achieve a balance between computational efficiency and model adaptability, paving the way for more scalable and resilient federated NLP systems.


\noindent \textbf{Our Solutions.} To tackle the aforementioned limitations of existing methods, we identify 
two promising opportunities for developing efficient and effective federated NLP solutions (\S \ref{sec:opportunities}). On one hand, we highlight that the key bottleneck in enhancing on-device training efficiency stems from the necessity to update all transformer layers in the LLM. To this end, we introduce a comprehensive solution, \ie, stochastic transformer layer dropout, to fundamentally address computation challenges in federated NLP (\S \ref{sec:layer_dropout}).
The motivation behind this solution is that LLMs poss a significant number of redundant layers \cite{michel2019sixteen, voita2019analyzing}. Therefore, during training, we can deactivate certain unimportant layers, thereby eliminating both the forward and backward overheads associated with updating these layers. 
% Since the input and output dimensions remain unchanged across all layers, the deactivation of layers will not disrupt the data flow. 
In contrast to model pruning, which permanently removes specific model parameters, stochastic layer dropout temporarily deactivates selected layers with certain probabilities (\ie, drop rates) during each training batch. A layer deactivated in the current batch retains the possibility of being activated in subsequent batches.
This approach not only ensures that every layer in the model has the opportunity to be updated, but also greatly reduces training costs by decreasing the effective model depth during training. 
% By adopting stochastic transformer layer dropout, we achieve a balance between computational efficiency and model adaptability, paving the way for more scalable and resilient federated NLP systems.

However, stochastic layer dropout cannot automatically result in optimal performance. The challenge is a large configuration space of the drop rates, which has a strong impact on training overheads as well as the model performance. Specifically, while a larger drop rate diminishes training costs, it also introduces
a risk of degrading the model performance. Besides, distributions of drop rates cross layers also impact the model accuracy. The choice is also dynamic: the favorable configuration drifts over time, depending on the learning progress and changing resources. As such, we identify configurations with high rewards, which is measured in terms of their model accuracy gains per unit wall clock time. We then employ an online exploration-exploitation
strategy to dynamically select configurations with high rewards for efficient and effective model training (\S \ref{sec:configurator}).
% drop rate configurations through an exploration-exploitation strategy. The controller identifies configurations with high rewards, which is measured in terms of their model accuracy gains per unit wall clock time


% In this work, we develop a comprehensive solution to fundamentally address the computation, communication, and model performance challenges in federated NLP.

% In this work, we propose Yagi to simultaneously (1) enable the
% flexible training of subnetworks, tailored to dynamic resource constraints., (2) ensure on-device computational efficiency by optimizing both the forward and backward passes, and (3) achieves state-of-the-art model performance on non-IID text data. 
% The key idea of $P^{3}$ is that, instead of fine-tuning the base LLMs in conventional federated NLP frameworks, each device will first find a personalized subnetwork that can generalize well for its local data and only the parameters of the subnetwork will be fine-tuned locally (\S 4.1). The key intuition behind $P^{3}$ is inspired by the “lottery ticket hypothesis" [14], which finds that an optimal substructure of the original network can be identified through pruning and such a subnetwork can reach similar performance as the original network. Through selectively removing non-critical coupled structures in the base LLM based on gradient information, we can maximally preserve the majority of the LLM’s functionality. In this way, $P^{3}$ can not only ensure that the model performance is not compromised in the case of non-IID data, but also significantly improve both the forward and backward pass efficiency due to the compact size of the subnetwork. 
% Specifically, rather than fine-tuning the entire base LLM as in conventional federated NLP frameworks, our approach has each device first identify an optimal subnetwork that generalizes well to its local data distribution (\S 4.1). Subsequently, only the parameters of this subnetwork are fine-tuned locally on devices . The intuition is that through \emph{pruning}, we can discover a substructure within the original network that maintains performance comparable to the full base LLM. By selectively removing non-critical coupled structures in the LLM based on gradient information, we can maximally preserve the core functionality of the LLM. This strategy can not only ensure that the performance of pruned models can be efficiently recovered through fine-tuning, but also significantly reduce the computational overhead of both the forward and backward passes due to the subnetwork's compressed size.

% \begin{figure}[t] \centering
%     \includegraphics[width=0.485\textwidth]
%     {content/picture/first_chapter/P3_overview.pdf}
%     \caption{Significant communication costs, computational overheads, and challenges posed by non-IID data are key bottlenecks in federated NLP. P$^{3}$ overcomes these obstacles trough novel techniques.}\label{fig:overview}
% \end{figure}

% After carefully LLMs pruning, we integrate PET methods into P$^{3}$ to further diminish the training overhead during local fine-tuning; however, 
On the other hand, one misconception in traditional federated NLP is that all local model parameters on devices should be aggregated into a single global model. This not only maximizes communication costs between devices and the server, but also fails to account for the inherently non-IID device data. Therefore, we propose personalized
transformer layer sharing to address this challenge (\S \ref{sec:layer_sharing}). The motivation is that certain personalized local encoders (\ie, certain transformer layers and the LLM head) instead of a single global model can better process specialized local data. Having personalized encoders extract useful local representations means that the global model now requires fewer number of layers. To this end, we partition each LLM on the device into two parts, \ie, personalized layers (with the LLM head) and global shared layers. In particular, layer partitioning on each device is driven by its local data, leading devices holding similar data distributions to share similar layer architectures and more overlapped parameters. After local fine-tuning in each round, devices only transmit the shared layers to the central server for global aggregation (\S 4.2). Consequently, LLMs on devices are able to capture representations embedded in local data while effectively sharing collective knowledge derived from global data.


% fine-tuned model parameters into two parts, \ie, \emph{personalized} parameters and global parameters. In particular, these partitioning on each device is driven by its local data, leading devices holding similar data distributions to share similar parameter architectures and more overlapped global parameters. After local fine-tuning in each round, devices only transmit the global parameters to the central server (\S 4.2). This enables each device to learn personalized local parameters for extracting local data features. Consequently, the fine-tuned LLMs are able to capture representations embedded in local data while effectively sharing collective knowledge derived from global data (\ie, the aggregation of local data from all devices). This strategy empowers P$^{3}$ to achieve optimal model performance on non-IID data.

% by allowing models to be tailored to the individual characteristics of each device.

% previous works that transmit all fine-tuned parameters between devices and the server to aggregate a globally unified model


 % we partition the fine-tuned model parameters into two parts, \ie, \emph{personalized} parameters and global parameters. In particular, these partitioning on each device is driven by its local data, leading devices holding similar data distributions to share similar parameter architectures and more overlapped global parameters. After local fine-tuning in each round, devices only transmit the global parameters to the central server (\S 4.2). This enables each device to learn personalized local parameters for extracting local data features. Consequently, the fine-tuned LLMs are able to capture representations embedded in local data while effectively sharing collective knowledge derived from global data (\ie, the aggregation of local data from all devices). This strategy empowers P$^{3}$ to achieve optimal model performance on non-IID data.

% \textbf{Practical Applications.}
% We further extend P$^{3}$ by exploring its realistic application in a more \emph{challenging} and \emph{practical} setting (\S 5), where heterogeneous devices in federated NLP systems have significantly different (and even dynamic) computational capabilities. To address these challenges, we propose pruning heterogeneous local LLMs with varying computational complexities tailored to each device's computing capabilities. Moreover, recognizing the impact of the pruned model size on model performance, we identify the local validation loss on each device as a key indicator to guide the setting of the model pruning ratio. This approach enables each device in the federated NLP system to efficiently participate in federated model fine-tuning and achieve satisfactory model performance, regardless of its computational limitations. By accommodating device heterogeneity in this manner, P$^{3}$ effectively enhances system efficiency, thereby advancing the practical deployment of federated NLP in real-world scenarios.\\
\noindent \textbf{Contributions.} 
% Figures \ref{fig:overview} illustrates the practical challenges in federated NLP and the high-level overview of P$^{3}$. 
Overall, we make the following contributions in this paper:
\begin{itemize}[leftmargin=*]
    \item We highlight the key limitations of existing federated NLP solutions in system efficiency and model performance.
    \item We address the limitations with several novel designs: stochastic transformer layer dropout, exploration-exploitation based drop rate decision and personalized transformer layer sharing.
    \item Through experiments on real hardware, we show our designs outperform state-of-the-art solutions across various datasets and NLP models on both system efficiency and model performance.
    
    
    
    
    % We propose P$^{3}$, a novel and efficient federated NLP framework that enhances system efficiency and model performance on non-IID text data.
    % \item To the best of our knowledge, P$^{2}$ is the first framework that achieves personalization while jointly improving the efficiency of communication and computation in federated NLP. We believe that our work represents a significant step towards applying practical federated NLP to resource-constrained mobile devices.
    % \item P$^{2}$ contributes several effective techniques, \eg, personalized pruning techniques and PET methods, that address the limitations in state-of-the-arts of federated NLP.
    % \item Addressing practical challenges in federated NLP, we extend P$^{3}$ to settings with devices having heterogeneous computational capabilities.
    % \item P$^{3}$ outperforms state-of-the-arts [9, 15 , 17, 18] across various datasets and NLP models on both system efficiency and model performance. Specifically, P$^{3}$ reduces communication and computation costs by 23.71\%-49.71\% and 23.71\%-49.71\%, respectively, while achieving 3.68\%-7.33\% higher final test accuracy, compared with state-of-the-arts.
\end{itemize}
 

==> content/introduction1.tex <==
Modern NLP has undergone significant advancements across various scenarios in recent years \cite{vaswani2017attention, devlin2018bert, liu2019roberta, radford2019language, brown2020language, zhao2023survey, kasneci2023chatgpt}. Notable examples include healthcare diagnostics \cite{thirunavukarasu2023large}, sentiment analysis \cite{zhang2023enhancing}, and machine translation \cite{zhang2023prompting}.
% and content recommendation \cite{liu2024once, ren2024representation}. 
To fully realize the potential of NLP, it is required to pre-train modern NLP models (\ie, LLMs) 
% with a substantial number of parameters (ranging from hundreds of millions to thousands of billions) 
using large public text corpora \cite{devlin2018bert, liu2019roberta, brown2020language, chowdhery2023palm, le2023bloom}. 
Following this, these pre-trained models are \emph{fine-tuned} on more specialized datasets labeled for downstream NLP tasks and domains \cite{devlin2018bert, liu2019roberta, huang2022large}, such as question answering for mathematical problems. Fine-tuning is crucial, as it allows LLMs to translate their generalized language comprehension into specific expertise for downstream tasks.

\noindent \textbf{Federated fine-tuning.} Traditionally, fine-tuning LLMs has involved transferring text data from numerous mobile devices to cloud servers for training \cite{devlin2018bert, liu2019roberta, huang2022large, chen2023longlora, tinn2023fine}. However, this approach raises significant privacy concerns due to the risks posed by untrusted servers and insecure communications. Fortunately, federated fine-tuning \cite{cai2023efficient, zhang2023fedpetuning, lin2021fednlp}, which empowers various mobile devices to collaboratively fine-tune a shared LLM while keeping their data localized, offers a promising paradigm for addressing the privacy issues. However, given that LLMs typically consist of a vast number of parameters, the memory footprint and computational/communication overheads for federated fine-tuning are extraordinarily high. For instance, in each federated round, fine-tuning GPT-2 \cite{} on each device requires over 24GB of GPU memory and 7 peta floating point operations (FLOPs), and consumes 3GB of network traffic. As a result, one round of fine-tuning takes several hours, and the end-to-end convergence time can stretch to thousands of hours \cite{cai2023efficient}.

\noindent \textbf{Status Quo and Limitations.} To optimize the training efficiency, federated parameter-efficient fine-tuning (PEFT) \cite{cai2023efficient, zhang2023fedpetuning, jiang2023low, cho2023heterogeneous} is the most common and straightforward approach. By adding lightweight modules (\eg, adapters \cite{houlsby2019parameter} and low-rank matrices \cite{hu2021lora}) while keeping the original model frozen, PEFT effectively reduces the on-device training overheads. Besides, since only the parameters in added modules are communicated between devices and the server, the communication overheads are also mitigated.
% Existing works in federated NLP optimize the training efficiency by leveraging solutions such as PEFT  and LLM pruning \cite{}. 
However, PEFT has notable limitations in achieving optimal performance. First, it only reduces the on-device training overheads during the backward pass but fails to optimize the forward pass, which accounts for 35-40\% and 40\%-50\% of the total memory footprint and on-device training time, respectively
(\S \ref{subsec:limitations}). Second, 
despite the use of lightweight modules, the parameters in
these modules can still be considerable due to large sizes of LLMs, leading to high communication overheads.
% due to the large size of LLMs, even the added modules in PEFT still have considerable parameters, resulting in high communication overheads.
% while PEFT only communicates the parameters in added modules,  still be large in absolute size. even parameters in added modules can still be large absolute size.
% Besides, model pruning, a one-time and computationally intensive process, is inflexible and costly. Once model pruning is completed, it fixes the model size of all devices throughout the life cycle of federated NLP, rendering it incapable of adapting to the changing system resources. 
% Moreover, performing pruning for LLMs inevitably incurs considerable computational overheads on devices. 
% Even more concerning is their significantly poor model performance in practical federated NLP scenarios, where devices always possess non-IID data \cite{zhang2023fedpetuning}. As we will show (\S \ref{}), these non-IID data render the prior works inadequate, resulting in significant loss in training accuracy.
The key bottlenecks in PEFT stem from its necessity to operate on all transformer layers in the LLM. Specifically, each layer in the model needs to be updated during on-device training and the parameter updates in all layers are transferred during communications. Since LLMs typically contain a significant number of redundant layers \cite{michel2019sixteen, voita2019analyzing}, this strategy introduces substantial overheads.

In addition to the inefficiency of the PEFT methods, even more concerning is their poor model performance in practical federated fine-tuning scenarios. In each round, the parameter updates from all layers on each device are aggregated into a single global model. While this approach is effective in ideal settings with IID data, it performs poorly in practical federated fine-tuning scenarios, where devices typically possess non-IID data \cite{zhang2023fedpetuning}. In non-IID scenarios, parameter gradients from any device provide a biased estimation of the global gradients on the total data from all devices. As we will show in \S \ref{subsec:limitations}, the presence of non-IID data undermines the effectiveness of prior methods, resulting in significant loss in training accuracy.
% Therefore, to fundamentally tackle the limitations of existing methods, it is essential to elaborately optimize federated fine-tuning at the granularity of individual transformer layers.

\noindent \textbf{Our Solutions.} In this work, we present an efficient and effective system called Yagi, which introduces two novel layer-wise optimization strategies as key building blocks of advanced PEFT. The core idea behind Yagi is that, instead of processing all transformer layers in the LLM, each device will stochastically update the lightweight modules in a subset of layers during on-device training (\ie, stochastic transformer layer dropout) and then only the parameter updates in partial layers instead of all layers will be communicated between devices and the server (\ie, personalized transformer layer sharing). Specifically, in each round of federated fine-tuning, each participating device in Yagi first performs local fine-tuning by deactivating certain unimportant layers with certain probabilities (\ie, drop rates) within each training batch. Once local fine-tuning is completed, devices partition their LLMs into two parts, \ie, personalized layers and globally shared layers. Only the parameter updates in shared layers are transmitted to the server for global aggregation. 
% Notably, Yagi is fully compatible with the PEFT methods. This is because PEFT injects new modules into each transformer layer, whereas Yagi’s layer-wise strategies are intentionally decoupled from the internal structure of the layers. 
% In \S \ref{sec:layer_dropout}, we discuss how Yagi can be easily and effectively combined with PEFT to further enhance training efficiency.
% Notably, Yagi is compatible with the vanilla full fine-tuning framework \cite{lin2021fednlp} without the PEFT methods. This is because Yagi’s layer-wise strategies are intentionally decoupled from the internal structure of the transformer layer, whereas PEFT injects new modules into each layer. This means that the layer-wise strategies in Yagi and the PEFT methods are fully orthogonal.

% To further enhance training efficiency, we propose to easily and seamlessly integrate PEFT into Yagi in \S \ref{sec:layer_dropout}.

By the two layer-wise strategies, Yagi has several advantages: (1) Yagi can 
eliminate both the forward and backward training overheads associated with the deactivated layers. Consequently, the memory footprint and training time required for on-device training are significantly reduced.
% (2) A layer deactivated in the current batch may be reactivated in subsequent batches, ensuring that every layer in the LLM has the opportunity to be updated over time.
(2) Yagi can effectively reduce communication overheads between devices and the server by only sharing the parameter updates of partial layers. (3) 
LLMs on devices are able to capture representations embedded in local data by the personalized layers, while effectively sharing collective knowledge derived from global data by the shared layers. This promotes Yagi to achieve more excellent training accuracy on non-IID data.
% To tackle the aforementioned limitations of existing methods, we identify two promising opportunities for developing efficient and effective federated NLP solutions (\S \ref{sec:opportunities}). 
% On one hand, we highlight that the key bottleneck in enhancing on-device training efficiency stems from the necessity to update all transformer layers in the LLM. 
% To this end, we introduce a comprehensive solution, \ie, stochastic transformer layer dropout, to fundamentally address computation challenges in federated NLP (\S \ref{sec:layer_dropout}).
% The motivation behind this solution is that LLMs poss a significant number of redundant layers \cite{michel2019sixteen, voita2019analyzing}. Therefore, during training, we can deactivate certain unimportant layers, thereby eliminating both the forward and backward overheads associated with updating these layers.
% In contrast to model pruning, which permanently removes specific model parameters, stochastic layer dropout temporarily deactivates selected layers with certain probabilities (\ie, drop rates) during each training batch. A layer deactivated in the current batch retains the possibility of being activated in subsequent batches.
% This approach not only ensures that every layer in the model has the opportunity to be updated, but also greatly reduces training costs by decreasing the effective model depth during training. 
% However, the design of Yagi involves two key technical challenges: (1) The first challenge lies in designing an effective method to decide a proper drop rate for each transformer layer. While a larger drop rate diminishes training costs, it also introduces a risk of degrading the model accuracy. Besides, the optimal drop rate varies with computing resources of devices, distributions of data, and locations of layers. (2) Considering the non-IID data and varying drop rate configurations across devices, 
However, unleash Yagi's maximum potential, \ie, achieving the optimal training efficiency and model performance, presents two key technical challenges: (1) Designing effective strategies to assign an appropriate drop rate to each transformer layer, and (2) determining which layers are shared for global aggregation. Specifically, the drop-rate configuration and personalized-shared layer partition have strong impact on training overheads and model performance. While a larger drop-rate configuration diminishes training overheads, it also introduces a risk of degrading the model performance. Besides, the optimal layer partition on each device varies across non-IID data. The choice is also dynamic: the favorable configuration and partition drift over time, depending on the learning progress and changing resources. To address these challenges, we integrate two online strategies into Yagi, which automatically and dynamically determine the proper drop-rate configuration and layer partition for each device (Section \ref{}).
% efficient and effective federated fine-tuning .

% % \begin{figure}[t] \centering
% %     \includegraphics[width=0.485\textwidth]
% %     {content/picture/first_chapter/P3_overview.pdf}
% %     \caption{Significant communication costs, computational overheads, and challenges posed by non-IID data are key bottlenecks in federated NLP. P$^{3}$ overcomes these obstacles trough novel techniques.}\label{fig:overview}
% % \end{figure}

% On the other hand, one misconception in traditional federated NLP is that all local model parameters on devices should be aggregated into a single global model. This not only maximizes communication costs between devices and the server, but also fails to account for the inherently non-IID device data. Therefore, we propose personalized
% transformer layer sharing to address this challenge (\S \ref{sec:layer_sharing}). The motivation is that certain personalized local encoders (\ie, certain transformer layers and the LLM head) instead of a single global model can better process specialized local data. Having personalized encoders extract useful local representations means that the global model now requires fewer number of layers. To this end, we partition each LLM on the device into two parts, \ie, personalized layers (with the LLM head) and global shared layers. In particular, layer partitioning on each device is driven by its local data, leading devices holding similar data distributions to share similar layer architectures and more overlapped parameters. After local fine-tuning in each round, devices only transmit the shared layers to the central server for global aggregation (\S 4.2). Consequently, LLMs on devices are able to capture representations embedded in local data while effectively sharing collective knowledge derived from global data.

\noindent \textbf{Contributions.} 
% Figures \ref{fig:overview} illustrates the practical challenges in federated NLP and the high-level overview of P$^{3}$. 
Overall, we make the following contributions in this paper:
\begin{itemize}[leftmargin=*]
    \item We analyze the limitations of the PEFT methods in training efficiency and model performance. Based on this analysis, we propose Yagi to enhance PEFT with two novel layer-wise strategies: stochastic transformer layer dropout and personalized transformer layer sharing.
    % \item We enhance federated fine-tuning with two novel layer-wise strategies: stochastic transformer layer dropout and personalized transformer layer sharing.
    \item We identify the challenges of the drop-rate configuration and layer partition in Yagi, then design the online algorithms to determine the optimal configuration and partition for efficient and effective federated fine-tuning.
    \item Through experiments on real hardware, we show Yagi outperform state-of-the-art solutions across various datasets and models.
    
    
    
    
    % We propose P$^{3}$, a novel and efficient federated NLP framework that enhances system efficiency and model performance on non-IID text data.
    % \item To the best of our knowledge, P$^{2}$ is the first framework that achieves personalization while jointly improving the efficiency of communication and computation in federated NLP. We believe that our work represents a significant step towards applying practical federated NLP to resource-constrained mobile devices.
    % \item P$^{2}$ contributes several effective techniques, \eg, personalized pruning techniques and PET methods, that address the limitations in state-of-the-arts of federated NLP.
    % \item Addressing practical challenges in federated NLP, we extend P$^{3}$ to settings with devices having heterogeneous computational capabilities.
    % \item P$^{3}$ outperforms state-of-the-arts [9, 15 , 17, 18] across various datasets and NLP models on both system efficiency and model performance. Specifically, P$^{3}$ reduces communication and computation costs by 23.71\%-49.71\% and 23.71\%-49.71\%, respectively, while achieving 3.68\%-7.33\% higher final test accuracy, compared with state-of-the-arts.
\end{itemize}
 

==> content/introduction2.tex <==
Modern NLP has undergone significant advancements across various scenarios in recent years \cite{vaswani2017attention, devlin2018bert, liu2019roberta, radford2019language, brown2020language, zhao2023survey, kasneci2023chatgpt}. Notable examples include healthcare diagnostics \cite{thirunavukarasu2023large}, sentiment analysis \cite{zhang2023enhancing}, and machine translation \cite{zhang2023prompting}.
% and content recommendation \cite{liu2024once, ren2024representation}. 
To fully realize the potential of NLP, it is required to pre-train modern NLP models (\ie, LLMs) 
% with a substantial number of parameters (ranging from hundreds of millions to thousands of billions) 
using large public text corpora \cite{devlin2018bert, liu2019roberta, brown2020language, chowdhery2023palm, le2023bloom}. 
Following this, these pre-trained LLMs are \emph{fine-tuned} on more specialized datasets labeled for various downstream NLP tasks \cite{devlin2018bert, liu2019roberta, huang2022large}, such as question answering for mathematical problems. Fine-tuning is crucial, as it allows LLMs to translate their generalized language comprehension into specific expertise for downstream tasks.

\noindent \textbf{Federated fine-tuning.} Traditionally, fine-tuning LLMs has involved transferring text data from numerous edge devices to cloud servers for training \cite{devlin2018bert, liu2019roberta, huang2022large, chen2023longlora, tinn2023fine}. However, this approach raises significant privacy concerns due to the risks posed by untrusted servers and insecure communications. Fortunately, federated fine-tuning \cite{cai2023efficient, zhang2023fedpetuning, lin2021fednlp}, which empowers various edge devices to collaboratively fine-tune a shared LLM while keeping their data localized, offers a promising paradigm to address the privacy issues. However, given that LLMs typically consist of a vast number of parameters, the memory footprint and computational overheads for federated fine-tuning are extraordinarily high. For instance, in each federated round, fine-tuning a relatively small LLM (GPT-2 \cite{radford2019language}) even requires over 30GB of GPU memory and 15 peta floating point operations (FLOPs). As a result, one round of fine-tuning takes several hours, and the end-to-end convergence time will stretch to thousands of hours \cite{cai2023efficient}.

% \noindent \textbf{Status quo and limitations.} To optimize the training efficiency, federated parameter-efficient fine-tuning (PEFT) \cite{cai2023efficient, zhang2023fedpetuning, jiang2023low, cho2023heterogeneous} has emerged as the dominant strategy. By adding lightweight modules (\eg, adapters \cite{houlsby2019parameter} and low-rank matrices \cite{hu2021lora}) while keeping the base LLM frozen, PEFT reduces the on-device fine-tuning overheads.
% However, PEFT has notable limitations in achieving optimal performance. First, on-device fine-tuning necessitates extensive GPU memory to store intermediate results such as activations and gradients. Although PEFT could omit most gradients with parameters frozen, activations continue to demand considerable memory (\S \ref{}). Second, PEFT only speeds up on-device fine-tuning during the backward pass but fails to optimize the forward pass. The majority of FLOPs in the forward pass come from the base model, which PEFT does not compress or skip. Thus, the forward pass computation remains nearly identical to full fine-tuning, accounting for about 45\% of the total on-device fine-tuning time (\S \ref{subsec:limitations}). These limitations make it impractical for existing PEFT methods to effectively fine-tuning even small LLMs (\eg, GPT-2) in federated fine-tuning scenarios, where most participating devices have limited computing capabilities and memory capacities (\eg, with less than 100 tera operations per second and 10GB memory).

% The key bottlenecks in PEFT stem from its nature to modify the LLM by adding parameters into each transformer layer rather than replacing or compressing existing one. Specifically, during on-device fine-tuning, the input must propagate through \emph{all} transformer layers (even with frozen parameters) in the LLM. As a result, the frozen base LLM’s computational graph of the forward pass remains intact. Besides, gradients for the trainable PEFT modules depend on activations from preceding transformer layers. For example, to compute gradients for a PEFT module in layer $L$, activations from layer $(L-1)$ are required. Thus, \emph{all} layers must retain intermediate activations to support gradient calculations for the trainable parameters. Since LLMs typically contain a significant number of redundant layers \cite{michel2019sixteen, voita2019analyzing}, PEFT introduces substantial computing and memory overheads.
% This prompts an essential question: is there a feasible approach for PEFT to eliminate computations and activations of certain transformer layers?

% \noindent \textbf{Status quo and limitations.} To optimize the training efficiency, federated parameter-efficient fine-tuning (PEFT) \cite{cai2023efficient, zhang2023fedpetuning, jiang2023low, cho2023heterogeneous} has emerged as the dominant strategy. By adding lightweight modules (\eg, adapters \cite{houlsby2019parameter} and low-rank matrices \cite{hu2021lora}) while keeping the base LLM frozen, PEFT reduces the fine-tuning overheads on devices.
% However, PEFT has two fundamental bottlenecks that throttle its practicality. First, on-device fine-tuning necessitates extensive GPU memory to store intermediate results such as activations and gradients. Although PEFT could omit most gradients with parameters frozen, activations continue to demand considerable memory (\S \ref{}). Second, PEFT only accelerates the backward pass during fine-tuning but fails to optimize the forward pass. The majority of FLOPs in the forward pass come from the base model, which PEFT does not skip. Thus, the forward pass computation remains nearly identical to full fine-tuning, accounting for about 45\% of the total on-device computation time (\S \ref{subsec:limitations}). Consequently, federated fine-tuning of even modest LLMs like GPT-2 remains infeasible for resource-constrained devices (\eg, those with less than 100 tera operations per second and 10GB memory).

% % These limitations make it impractical for existing PEFT methods to effectively fine-tuning even modest LLMs (\eg, GPT-2) in federated fine-tuning scenarios, where most participating devices have limited computing capabilities and memory capacities (\eg, with less than 100 tera operations per second and 10GB memory).

% The root cause lies in PEFT's \emph{additive} design philosophy: it grafts new parameters onto each transformer layer in the LLM rather than compressing these layers. This architectural choice imposes an unavoidable tax: during fine-tuning, inputs must propagate through \emph{all} transformer layers. As a result, the frozen base model's computational graph of the forward pass remains intact. Besides, gradients for PEFT modules depend recursively on activations from preceding transformer layers. For example, computing gradients for a PEFT module at layer $L$ requires cached activations from layer $(L-1)$. Thus, \emph{all} layers must retain intermediate activations to support gradient calculations. Since LLMs typically contain a significant number of redundant layers \cite{michel2019sixteen, voita2019analyzing}, PEFT introduces substantial computing and memory overheads.
% This raises a pivotal question: \emph{Can we redesign PEFT to strategically bypass redundant layers, eliminating both their computations and activations without compromising model fidelity?}

\noindent \textbf{Status quo and limitations.} To optimize the training efficiency, federated parameter-efficient fine-tuning (PEFT) \cite{cai2023efficient, zhang2023fedpetuning, jiang2023low, cho2023heterogeneous} has emerged as the dominant strategy. By adding lightweight modules (\eg, adapters \cite{houlsby2019parameter} or low-rank matrices \cite{hu2021lora}) while keeping the base LLM frozen, PEFT effectively reduces the trainable parameters on devices.
However, PEFT has two fundamental bottlenecks that throttle its practicality due to its \emph{additive} design philosophy: it grafts new parameters onto each transformer layer in the LLM rather than compressing these layers (\S \ref{subsec:limitations}).

% However, PEFT has two fundamental bottlenecks that throttle its practicality (\S \ref{subsec:limitations}). The root cause lies in PEFT's \emph{additive} design philosophy: it grafts new parameters onto each transformer layer in the LLM rather than compressing these layers. 

First, this architectural choice imposes an unaffordable computational tax: during fine-tuning, inputs must propagate through \emph{all} transformer layers even with frozen parameters. While PEFT accelerates the backward pass during fine-tuning, the frozen base model's computational graph of the forward pass remains intact. The majority of FLOPs in the forward pass come from the frozen base model, which PEFT does not skip. As a result, PEFT fails to optimize the forward pass, whose computation remains nearly identical to full fine-tuning (FFT)\footnote{FFT updates all parameters in the LLM during the backward pass.}, accounting for about 45\% of the total on-device computation time (\S \ref{subsec:limitations}). Second, fine-tuning LLMs necessitates extensive GPU memory to store intermediate results such as activations and gradients \cite{korthikanti2023reducing}. Gradients for PEFT modules depend recursively on activations from preceding transformer layers. For example, computing gradients for a PEFT module at layer $L$ requires cached activations from layer $(L-1)$. Thus, \emph{all} layers must retain intermediate activations to support gradient calculations. Although PEFT could omit most gradients with parameters frozen, activations continue to demand considerable memory. 

Since LLMs typically contain a significant number of transformer layers \cite{michel2019sixteen, voita2019analyzing}, PEFT introduces substantial computing and memory overheads for all layers. Consequently, federated fine-tuning of even modest LLMs like GPT-2 remains infeasible for resource-constrained devices, \eg, those with computational capabilities of $<10$ tera operations per second (TOPS) and $<10$GB GPU memory. This raises a pivotal question: \emph{Can we redesign PEFT to strategically bypass certain layers, eliminating both their computations and activations without compromising model fidelity?}

% The root cause lies in PEFT's \emph{additive} design philosophy: it grafts new parameters onto each transformer layer in the LLM rather than compressing these layers. This architectural choice imposes an unavoidable tax: during fine-tuning, inputs must propagate through \emph{all} transformer layers. As a result, the frozen base model's computational graph of the forward pass remains intact. Besides, gradients for PEFT modules depend recursively on activations from preceding transformer layers. For example, computing gradients for a PEFT module at layer $L$ requires cached activations from layer $(L-1)$. Thus, \emph{all} layers must retain intermediate activations to support gradient calculations. Since LLMs typically contain a significant number of redundant layers \cite{michel2019sixteen, voita2019analyzing}, PEFT introduces substantial computing and memory overheads.
% This raises a pivotal question: \emph{Can we redesign PEFT to strategically bypass redundant layers, eliminating both their computations and activations without compromising model fidelity?}


\noindent \textbf{Our solutions.} We thereby present an efficient and effective system called Yagi, which introduces a novel layer-wise optimization strategy, \ie, stochastic transformer layer dropout, as the key building block to enhance PEFT. Unlike conventional PEFT methods that retain all transformer layers during training, Yagi dynamically identifies and skips certain computationally costly layers in both forward and backward passes. This innovation hinges on a key insight: transformer layers exhibit considerable redundancy, enabling selective deactivation without catastrophic knowledge loss \cite{men2024shortgpt, song2024sleb, chen2024compressing}.
% Shortgpt: Layers in large language models are more redundant than you expect
% SLEB: Streamlining LLMs through Redundancy Verification and Elimination of Transformer Blocks
% Compressing large language models by streamlining the unimportant layer


At its core, Yagi operates through probabilistic layer dropout. During each training batch, participating devices fine-tune the LLM by stochastically deactivating subsets of transformer layers according to certain probabilities (\ie, drop rates). Inputs propagate only through activated layers, while deactivated layers reuse activations from their nearest active predecessors. Critically, this dropout is temporary and dynamic: a layer deactivated in one batch may be reactivated in subsequent batches, ensuring all layers in the LLM contribute cumulatively over time. By stochastic transformer layer dropout, Yagi eliminates both computations and activations for deactivated layers. Consequently, the memory usage and training time required for fine-tuning are significantly reduced.

However, unleashing Yagi's full potential presents a key technical challenge: \emph{How to design an effective strategy to assign an appropriate drop rate to each transformer layer.} This drop-rate configuration govern the trade-off between fine-tuning efficiency and model fidelity. Overly aggressive dropout introduces a risk of degrading the model performance, while overly conservative drop rates squander computational resources. Compounding this, the importance of a layer varies with its position in the LLM. For instance, deeper layers may prioritize semantic coherence while shallower layers tend to extract shallow features.
% Besides, since different layers have various importance, proper distributions of drop rates cross layers are essential for model performance. 
The choice is also dynamic: the favorable drop-rate configuration drifts over time and devices, depending on the learning progress and changing resources. 
To address this, Yagi employs an online exploration-exploitation strategy that dynamically optimizes drop rates based on real-time rewards, quantified as model accuracy gains per unit wall-clock time. This adaptive mechanism evaluates candidate configurations through a multi-armed bandit framework, prioritizing high-reward dropout policies while maintaining exploratory diversity. By continuously adapting to device and learning-phase demands, Yagi achieves efficient and effective federated fine-tuning.
% To address this challenge, we identify configurations with high rewards, which are measured in terms of their model accuracy gains per unit wall clock time. We then employ an online exploration-exploitation strategy to dynamically select configurations with high rewards for efficient and effective model fine-tuning (\S \ref{}).
% efficient and effective federated fine-tuning.

% % \begin{figure}[t] \centering
% %     \includegraphics[width=0.485\textwidth]
% %     {content/picture/first_chapter/P3_overview.pdf}
% %     \caption{Significant communication costs, computational overheads, and challenges posed by non-IID data are key bottlenecks in federated NLP. P$^{3}$ overcomes these obstacles trough novel techniques.}\label{fig:overview}
% % \end{figure}

% On the other hand, one misconception in traditional federated NLP is that all local model parameters on devices should be aggregated into a single global model. This not only maximizes communication costs between devices and the server, but also fails to account for the inherently non-IID device data. Therefore, we propose personalized
% transformer layer sharing to address this challenge (\S \ref{sec:layer_sharing}). The motivation is that certain personalized local encoders (\ie, certain transformer layers and the LLM head) instead of a single global model can better process specialized local data. Having personalized encoders extract useful local representations means that the global model now requires fewer number of layers. To this end, we partition each LLM on the device into two parts, \ie, personalized layers (with the LLM head) and global shared layers. In particular, layer partitioning on each device is driven by its local data, leading devices holding similar data distributions to share similar layer architectures and more overlapped parameters. After local fine-tuning in each round, devices only transmit the shared layers to the central server for global aggregation (\S 4.2). Consequently, LLMs on devices are able to capture representations embedded in local data while effectively sharing collective knowledge derived from global data.

\noindent \textbf{Contributions.} 
% Figures \ref{fig:overview} illustrates the practical challenges in federated NLP and the high-level overview of P$^{3}$. 
Overall, we make the following contributions in this paper:
\begin{itemize}[leftmargin=*]
    \item We analyze the limitations of the PEFT methods in training efficiency and propose Yagi to enhance PEFT with a novel layer-wise strategy, \ie, stochastic transformer layer dropout.
    % \item We enhance federated fine-tuning with two novel layer-wise strategies: stochastic transformer layer dropout and personalized transformer layer sharing.
    \item We identify the challenges of the drop-rate configuration in Yagi, then design an online exploration-exploitation algorithm to determine the optimal configuration for efficient and effective federated fine-tuning.
    \item Through experiments on real hardware, we show Yagi outperform state-of-the-art solutions across various datasets and models.
    
    
    
    
    % We propose P$^{3}$, a novel and efficient federated NLP framework that enhances system efficiency and model performance on non-IID text data.
    % \item To the best of our knowledge, P$^{2}$ is the first framework that achieves personalization while jointly improving the efficiency of communication and computation in federated NLP. We believe that our work represents a significant step towards applying practical federated NLP to resource-constrained mobile devices.
    % \item P$^{2}$ contributes several effective techniques, \eg, personalized pruning techniques and PET methods, that address the limitations in state-of-the-arts of federated NLP.
    % \item Addressing practical challenges in federated NLP, we extend P$^{3}$ to settings with devices having heterogeneous computational capabilities.
    % \item P$^{3}$ outperforms state-of-the-arts [9, 15 , 17, 18] across various datasets and NLP models on both system efficiency and model performance. Specifically, P$^{3}$ reduces communication and computation costs by 23.71\%-49.71\% and 23.71\%-49.71\%, respectively, while achieving 3.68\%-7.33\% higher final test accuracy, compared with state-of-the-arts.
\end{itemize}
 

==> content/introduction3.tex <==
Modern NLP has undergone significant advancements across various domains in recent years \cite{vaswani2017attention, devlin2018bert, liu2019roberta, radford2019language, brown2020language, zhao2023survey, kasneci2023chatgpt}. Notable examples include healthcare diagnostics \cite{thirunavukarasu2023large}, sentiment analysis \cite{zhang2023enhancing}, and machine translation \cite{zhang2023prompting}.
% and content recommendation \cite{liu2024once, ren2024representation}. 
These breakthroughs are driven by large language models (LLMs), which are pre-trained on extensive public text corpora \cite{devlin2018bert, liu2019roberta, brown2020language, chowdhery2023palm, le2023bloom}. To fully realize the potential of NLP, these models are then
\emph{fine-tuned} on domain-specific datasets to optimize their performance for downstream tasks, such as question answering for mathematical problems. Fine-tuning plays a crucial role in enabling LLMs to evolve from general language comprehension to task-specific expertise \cite{devlin2018bert, liu2019roberta, huang2022large}.


% % To fully realize the potential of NLP, modern NLP models (\ie, LLMs) are pre-trained on large public text corpora \cite{devlin2018bert, liu2019roberta, brown2020language, chowdhery2023palm, le2023bloom}.
% Subsequently, these pre-trained models are \emph{fine-tuned} on specialized datasets tailored to downstream NLP tasks and domains \cite{devlin2018bert, liu2019roberta, huang2022large}, such as question answering for mathematical problems. Fine-tuning is crucial, as it enables LLMs to adapt their generalized language comprehension into task-specific expertise.

\noindent \textbf{Federated fine-tuning.} Typically, task-specific data for fine-tuning, such as user messages or emails, are continuously generated by end users across a variety of end devices (\eg, mobile devices, personal computers and embedded devices). However, such data are privacy-sensitive in many cases, 
raising significant privacy concerns when collected for fine-tuning LLMs.
To address this issue, federated fine-tuning has emerged as the de facto methodology for privacy-aware LLM adaptation \cite{cai2023efficient, zhang2023fedpetuning, lin2021fednlp, xu2024fwdllm}. Under this paradigm, multiple end devices independently fine-tune a local copy of a global LLM (initialized by a central server) using their private data. These devices then transmit only model updates, not sensitive user data, to the central server for global aggregation (\eg, via weighted averaging \cite{mcmahan2017communication}).

\noindent \textbf{Challenges.} 
% Given the vast number of parameters in LLMs and limited resources (\eg, communication bandwidth, computing power, and memory) on end devices, the practical deployment of efficient federated fine-tuning systems is challenging. 
% The constraints are threefold: (1) Transmission of model updates between devices and the server incurs excessive \textbf{communication} costs (\eg, communication time); (2) Expensive on-device \textbf{computation} for updating LLMs introduces significant delays; (3) Fine-tuning LLMs requires unaffordable \textbf{storage} space on end devices.
% For instance, in each federated round, fine-tuning a relatively small LLM (GPT-2 \cite{radford2019language}) on each device even requires $12$ GB of network traffic and over $15$ petaFLOPs of computation. Considering that typical end devices are capable of $<2$ TFLOPS of computational capability and $<100$ Mbps of bandwidth, one round of federated fine-tuning can take several hours, and the end-to-end convergence time can extend to hundreds of hours \cite{cai2023efficient}. Moreover, fine-tuning GPT-2 necessitates about $30$ GB of memory, which is impractical for most end devices, typically equipped with $<16$ GB of GPU memory \cite{kang2021benchmarking, magalhaes2023benchmarking, baller2021deepedgebench}.
Given the vast number of parameters in LLMs and the limited resources (\eg, communication bandwidth, computing power, and memory) available on end devices, the practical deployment of efficient federated fine-tuning systems remains challenging. The challenges are threefold: (1) Transmission of model updates between devices and the server incurs excessive \textbf{communication} time; (2) Expensive on-device \textbf{computation} for updating LLMs introduces significant delays; (3) Fine-tuning LLMs requires unaffordable \textbf{storage} space on end devices.
For instance, in each federated round, fine-tuning a relatively small LLM (GPT-2 \cite{radford2019language}) on each device even requires $12$ GB of network traffic and over $15$ petaFLOPs of computation. Considering that typical end devices are capable of $<2$ TFLOPS of computational capability and $<100$ Mbps of bandwidth, one round of federated fine-tuning can take several hours, and the end-to-end convergence time can extend to hundreds of hours \cite{cai2023efficient}. Moreover, fine-tuning GPT-2 necessitates about $30$ GB of memory, which is impractical for most end devices, typically equipped with $<16$ GB of GPU memory \cite{kang2021benchmarking, magalhaes2023benchmarking, baller2021deepedgebench}.

\noindent \textbf{Status quo and limitations.} 
Recent research on federated fine-tuning primarily addresses the communication issue, with federated parameter-efficient fine-tuning (PEFT) \cite{cai2023efficient, zhang2023fedpetuning, jiang2023low, cho2023heterogeneous} emerging as the dominant strategy. However, the fine-tuning overhead remains significant for developers. Specifically, PEFT inserts lightweight trainable modules into the LLM while keeping the base model frozen. During communication rounds, only parameter updates from the added modules are shared between devices and the server.
Since the size of these modules is typically less than 5\% of the base LLM, network traffic for federated fine-tuning is significantly reduced. However, PEFT cannot fundamentally address the computation and storage challenges, which act as primary bottlenecks of federated fine-tuning. As illustrated in Table \ref{tab:memory_time}, while communication time has decreased by over $99\%$ with the PEFT methods, computation time remains substantially high (\eg, about one hour per round on each device), accounting for more than 99\% of the total fine-tuning time. Moreover, PEFT provides limited memory savings (approximately $30\%$), making it impractical to deploy popular LLMs on real-world end devices with $< 16$ GB of memory. More severely, even only a portion of that memory on end devices can be allocated for fine-tuning tasks without compromising user experience \cite{lebeck2020end, li2017optimizing}.
% Recent research on federated fine-tuning primarily addresses the communication issue; however, the fine-tuning overhead remains significant for developers. Federated parameter-efficient fine-tuning (PEFT) \cite{cai2023efficient, zhang2023fedpetuning, jiang2023low, cho2023heterogeneous} has emerged as the dominant strategy to  improve communication efficiency. Specifically, PEFT inserts lightweight trainable modules into the LLM while keeping the base model frozen. During communication rounds, only parameter updates from the added modules are shared between devices and the server.
% Since the size of these modules is typically less than 5\% of the base LLM, network traffic for federated fine-tuning is significantly reduced. However, PEFT cannot fundamentally address the computation and storage challenges, which act as primary bottlenecks of federated fine-tuning. As illustrated in Table \ref{tab:memory_time}, while communication time has decreased by over $99\%$ with the PEFT methods, computation time is only reduced by $32.0\%$-$34.9\%$. Consequently, computation time accounts for more than 99\% of the total fine-tuning time. Moreover, PEFT provides limited memory savings (approximately $30\%$), making it impractical to deploy popular LLMs on real-world end devices. More severely, even only a portion of that memory on end devices could be used for fine-tuning tasks without compromising user experience \cite{lebeck2020end, li2017optimizing}.

\begin{table}[t]
    \includegraphics[width=8.5cm]{content/picture/first_chapter/time_memory.pdf}
\caption{Communication (both downlink/uplink), computation, and storage overhead during a single round on each device. Model: DeBERTa-xxlarge (1.5B) \cite{he2020deberta}; Dataset: MNLI \cite{wang2018glue}; End device: Jetson AGX \cite{agx}, a high-performance embedded device; Bandwidth: 40 Mbps.}
\label{tab:memory_time}
\vspace{-0.5cm}
\end{table}

% Table \ref{} reports the 
% % PEFT has two fundamental bottlenecks that throttle its practicality due to its \emph{additive} design philosophy: it grafts new parameters onto each transformer layer in the LLM rather than compressing these layers (\S \ref{subsec:limitations}).

% % However, PEFT has two fundamental bottlenecks that throttle its practicality (\S \ref{subsec:limitations}). The root cause lies in PEFT's \emph{additive} design philosophy: it grafts new parameters onto each transformer layer in the LLM rather than compressing these layers. 

\noindent \textbf{Root causes of limitations.} The computation and storage bottlenecks in PEFT stem from its \emph{additive} design philosophy: it grafts new parameters onto each transformer layer in the LLM rather than compressing these layers. First, the architectural choice of PEFT imposes an unaffordable computational burden: during fine-tuning, inputs must propagate through \emph{all} transformer layers, even those with frozen parameters. While PEFT accelerates the backward pass during fine-tuning, the computational graph of the forward pass for the frozen base model remains intact. The majority of FLOPs in the forward pass originate from the frozen base model, which PEFT does not skip. Consequently, PEFT fails to optimize the forward pass, whose computational load remains nearly identical to full fine-tuning (FFT)\footnote{FFT updates all parameters in the LLM during the backward pass.}, accounting for about 45\% of the total on-device computation time (\S \ref{subsec:limitations}). Second, fine-tuning LLMs necessitates extensive GPU memory to store intermediate results, \ie, activations \cite{korthikanti2023reducing}. This is because gradients used to update PEFT modules depend recursively on activations from preceding transformer layers. For example, computing gradients for a PEFT module at layer $L$ requires cached activations from layer $(L-1)$. Thus, \emph{all} layers must retain intermediate activations to support gradient calculations.
Consequently, the activations generated during the forward pass take up most of the memory usage ($>79\%$), which cannot be eliminated by PEFT (\S \ref{subsec:limitations}).
% Second, fine-tuning LLMs necessitates extensive GPU memory to store intermediate results, such as activations and gradients \cite{korthikanti2023reducing}. Gradients for PEFT modules depend recursively on activations from preceding transformer layers. For example, computing gradients for a PEFT module at layer $L$ requires cached activations from layer $(L-1)$. Thus, \emph{all} layers must retain intermediate activations to support gradient calculations. Although PEFT avoids storing gradients for most frozen parameters, activations alone still consume considerable memory. 

% Since LLMs typically contain a significant number of transformer layers \cite{michel2019sixteen, voita2019analyzing}, PEFT introduces substantial computing and memory overheads for all layers. Consequently, federated fine-tuning of even modest LLMs like GPT-2 remains infeasible for resource-constrained devices, \eg, those with computational capabilities of $<10$ tera operations per second (TOPS) and $<10$GB GPU memory. 
% This raises a pivotal question: \emph{Can we redesign PEFT to strategically bypass certain layers, eliminating both their computations and activations without compromising model fidelity?}

% The root cause lies in PEFT's \emph{additive} design philosophy: it grafts new parameters onto each transformer layer in the LLM rather than compressing these layers. This architectural choice imposes an unavoidable tax: during fine-tuning, inputs must propagate through \emph{all} transformer layers. As a result, the frozen base model's computational graph of the forward pass remains intact. Besides, gradients for PEFT modules depend recursively on activations from preceding transformer layers. For example, computing gradients for a PEFT module at layer $L$ requires cached activations from layer $(L-1)$. Thus, \emph{all} layers must retain intermediate activations to support gradient calculations. Since LLMs typically contain a significant number of redundant layers \cite{michel2019sixteen, voita2019analyzing}, PEFT introduces substantial computing and memory overheads.
% This raises a pivotal question: \emph{Can we redesign PEFT to strategically bypass redundant layers, eliminating both their computations and activations without compromising model fidelity?}


\noindent \textbf{Our solution.} We thereby present an efficient system called DropPEFT, which introduces a novel layer-wise optimization strategy, \ie, stochastic transformer layer dropout, as the key building block to enhance PEFT. Unlike conventional PEFT methods that retain all transformer layers during training, Yagi dynamically identifies and skips certain computationally costly layers in both forward and backward passes. This innovation hinges on a key insight: transformer layers exhibit considerable redundancy, enabling selective deactivation without catastrophic knowledge loss \cite{men2024shortgpt, song2024sleb, chen2024compressing}.
% Shortgpt: Layers in large language models are more redundant than you expect
% SLEB: Streamlining LLMs through Redundancy Verification and Elimination of Transformer Blocks
% Compressing large language models by streamlining the unimportant layer

% \begin{table}[t]
%     \includegraphics[width=8.5cm]{content/picture/first_chapter/advantages.pdf}
% \caption{Yagi is efficient in communication, computation and storage.}
% \label{tab:advantages}
% \vspace{-0.5cm}
% \end{table}

At its core, Yagi operates through probabilistic layer dropout. During each training batch, participating devices fine-tune the LLM by stochastically deactivating subsets of transformer layers according to certain probabilities (\ie, drop rates). Inputs propagate only through activated layers, while deactivated layers reuse activations from their nearest active predecessors. Critically, this dropout is temporary and dynamic: a layer deactivated in one batch may be reactivated in subsequent batches, ensuring all layers in the LLM contribute cumulatively over time. By stochastic transformer layer dropout, Yagi eliminates both computations and activations for deactivated layers. Consequently, the memory usage and training time required for fine-tuning are significantly reduced.

However, unleashing Yagi's full potential presents a key technical challenge: \emph{How to design an effective strategy to assign an appropriate drop rate to each transformer layer.} This drop-rate configuration govern the trade-off between fine-tuning efficiency and model fidelity. Overly aggressive dropout introduces a risk of degrading the model performance, while overly conservative drop rates squander computational resources. Compounding this, the importance of a layer varies with its position in the LLM. For instance, deeper layers may prioritize semantic coherence while shallower layers tend to extract shallow features.
% Besides, since different layers have various importance, proper distributions of drop rates cross layers are essential for model performance. 
The choice is also dynamic: the favorable drop-rate configuration drifts over time and devices, depending on the learning progress and changing resources. 
To address this, Yagi employs an online exploration-exploitation strategy that dynamically optimizes drop rates based on real-time rewards, quantified as model accuracy gains per unit wall-clock time. This adaptive mechanism evaluates candidate configurations through a multi-armed bandit framework, prioritizing high-reward dropout policies while maintaining exploratory diversity. By continuously adapting to device and learning-phase demands, Yagi achieves efficient and effective federated fine-tuning.
% To address this challenge, we identify configurations with high rewards, which are measured in terms of their model accuracy gains per unit wall clock time. We then employ an online exploration-exploitation strategy to dynamically select configurations with high rewards for efficient and effective model fine-tuning (\S \ref{}).
% efficient and effective federated fine-tuning.

% % \begin{figure}[t] \centering
% %     \includegraphics[width=0.485\textwidth]
% %     {content/picture/first_chapter/P3_overview.pdf}
% %     \caption{Significant communication costs, computational overheads, and challenges posed by non-IID data are key bottlenecks in federated NLP. P$^{3}$ overcomes these obstacles trough novel techniques.}\label{fig:overview}
% % \end{figure}

% On the other hand, one misconception in traditional federated NLP is that all local model parameters on devices should be aggregated into a single global model. This not only maximizes communication costs between devices and the server, but also fails to account for the inherently non-IID device data. Therefore, we propose personalized
% transformer layer sharing to address this challenge (\S \ref{sec:layer_sharing}). The motivation is that certain personalized local encoders (\ie, certain transformer layers and the LLM head) instead of a single global model can better process specialized local data. Having personalized encoders extract useful local representations means that the global model now requires fewer number of layers. To this end, we partition each LLM on the device into two parts, \ie, personalized layers (with the LLM head) and global shared layers. In particular, layer partitioning on each device is driven by its local data, leading devices holding similar data distributions to share similar layer architectures and more overlapped parameters. After local fine-tuning in each round, devices only transmit the shared layers to the central server for global aggregation (\S 4.2). Consequently, LLMs on devices are able to capture representations embedded in local data while effectively sharing collective knowledge derived from global data.

\noindent \textbf{Contributions.} 
% Figures \ref{fig:overview} illustrates the practical challenges in federated NLP and the high-level overview of P$^{3}$. 
% Table \ref{tab:advantages} summarizes advantages of Yagi over prior literature. 
Overall, we make the following contributions in this paper:
\begin{itemize}[leftmargin=*]
    \item We analyze the limitations of PEFT in computation and storage efficiency. To make federated fine-tuning practical for end devices, we propose Yagi to enhance PEFT with a novel layer-wise strategy, \ie, stochastic transformer layer dropout.
    % \item We enhance federated fine-tuning with two novel layer-wise strategies: stochastic transformer layer dropout and personalized transformer layer sharing.
    \item We identify the challenges of the drop-rate configuration in Yagi, then design an online exploration-exploitation algorithm to determine the optimal configuration for efficient and effective layer dropout.
    \item Through experiments on real hardware, we show Yagi outperform state-of-the-art solutions across various datasets and models.
    
    
    
    
    % We propose P$^{3}$, a novel and efficient federated NLP framework that enhances system efficiency and model performance on non-IID text data.
    % \item To the best of our knowledge, P$^{2}$ is the first framework that achieves personalization while jointly improving the efficiency of communication and computation in federated NLP. We believe that our work represents a significant step towards applying practical federated NLP to resource-constrained mobile devices.
    % \item P$^{2}$ contributes several effective techniques, \eg, personalized pruning techniques and PET methods, that address the limitations in state-of-the-arts of federated NLP.
    % \item Addressing practical challenges in federated NLP, we extend P$^{3}$ to settings with devices having heterogeneous computational capabilities.
    % \item P$^{3}$ outperforms state-of-the-arts [9, 15 , 17, 18] across various datasets and NLP models on both system efficiency and model performance. Specifically, P$^{3}$ reduces communication and computation costs by 23.71\%-49.71\% and 23.71\%-49.71\%, respectively, while achieving 3.68\%-7.33\% higher final test accuracy, compared with state-of-the-arts.
\end{itemize}
 

==> content/motivation.tex <==
In this section, we highlight key limitations of existing solutions for federated NLP and outline opportunities that motivate our work (\S \ref{subsec:limitations}).

\subsection{Limitations of Status Quo}\label{subsec:limitations}
While existing federated NLP solutions have made considerable progress
in reducing training costs, they have large optimization spaces in fully exploiting both system efficiency and model performance due to the issues discussed below.\\
\textbf{PEFT is suboptimal in computing efficiency.} Fine-tuning a model on-device involves both forward and backward passes. Traditional PEFT methods could only improve the efficiency of the backward pass but fail to reduce the computational demands of the forward pass. As shown in Figure \ref{fig:computing_path}, while PEFT methods freeze the parameters in the original pre-trained network to avoid gradient calculation during the backward pass, the forward pass remains computationally burdensome. The frozen parameters do not alter the computational graph and operations in the forward pass, leaving the full forward path intact. Common language models, such as LLaMA 2-7B, contain billions of parameters accessed during the forward pass, making it computationally demanding in terms of GPU memory and training time.
% Moreover, PEFT introduces additional structures (\eg, adapters or LoRA modules) into the network, which can further increase the computation complexity for forward pass due to the added operations.
To illustrate this, we fine-tune GPT-2 and LLaMA 2-7B on Semeval using an A6000 GPU, and record time for the forward pass, backward pass, and other tasks (\eg, data loading and optimizer stepping) over 100 batches. As shown in Figure \ref{fig:breakdown-time}, the backward pass is a major bottleneck in full fine-tuning, consuming nearly 60$\sim$63\% of total training time. Although PEFT methods effectively reduce backward pass computation, they fail to address the forward pass overhead, which now emerges as a primary bottleneck in model fine-tuning.
According to our experimental results, forward pass computation alone accounts for at least 50\% of the total training time in the PEFT process.
% Therefore, it is important to find a method that can effectively optimize both the forward and backward pass simultaneously.\\
% \textbf{Suboptimality in system efficiency.}
% % While PEFT methods in federated NLP can effectively reduce training overheads, they have limitations and optimization spaces in fully exploiting both system efficiency and model performance. 
% First, an entire local LLMs fine-tuning process includes both the forward and backward propagation steps. Traditional PEFT methods could only exploit the backward propagation efficiency but not that of forward propagation. Specifically, in PEFT process, freezing the original parameters in the pre-trained LLM can only avoid calculating their gradients in backward propagation. However, overall computational graph and operations remain largely unchanged, leading to original forward propagation path remaining intact. Besides, LoRA and Adapter introduce lightweight modules, which still require computation during the forward pass. In some cases, this can even lead to a slight increase in computation time due to the extra operations involved. As we illustrate in the following, such an inefficient computing strategy leaves a large room for improvement.
% To illustrate this, we conduct 

\noindent \textbf{Model pruning is inflexible and costly.} Standard federated learning algorithms such as FedAvg \cite{mcmahan2017communication} assume that all clients share the same model architecture with the central server. However, in federated NLP systems, devices always have different computational capabilities and communication bandwidths \cite{lai2021oort, li2022pyramidfl}, necessitating heterogeneous pruning strategies tailored to the specific constraints of each device. This directly violates the fundamental assumption in FL, thus requiring complex new algorithms or adaptations to handle varying model architectures across devices while ensuring effective learning and convergence. Moreover, the computational resources available on the devices are not static; they change dynamically over time due to factors such as background processes, battery levels, or network conditions. Yet, model pruning is typically executed as a one-time process \cite{ma2023llm, zhang2024structured}, fixing the model size after pruning and rendering it incapable of adapting to the changing system resources of devices. This rigidity prevents model pruning from being responsive to temporal changes in device capabilities, limiting its practical applicability in dynamic environments.
\begin{figure}[t]\centering
    \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/computing_path.pdf}
    \caption{Illustration of forward and backward passes in parameter-efficient fine-tuning.}\label{fig:computing_path}
\end{figure}
\begin{figure}[t]\centering
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[GPT-2.]{\centering
                \label{fig:breakdown-time-GPT-2}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/time-breakdown.pdf}
            }
    \end{minipage}
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[LLaMA 2-7B.]{\centering
                \label{fig:breakdown-time-LLaMA}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/time-breakdown.pdf}
            }
    \end{minipage}
    \caption{Breakdown of training time for fine-tuning models using an A6000 GPU.}\label{fig:breakdown-time}
\end{figure}
In addition to its inflexibility, performing model pruning operations itself, which is computationally intensive, inevitably incurs extra computational overhead on devices. This overhead is particularly problematic with large language models, whose substantial size and computational complexity exacerbate the issue. In federated NLP, devices, such as smartphones and edge devices, generally have limited computational resources. Additional pruning calculations can lead to higher energy consumption, increased training latency, and a larger memory footprint, which is undesirable for devices that are resource-constrained.

\noindent \textbf{PEFT and pruning suffer poor model performance.} 
% Fine-tuning only a subset of a model's parameters inherently constrains its ability to learn task-specific nuances, leading to suboptimal model performance compared to full fine-tuning.
% In federated NLP, this limitation is further exacerbated when each client possesses data that is not independently and identically distributed (non-IID). PEFT might not generalize effectively across these heterogeneous client datasets, leading to inconsistent and often inadequate performance \cite{zhang2023fedpetuning}. Moreover, model pruning typically relies on global importance measures of parameters, which are hard to compute without centralized data. Parameters deemed unimportant on one client's data may be crucial when considering the entire dataset distributed across all clients. The primary incentive for devices to participate in federated NLP is learning a global model that outperforms models trained locally \cite{li2021hermes}. However, when data heterogeneity is present, locally fine-tuned models often outperform the globally fine-tuned model produced by PEFT and pruning methods. This outcome not only undermines the fundamental motivation for federated NLP but also raises questions about the efficacy of these methods.
In federated NLP, the local data across different clients is not independently and identically distributed (non-IID) \cite{zhang2023fedpetuning, lin2021fednlp}. PEFT might not generalize effectively across these heterogeneous client datasets, leading to inconsistent and inadequate model performance \cite{zhang2023fedpetuning}. Moreover, model pruning typically relies on global importance measures of parameters, which are hard to compute without centralized data. Parameters deemed unimportant on one client's data may be crucial when considering the entire dataset distributed across all clients. These facts lead to suboptimal model performance of PEFT and pruning compared to full fine-tuning. To demonstrate this issue, we apply three classical PEFT and pruning technologies to fine-tune two popular NLP models (\ie, xxx and xxx) with the xxx dataset over 100 communication rounds. In each round, we randomly select 10 out of 100 devices for training.
To simulate real-world non-IID data distributions, we follow the prior works \cite{zhang2023fedpetuning, lin2021fednlp, cai2023efficient} and partition the dataset using three Dirichlet distributions, \ie, $Dir(10.0)$, $Dir(1.0)$, $Dir(0.1)$, which represent low, medium, and high non-IID degrees, respectively. As shown in Figure \ref{fig:acc-iid}, 
the final model accuracy of the PEFT and pruning methods (\ie, FedAdapter, FedLoRA and FedPruning) is far from that of full fine-tuning (\ie, FedFull). As the non-IID degree changes from low to high, the performance gaps between these methods and full fine-tuning even sharply increase.
% the PEFT and pruning methods suffer poor model performance in non-IID situations. 
\begin{figure}[t]\centering
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[GPT-2.]{\centering
                \label{fig:}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/acc-iid.pdf}
            }
    \end{minipage}
    \begin{minipage}[t]{0.495\linewidth}\centering
        \subfigure[LLaMA 2-7B.]{\centering
                \label{fig:}
                \includegraphics[width=1.0\linewidth]{content/picture/second_chapter/acc-iid.pdf}
            }
    \end{minipage}
    \caption{PEFT and model pruning are suboptimal in model performance.}\label{fig:acc-iid}
\end{figure}

Moreover, the primary incentive for devices to participate in federated NLP is learning a global model that outperforms models trained locally \cite{li2021hermes}. However, when data heterogeneity is present, locally fine-tuned models (\ie, LocalFull) often outperform the globally fine-tuned model produced by PEFT and pruning methods, as shown in Figure \ref{fig:acc-iid}. This outcome not only undermines the fundamental motivation for federated NLP but also raises questions about the efficacy of these methods.





% The primary incentive for devices to participate in federated NLP is learning a global model that outperforms models trained locally \cite{li2021hermes}. However, when data heterogeneity is present, locally fine-tuned models often outperform the globally fine-tuned model produced by PEFT and pruning methods. This outcome not only undermines the fundamental motivation for federated NLP but also raises questions about the efficacy of these methods.

% To empirically demonstrate this issue, we apply three classical PEFT and pruning technologies to fine-tune the xxx model using the xxx dataset over communication 100 rounds. In each round, we randomly select 10 out of 100 devices for training.
% To simulate a non-IID data distribution, we follow the prior works \cite{zhang2023fedpetuning, lin2021fednlp, cai2023efficient} and partition the dataset using a Dirichlet distribution $Dir(1.0)$. 
% % In particular, we sample local dataset $_{i}\sim Dir_{i}(\alpha)$ and allocate it to device $i$, where $\alpha$ determines the non-IID degree, and a lower value of $\alpha$ generates a high label distribution shift. In this experiment, we set $\alpha=1.0$.
% The experimental results in Figure \ref{} show that the globally trained models utilizing PEFT and pruning methods achieve an accuracy of 47.67\%, while the models fine-tuned locally attain an average accuracy of up to 65.44\%. 
% % Therefore, it is of a great challenge to train a good, one-fits-all model working consistently well for all devices with heterogeneous data.

% % The pruning process may need to be adaptive over time as devices' system resources (\eg, available GPU memory and communication bandwidth) change. Managing these dynamic changes in a federated environment adds complexity to both the client-side operations and the server-side aggregation process. Such pruning process inevitably incurs extra computational overhead.





% \begin{table}[t]
%     \centering
%     \caption{Opportunities for advanced federated NLP solutions.} \label{table:}
%     \resizebox{83mm}{!}{
%         \centering
%         \begin{tabular}{|c|c|c|c|c|}  
%     		\hline
%     		% & & & \\[-6pt]  %可以避免文字偏上来调整文字与上边界的距离
%     		Solutions & \makecell{Efficient\\Forward Pass} & \makecell{Flexible\\Sub-Network} & \makecell{No Extra\\Overhead} & \makecell{High Model\\Performance}\\  % 表格中的内容，用&分开，\\表示下一行
%             % \cmidrule{4-5}
%             \hline
%     		% & & & \\[-6pt]  %可以避免文字偏上 
%     		\rule{0pt}{15pt} PEFT & \XSolidBrush & \XSolidBrush & \CheckmarkBold & \XSolidBrush \\ [4pt]
%     		\hline
%             \rule{0pt}{15pt} Pruning & \CheckmarkBold & \XSolidBrush & \XSolidBrush & \XSolidBrush \\ [4pt]
%     		\hline
%             \makecell{Advanced\\Method} & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold \\
%     		\hline
%         \end{tabular}
%     }
% \end{table}


% In summary, existing techniques are inadequate for federated NLP in terms of system efficiency and model performance.
% To enable practical federated NLP with optimized training overheads and performance, the model structure and training paradigm need to be re-architected.
% In an ideal situation, we would be able to extract sub-networks automatically and dynamically from this over-parameterized network, for any real-time given memory or training time constraint, while maintaining good performance.

% Large language models are extremely redundant due to their significant number of parameters. This makes it possible to compress large language models without having a drastic effect on performance. 
% Various papers \cite{michel2019sixteen, voita2019analyzing} have shown evidence that Transformers are over-parameterized.

% The resulting network learns to be explicitly robust, comparing to more complicated model pruning schemes while at the same time being extremely simple to implement.

% To address these problems, we propose Layer dropoutping, a training procedure that enables the seemingly contradictory setup to train shallow networks and use deep networks at inference time.
% In this paper, we propose deep networks with stochastic depth, a novel training
% algorithm that is based on the seemingly contradictory insight that ideally
% we would like to have a deep network during testing but a short network during
% training.
% \begin{table}[t]
%     \centering
%     \caption{Communication and computation costs within one training round for a single Jetson TX2 device in federated NLP. Specifically, we fine-tune (FT) three popular LLMs on the 20NEWS dataset.} \label{table:efficiency_peft}
%     \resizebox{85mm}{!}{
%         \centering
%         \begin{tabular}{c|c|c|c}  
%     		\hline
%     		% & & & \\[-6pt]  %可以避免文字偏上来调整文字与上边界的距离
%     		Model & Method & Computing Time &  Network Traffic \\  % 表格中的内容，用&分开，\\表示下一行
%             \hline
%             \multirow{3}{*}{Bert-Large} & Full FT & 10.3 mins & 1.3GB \\
%             % \cmidrule(r){2-4}
%             & Adapter & 7.9 mins & 8.2MB \\
%             % \cmidrule(r){2-4}
%             & LoRA & 6.1 mins & 4.1MB \\
%             \hline
%             \multirow{3}{*}{GPT-2} & Full FT & 42.3 mins & 6.1GB \\
%             % \cmidrule(r){2-4}
%             & Adapter & 31.1 mins & 50.9MB \\
%             % \cmidrule(r){2-4}
%             & LoRA & 26.9 mins & 32.7MB \\
%             \hline
%             \multirow{3}{*}{LLaMA 2-7B} & FT & 134.8 mins & 28.2GB \\
%             % \cmidrule(r){2-4}
%             & Adapter & 97.1 mins & 312.7MB \\
%             % \cmidrule(r){2-4}
%             & LoRA & 88.2 mins & 256.9MB \\
%             \hline
%         \end{tabular}
%     }
% \end{table}

==> content/overview.tex <==
The core of our method is to dynamically sample small sub-networks from the larger model at the beginning of each batch of training by randomly dropping transformer layers.
We start with very deep networks but during training, for each mini-batch, randomly drop a subset of layers and bypass them with the identity function.
during training we shorten the network significantly by randomly
removing a substantial fraction of layers independently for each sample or
mini-batch.

An advantage of our layer dropping technique is that from one single local language model on the client, we can extract shallow sub-networks of any desired depth on demand for global aggregation.

To address these problems, we propose Layer Dropping, a training procedure that enables the seemingly contradictory setup to train shallow networks and use deep networks at inference time.

These PEFT approaches are complementary to our Layer Drop method and should benefit from each other.

Shortening the expected depth during training reduces not only the
chain of forward pass steps but also gradient computations of backward pass. Besides, Layer Dropping can strengthen the gradients especially in earlier layers during backward pass.

Networks trained with stochastic depth can be interpreted as an implicit ensemble of networks of different depths.

To reduce the effective length of a neural network during training, we randomly skip layers entirely.

We achieve this by introducing skip connections, however the connection pattern is randomly altered for each minibatch.
For each mini-batch we randomly select sets of layers and remove their corresponding transformation functions, only keeping the identity skip connection.

Unlike quantization or sparsity, acceleration by reducing number of layers does not require specialized hardware or software kernels.

if layer $l$ is dropped and $H_{l}$ denotes the output of the $l$-th layer, we obtain $H_{l} = Identify(H_{l-1})$, where $Identify(\cdot)$ denotes the identify transformation. Figures \ref{fig:dropped-layer} illustrates an example of the identify transformation function.
Stochastic depth aims to shrink the depth of a network during training,
while keeping it unchanged during inference. We can achieve this goal by randomly dropping entire transformer layers during training and bypassing their transformations through the identify transformation function.
\begin{figure*}[t]\centering
    \includegraphics[width=1.0\linewidth]{content/picture/design_chapter/dropped_layer.pdf}
    \caption{A close look at the dropped layer with an identify transformation function in a transformer-based language model.}\label{fig:dropped-layer}
\end{figure*}
Let $d_{l}\in\{0, 1\}$ denote a Bernoulli random variable, which indicates whether the $l$-th transformer layer is active ($d_{l}=0$) or inactive ($d_{l}=1$).
Further, let us denote the probability of dropping the layer $l$ as $p_{l} = Probability(d_{l}=1)$.
With this definition we can bypass the $l$-th transformer layer by multiplying its function $trans_{l}(\cdot)$ with $(1-d_{l})$, \ie, $H_{l} = (1-d_{l})\cdot trans_{l}(H_{l-1}) + d_{l} \cdot Identify(H_{l-1})$. If $d_{l}=0$, it reduces to the original $l$-th transformer transformation function $H_{l}=trans_{l}(H_{l-1})$. If $d_{l}=1$, it reduces to the identify transformation function $H_{l}=Identify(H_{l-1})$.

$P=\{p_{l}, l=1, 2, ... , L\}$ are new hyper-parameters of our training procedure. One option is to set $p_{l} = p$ uniformly for all $l$ to obtain a single hyper-parameter $p$. Another possibility is in \cite{huang2016deep}.
\begin{figure*}[t]\centering
    \includegraphics[width=1.0\linewidth]{content/picture/design_chapter/layer_drop_ratio.pdf}
    \caption{Example of drop ratios of all layers. $p_{l}$ is the survival ratio the $l$-th layer.}\label{fig:layer-drop-ratios}
\end{figure*}

With stochastic depth, the number of effective transformer layer during training, denoted as $\widetilde{L}$, becomes a random variable. Its expectation is $E(\widetilde{L}) = \sum_{l=1}^{L}(1-p_{l})$. In other words, with stochastic depth, we train a language model with an average number of $E(\widetilde{L})$ layers for each batch, but recover a entire network with $L$ layer at inference time. Note that because the connectivity
is random, there will be updates with significantly shorter networks and more
direct paths to individual layers. Training with stochastic depth can be viewed as training an ensemble of sub-networks implicitly. Each of the $L$ layers is either active or inactive, resulting in $2^{L}$ possible network combinations. For each training mini-batch one of the $2^{L}$ networks (with shared weights) is sampled and updated. Stochastic depth during testing requires small modifications to the network. We keep transformer transformation functions of all layers active throughout inference in order to utilize the full-length network with all its model capacity. However, during training, function of the $l$-th layer is only active for a fraction $(1-p_{l})$ of all updates, and the corresponding weights of the next layer are calibrated for this probability. We therefore need to re-calibrate the outputs of any given function by the expected number of times it participates in training, \ie, $1-p_{l}$. The forward propagation update rule becomes $H_{l}=(1-p_{l})\cdot trans_{l}(H_{l-1}) + p_{l} \cdot Identify(H_{l-1})$. From the model ensemble perspective, the update rule can be interpreted
as combining all possible networks into a single inference architecture, in which each layer is weighted by its dropping probability.

we fine-tune a language model that is equivalent to an ensemble of sub-networks of various depths, capable of skipping from different transfomer layers to the LM head.

When a transformer layer is bypassed for a specific iteration,
there is no need to perform forward and backward computation or gradient updates. As the forward-backward computation dominates the training time, stochastic depth significantly speeds up the training process. The timings in practice using our implementation are consistent with this analysis
